The Southern HII Region Discovery Survey. II. The Full Catalog

The Southern HII Region Discovery Survey (SHRDS) is a 900 hour Australia Telescope Compact Array 4-10 GHz radio continuum and radio recombination line (RRL) survey of Galactic HII regions and infrared-identified HII region candidates in the southern sky. For this data release, we reprocess all previously published SHRDS data and include an additional ~450 hours of observations. The search for new HII regions is now complete over the range 259 deg < Galactic longitude < 346 deg, |Galactic latitude| < 4 deg for HII region candidates with predicted 6 GHz continuum peak brightnesses >30 mJy/beam. We detect radio continuum emission toward 730 targets altogether including previously known nebulae and HII region candidates. By averaging ~18 RRL transitions, we detect RRL emission toward 206 previously known HII regions and 436 HII region candidates. Including the northern sky surveys, over the last decade the HII Region Discovery Surveys have more than doubled the number of known Galactic HII regions. The census of HII regions in the WISE Catalog of Galactic HII Regions is now complete for nebulae with 9 GHz continuum flux densities > 250 mJy. We compare the RRL properties of the newly discovered SHRDS nebulae with those of all previously known HII regions. The median RRL full-width at half-maximum line width of the entire WISE Catalog HII region population is 23.9 km/s and is consistent between Galactic quadrants. The observed Galactic longitude-velocity asymmetry in the population of HII regions probably reflects underlying spiral structure in the Milky Way.

==> fields.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lccccccrl}
\centering
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Full Catalog Fields and Targets\label{tab:fields}}
\tablehead{
\colhead{Field} & \colhead{RA}         & \colhead{Dec.}       & \colhead{Target} & \colhead{Catalog\tablenotemark{a}} & \colhead{RA}         & \colhead{Dec.}       & \colhead{\(R_{\rm IR}\)}   & \colhead{Author} \\
\colhead{}      & \colhead{J2000}      & \colhead{J2000}      & \colhead{}       & \colhead{}                         & \colhead{J2000}      & \colhead{J2000}      & \colhead{(arcsec)}         & \colhead{}      \\
\colhead{}      & \colhead{(hh:mm:ss)} & \colhead{(dd:mm:ss)} & \colhead{}       & \colhead{}                         & \colhead{(hh:mm:ss)} & \colhead{(dd:mm:ss)} & \colhead{}                 & \colhead{}      
}
\startdata
ch1 & 07:30:05.8 & $-18$:32:27.2 & G233.676$-$00.186 & Q & 07:29:56.6 & $-18$:27:50.1 & $59.11$ &  \\
 & & & G233.753$-$00.193 & K & 07:30:04.6 & $-18$:32:03.9 & $311.06$ & B11  \\
 & & & G233.830$-$00.180 & G & 07:30:16.9 & $-18$:35:44.5 & $114.85$ &  \\
ch4 & 08:20:56.3 & $-36$:12:32.0 & G254.682+00.220 & K & 08:20:55.5 & $-36$:13:09.9 & $385.32$ & CH87  \\
shrds027 & 08:23:21.5 & $-40$:39:59.7 & G258.608$-$01.925 & Q & 08:23:21.7 & $-40$:39:57.7 & $136.61$ &  \\
shrds029 & 08:26:13.4 & $-40$:46:45.4 & G259.013$-$01.546 & Q & 08:26:13.5 & $-40$:46:45.0 & $68.08$ &  \\
 & & & G259.057$-$01.544 & C & 08:26:22.1 & $-40$:48:49.5 & $103.98$ &  \\
 & & & G259.086$-$01.612 & C & 08:26:09.9 & $-40$:52:36.2 & $103.98$ &  \\
shrds030 & 08:26:18.8 & $-40$:48:36.5 & G259.013$-$01.546 & Q & 08:26:13.5 & $-40$:46:45.0 & $68.08$ &  \\
 & & & G259.057$-$01.544 & C & 08:26:22.1 & $-40$:48:49.5 & $103.98$ &  \\
 & & & G259.086$-$01.612 & C & 08:26:09.9 & $-40$:52:36.2 & $103.98$ &  \\
shrds034 & 08:22:22.1 & $-41$:35:59.1 & G259.268$-$02.611 & Q & 08:22:22.3 & $-41$:35:57.5 & $94.53$ &  \\
shrds035 & 08:37:05.6 & $-39$:44:51.8 & G259.359+00.820 & C & 08:37:17.6 & $-39$:39:30.3 & $500.76$ &  \\
 & & & G259.771+00.541 & C & 08:37:25.8 & $-40$:09:15.3 & $3361.35$ &  \\
shrds036 & 08:22:52.1 & $-41$:42:22.8 & G259.409$-$02.595 & C & 08:22:52.2 & $-41$:42:22.1 & $146.41$ &  \\
shrds037 & 08:23:15.0 & $-41$:46:12.0 & G259.409$-$02.595 & C & 08:22:52.2 & $-41$:42:22.1 & $146.41$ &  \\
 & & & G259.502$-$02.573 & Q & 08:23:15.1 & $-41$:46:11.4 & $93.61$ &  \\
shrds041 & 08:21:43.7 & $-42$:05:42.9 & G259.608$-$02.991 & Q & 08:21:43.8 & $-42$:05:41.8 & $123.23$ &  \\
shrds042 & 08:23:02.2 & $-41$:55:53.8 & G259.612$-$02.698 & Q & 08:23:02.4 & $-41$:55:52.1 & $93.92$ &  \\
shrds051 & 08:26:45.1 & $-43$:32:10.3 & G261.319$-$03.063 & Q & 08:26:45.1 & $-43$:32:10.3 & $74.77$ &  \\
shrds053 & 08:34:46.5 & $-42$:37:46.8 & G261.449$-$01.345 & Q & 08:34:46.8 & $-42$:37:48.8 & $89.38$ &  \\
shrds054 & 08:31:54.7 & $-43$:14:51.5 & G261.634$-$02.134 & Q & 08:31:54.8 & $-43$:14:50.3 & $78.01$ &  \\
 & & & G261.638$-$02.095 & Q & 08:32:05.9 & $-43$:13:39.2 & $98.89$ &  \\
shrds055 & 08:32:05.8 & $-43$:13:40.1 & G261.634$-$02.134 & Q & 08:31:54.8 & $-43$:14:50.3 & $78.01$ &  \\
 & & & G261.638$-$02.095 & Q & 08:32:05.9 & $-43$:13:39.2 & $98.89$ &  \\
shrds056 & 08:34:07.5 & $-42$:57:59.9 & G261.648$-$01.642 & Q & 08:34:07.9 & $-42$:58:01.4 & $106.81$ &  \\
shrds057 & 08:35:04.5 & $-43$:00:50.6 & G261.790$-$01.531 & C & 08:35:04.6 & $-43$:00:50.0 & $108.63$ &  \\
shrds058 & 08:34:27.3 & $-43$:34:47.5 & G262.176$-$01.960 & Q & 08:34:27.3 & $-43$:34:47.2 & $80.19$ &  \\
shrds060 & 08:48:40.9 & $-42$:53:10.3 & G263.237+00.509 & C & 08:48:44.0 & $-42$:54:01.6 & $204.56$ &  \\
shrds061 & 08:53:09.2 & $-42$:13:01.3 & G262.578+01.423 & Q & 08:50:18.6 & $-41$:48:42.5 & $2328.89$ &  \\
 & & & G263.227+01.572 & Q & 08:53:09.4 & $-42$:12:59.4 & $103.52$ &  \\
shrds063 & 08:49:49.2 & $-43$:09:37.3 & G263.554+00.656 & C & 08:50:27.3 & $-43$:03:08.8 & $1043.51$ &  \\
ch5 & 08:45:35.0 & $-43$:51:05.9 & G263.615$-$00.534 & K & 08:45:34.1 & $-43$:50:55.8 & $391.20$ & CH87  \\
shrds067 & 08:58:13.7 & $-42$:37:38.2 & G264.124+01.926 & Q & 08:57:45.5 & $-42$:40:20.8 & $269.04$ &  \\
 & & & G264.146+02.021 & C & 08:58:13.8 & $-42$:37:37.0 & $103.85$ &  \\
ch6 & 08:56:29.2 & $-43$:05:38.8 & G264.343+01.457 & K & 08:56:35.4 & $-43$:08:37.7 & $390.07$ & CH87  \\
shrds070 & 08:46:39.3 & $-45$:00:53.2 & G264.647$-$01.110 & Q & 08:46:39.4 & $-45$:00:53.0 & $70.24$ &  \\
shrds071 & 08:50:20.5 & $-44$:29:56.9 & G264.597$-$00.246 & Q & 08:50:15.6 & $-44$:25:51.3 & $78.15$ &  \\
 & & & G264.670$-$00.285 & C & 08:50:20.9 & $-44$:30:44.4 & $140.64$ &  \\
shrds074 & 08:59:26.5 & $-43$:26:08.6 & G264.903+01.660 & Q & 08:59:26.7 & $-43$:26:07.0 & $104.02$ &  \\
ch7 & 08:59:28.8 & $-43$:45:28.7 & G265.151+01.454 & K & 08:59:28.8 & $-43$:45:28.6 & $809.98$ & CH87  \\
shrds075 & 08:50:35.2 & $-45$:10:44.6 & G265.191$-$00.641 & C & 08:50:39.7 & $-45$:08:28.0 & $124.22$ &  \\
shrds078 & 08:58:03.7 & $-47$:22:59.3 & G267.730$-$01.100 & G & 08:58:05.4 & $-47$:22:43.9 & $200.97$ &  \\
 & & & G267.935$-$01.075 & K & 08:58:59.6 & $-47$:31:03.8 & $557.50$ & CH87  \\
ch9 & 08:59:04.7 & $-47$:31:16.2 & G267.935$-$01.075 & K & 08:58:59.6 & $-47$:31:03.8 & $557.50$ & CH87  \\
ch10 & 09:02:02.1 & $-47$:45:32.7 & G268.419$-$00.843 & K & 09:01:55.4 & $-47$:43:44.1 & $263.78$ & CH87  \\
shrds081 & 09:03:03.1 & $-47$:51:18.3 & G268.618$-$00.739 & C & 09:03:10.3 & $-47$:48:32.5 & $170.01$ &  \\
shrds082 & 09:01:24.6 & $-48$:34:47.9 & G269.001$-$01.469 & Q & 09:01:24.6 & $-48$:34:47.8 & $63.30$ &  \\
 & & & G269.174$-$01.436 & K & 09:02:15.2 & $-48$:41:16.0 & $414.43$ & CH87  \\
ch11 & 09:03:26.3 & $-48$:27:31.4 & G269.068$-$01.114 & K & 09:03:17.1 & $-48$:23:40.2 & $290.19$ & CH87  \\
 & & & G269.158$-$01.137 & G & 09:03:32.4 & $-48$:28:38.6 & $64.13$ &  \\
 & & & G269.159$-$01.119 & G & 09:03:37.5 & $-48$:27:57.9 & $64.13$ &  \\
 & & & G269.186$-$01.177 & Q & 09:03:28.3 & $-48$:31:29.3 & $64.13$ &  \\
shrds085 & 09:03:36.9 & $-48$:28:13.1 & G269.068$-$01.114 & K & 09:03:17.1 & $-48$:23:40.2 & $290.19$ & CH87  \\
 & & & G269.158$-$01.137 & G & 09:03:32.4 & $-48$:28:38.6 & $64.13$ &  \\
 & & & G269.159$-$01.119 & G & 09:03:37.5 & $-48$:27:57.9 & $64.13$ &  \\
 & & & G269.186$-$01.177 & Q & 09:03:28.3 & $-48$:31:29.3 & $64.13$ &  \\
shrds086 & 09:02:31.5 & $-48$:38:04.8 & G269.167$-$01.357 & G & 09:02:35.2 & $-48$:37:46.8 & $63.30$ &  \\
 & & & G269.174$-$01.436 & K & 09:02:15.2 & $-48$:41:16.0 & $414.43$ & CH87  \\
shrds087 & 09:03:28.3 & $-48$:31:29.6 & G269.068$-$01.114 & K & 09:03:17.1 & $-48$:23:40.2 & $290.19$ & CH87  \\
 & & & G269.158$-$01.137 & G & 09:03:32.4 & $-48$:28:38.6 & $64.13$ &  \\
 & & & G269.159$-$01.119 & G & 09:03:37.5 & $-48$:27:57.9 & $64.13$ &  \\
 & & & G269.186$-$01.177 & Q & 09:03:28.3 & $-48$:31:29.3 & $64.13$ &  \\
ch13 & 09:03:14.0 & $-48$:56:10.3 & G269.454$-$01.468 & K & 09:03:14.1 & $-48$:55:06.5 & $195.95$ & CH87  \\
shrds088 & 09:04:29.9 & $-48$:49:26.2 & G269.522$-$01.250 & Q & 09:04:30.0 & $-48$:49:25.9 & $103.74$ &  \\
 & & & G269.567$-$01.322 & C & 09:04:21.6 & $-48$:54:17.8 & $103.74$ &  \\
shrds089 & 09:04:21.3 & $-48$:54:19.9 & G269.522$-$01.250 & Q & 09:04:30.0 & $-48$:49:25.9 & $103.74$ &  \\
 & & & G269.567$-$01.322 & C & 09:04:21.6 & $-48$:54:17.8 & $103.74$ &  \\
shrds091 & 09:09:22.9 & $-48$:22:04.3 & G269.731$-$00.344 & C & 09:09:24.1 & $-48$:22:03.4 & $100.13$ &  \\
shrds094 & 09:04:33.2 & $-49$:41:15.0 & G270.171$-$01.820 & Q & 09:04:33.2 & $-49$:41:14.7 & $120.07$ &  \\
shrds095 & 09:05:45.5 & $-49$:37:29.1 & G270.141$-$01.607 & C & 09:05:24.6 & $-49$:31:19.9 & $264.39$ &  \\
 & & & G270.255$-$01.633 & Q & 09:05:45.7 & $-49$:37:27.8 & $94.75$ &  \\
ch15 & 09:24:29.5 & $-51$:59:35.1 & G274.004$-$01.152 & K & 09:24:24.0 & $-51$:59:40.7 & $424.67$ & CH87  \\
 & & & G274.122$-$01.133 & G & 09:25:02.2 & $-52$:03:47.1 & $198.16$ &  \\
shrds111 & 09:58:22.9 & $-56$:22:20.2 & G280.626$-$01.186 & C & 09:58:25.7 & $-56$:22:19.3 & $207.05$ &  \\
shrds113 & 10:02:28.7 & $-56$:04:34.6 & G280.903$-$00.522 & C & 10:02:53.9 & $-56$:00:34.4 & $441.52$ &  \\
shrds1005 & 09:59:14.5 & $-56$:54:33.8 & G280.989$-$01.527 & K & 09:59:00.6 & $-56$:51:49.2 & $254.18$ & CH87  \\
 & & & G281.047$-$01.541 & G & 09:59:17.1 & $-56$:54:35.6 & $116.87$ &  \\
 & & & G281.095$-$01.594 & G & 09:59:19.7 & $-56$:58:51.6 & $116.87$ &  \\
ch17 & 09:59:30.8 & $-57$:03:30.6 & G281.095$-$01.594 & G & 09:59:19.7 & $-56$:58:51.6 & $116.87$ &  \\
 & & & G281.175$-$01.645 & K & 09:59:34.0 & $-57$:04:13.3 & $189.51$ & CH87  \\
caswell1 & 09:59:32.0 & $-57$:04:05.2 & G281.095$-$01.594 & G & 09:59:19.7 & $-56$:58:51.6 & $116.87$ &  \\
 & & & G281.175$-$01.645 & K & 09:59:34.0 & $-57$:04:13.3 & $189.51$ & CH87  \\
shrds114 & 09:58:01.9 & $-57$:57:49.3 & G281.560$-$02.478 & C & 09:58:03.7 & $-57$:57:54.4 & $210.09$ &  \\
ch18 & 10:04:59.9 & $-56$:46:50.0 & G281.584$-$00.971 & K & 10:04:55.5 & $-56$:46:32.4 & $122.91$ & CH87  \\
 & & & G281.598$-$00.929 & Q & 10:05:11.6 & $-56$:44:57.3 & $82.61$ &  \\
shrds117 & 10:03:40.2 & $-57$:26:42.3 & G281.840$-$01.609 & C & 10:03:39.4 & $-57$:26:27.4 & $113.02$ &  \\
 & & & G281.865$-$01.649 & Q & 10:03:37.8 & $-57$:29:16.2 & $78.60$ &  \\
shrds1007 & 10:06:56.8 & $-57$:02:13.4 & G282.015$-$00.997 & G & 10:07:22.3 & $-57$:02:57.6 & $284.54$ &  \\
 & & & G282.027$-$01.182 & K & 10:06:38.5 & $-57$:12:25.2 & $496.08$ & CH87  \\
 & & & G282.372$-$01.044 & K & 10:09:18.8 & $-57$:17:42.1 & $1280.53$ & CH87  \\
ch19 & 10:06:38.4 & $-57$:12:20.2 & G282.027$-$01.182 & K & 10:06:38.5 & $-57$:12:25.2 & $496.08$ & CH87  \\
 & & & G282.372$-$01.044 & K & 10:09:18.8 & $-57$:17:42.1 & $1280.53$ & CH87  \\
shrds1232 & 10:11:15.3 & $-57$:44:02.4 & G282.788$-$01.321 & C & 10:10:39.3 & $-57$:45:40.2 & $117.84$ &  \\
 & & & G282.842$-$01.252 & C & 10:11:17.0 & $-57$:44:07.9 & $84.34$ &  \\
shrds132 & 10:16:15.1 & $-57$:10:21.0 & G283.098$-$00.400 & C & 10:16:26.0 & $-57$:10:37.6 & $106.64$ &  \\
 & & & G283.140$-$00.490 & C & 10:16:19.2 & $-57$:16:30.6 & $240.27$ &  \\
 & & & G283.157$-$00.334 & C & 10:17:03.9 & $-57$:09:18.8 & $172.57$ &  \\
shrds1013 & 10:19:41.0 & $-57$:51:29.6 & G283.729$-$00.774 & G & 10:18:48.2 & $-57$:50:17.1 & $203.39$ &  \\
 & & & G283.832$-$00.730 & G & 10:19:37.9 & $-57$:51:28.4 & $165.84$ &  \\
 & & & G283.895$-$00.956 & K & 10:19:05.8 & $-58$:04:52.0 & $755.56$ & CH87  \\
shrds1014 & 10:20:15.3 & $-58$:03:50.8 & G283.895$-$00.956 & K & 10:19:05.8 & $-58$:04:52.0 & $755.56$ & CH87  \\
 & & & G284.014$-$00.857 & G & 10:20:15.4 & $-58$:03:50.2 & $66.62$ &  \\
ch32 & 10:29:25.2 & $-57$:26:58.0 & G284.682+00.271 & G & 10:28:60.0 & $-57$:27:49.5 & $92.52$ &  \\
 & & & G284.712+00.317 & K & 10:29:22.1 & $-57$:26:23.1 & $201.20$ & CH87  \\
caswell2 & 10:29:29.1 & $-57$:26:47.6 & G284.682+00.271 & G & 10:28:60.0 & $-57$:27:49.5 & $92.52$ &  \\
 & & & G284.712+00.317 & K & 10:29:22.1 & $-57$:26:23.1 & $201.20$ & CH87  \\
shrds141 & 10:29:36.0 & $-57$:45:21.5 & G284.902+00.060 & C & 10:29:35.3 & $-57$:45:30.5 & $148.57$ &  \\
ch33 & 10:31:25.1 & $-58$:02:08.6 & G285.260$-$00.051 & K & 10:31:28.4 & $-58$:02:14.7 & $399.08$ & CH87  \\
shrds143 & 10:32:17.3 & $-58$:02:15.3 & G285.260$-$00.051 & K & 10:31:28.4 & $-58$:02:14.7 & $399.08$ & CH87  \\
 & & & G285.353+00.004 & C & 10:32:17.3 & $-58$:02:14.9 & $134.94$ &  \\
shrds1017 & 10:37:47.8 & $-58$:47:27.5 & G286.260$-$00.155 & K & 10:37:40.5 & $-58$:37:38.7 & $622.58$ & CH87  \\
 & & & G286.362$-$00.297 & G & 10:37:49.4 & $-58$:48:03.9 & $131.94$ &  \\
 & & & G286.376$-$00.257 & G & 10:38:04.0 & $-58$:46:24.6 & $86.59$ &  \\
 & & & G286.455$-$00.252 & G & 10:38:37.1 & $-58$:48:28.0 & $180.64$ &  \\
 & & & G286.468$-$00.358 & C & 10:38:18.3 & $-58$:54:24.4 & $314.11$ &  \\
shrds1018g & 10:38:04.0 & $-58$:46:25.9 & G286.260$-$00.155 & K & 10:37:40.5 & $-58$:37:38.7 & $622.58$ & CH87  \\
 & & & G286.362$-$00.297 & G & 10:37:49.4 & $-58$:48:03.9 & $131.94$ &  \\
 & & & G286.376$-$00.257 & G & 10:38:04.0 & $-58$:46:24.6 & $86.59$ &  \\
 & & & G286.455$-$00.252 & G & 10:38:37.1 & $-58$:48:28.0 & $180.64$ &  \\
 & & & G286.468$-$00.358 & C & 10:38:18.3 & $-58$:54:24.4 & $314.11$ &  \\
ch35 & 10:34:00.7 & $-59$:43:55.2 & G286.391$-$01.351 & K & 10:33:55.4 & $-59$:43:52.5 & $189.33$ & CH87  \\
ch36 & 10:33:36.1 & $-59$:51:08.7 & G286.412$-$01.468 & K & 10:33:36.1 & $-59$:50:32.3 & $89.31$ & CH87  \\
 & & & G286.439$-$01.496 & K & 10:33:40.5 & $-59$:52:49.0 & $89.31$ & CH87  \\
shrds158 & 10:39:21.0 & $-59$:39:57.1 & G286.951$-$00.955 & C & 10:39:20.2 & $-59$:39:46.0 & $71.10$ &  \\
 & & & G287.524$-$00.735 & K & 10:44:09.5 & $-59$:44:36.2 & $2283.37$ & CH87  \\
shrds159 & 10:42:12.9 & $-59$:08:37.7 & G287.025$-$00.321 & C & 10:42:14.3 & $-59$:08:33.4 & $135.41$ &  \\
 & & & G287.524$-$00.735 & K & 10:44:09.5 & $-59$:44:36.2 & $2283.37$ & CH87  \\
shrds162 & 10:44:40.2 & $-60$:48:06.2 & G288.074$-$01.642 & C & 10:44:39.1 & $-60$:48:06.5 & $99.09$ &  \\
shrds1020 & 10:47:42.6 & $-60$:25:03.6 & G288.230$-$01.153 & Q & 10:47:37.4 & $-60$:26:26.0 & $81.41$ &  \\
 & & & G288.233$-$01.118 & C & 10:47:46.5 & $-60$:24:39.5 & $95.40$ &  \\
shrds167 & 10:55:48.5 & $-59$:46:53.5 & G288.823$-$00.088 & C & 10:55:40.9 & $-59$:45:00.1 & $43.34$ &  \\
 & & & G288.851$-$00.108 & C & 10:55:48.7 & $-59$:46:49.9 & $95.85$ &  \\
 & & & G288.928$-$00.010 & C & 10:56:42.1 & $-59$:43:27.2 & $214.89$ &  \\
 & & & G288.929$-$00.118 & C & 10:56:20.3 & $-59$:49:23.0 & $102.60$ &  \\
shrds173 & 10:54:12.5 & $-60$:47:24.5 & G289.109$-$01.107 & C & 10:54:12.1 & $-60$:47:31.6 & $87.86$ &  \\
shrds1024 & 10:57:37.1 & $-60$:05:27.4 & G289.077$-$00.346 & K & 10:56:37.8 & $-60$:05:30.3 & $396.59$ & CH87  \\
 & & & G289.188$-$00.293 & G & 10:57:37.0 & $-60$:05:28.5 & $87.50$ &  \\
shrds177 & 10:54:05.8 & $-61$:08:04.8 & G289.249$-$01.423 & C & 10:54:06.2 & $-61$:08:15.0 & $81.98$ &  \\
shrds181 & 10:57:38.1 & $-60$:45:55.8 & G289.470$-$00.928 & C & 10:57:30.2 & $-60$:47:08.2 & $88.92$ &  \\
 & & & G289.476$-$00.899 & C & 10:57:38.7 & $-60$:45:46.0 & $112.41$ &  \\
shrds184 & 10:59:19.6 & $-60$:33:50.3 & G289.582$-$00.636 & C & 10:59:20.1 & $-60$:34:07.2 & $103.50$ &  \\
 & & & G289.612$-$00.611 & C & 10:59:38.6 & $-60$:33:28.9 & $217.89$ &  \\
shrds1026 & 10:58:43.0 & $-61$:10:38.8 & G289.769$-$01.220 & G & 10:58:43.1 & $-61$:10:37.3 & $59.93$ &  \\
 & & & G289.806$-$01.242 & K & 10:58:55.2 & $-61$:12:45.7 & $1088.92$ & CH87  \\
shrds187 & 10:57:34.3 & $-61$:35:32.6 & G289.720$-$01.597 & G & 10:57:01.0 & $-61$:29:52.6 & $173.52$ &  \\
 & & & G289.822$-$01.657 & C & 10:57:34.8 & $-61$:35:42.6 & $80.87$ &  \\
shrds1028 & 11:01:04.3 & $-60$:47:12.7 & G289.799$-$00.839 & G & 11:00:15.4 & $-60$:50:37.1 & $225.36$ &  \\
 & & & G289.874$-$00.752 & G & 11:01:06.8 & $-60$:47:41.3 & $151.30$ &  \\
 & & & G289.880$-$00.801 & K & 11:00:59.5 & $-60$:50:32.1 & $115.69$ & CH87  \\
 & & & G289.929$-$00.784 & Q & 11:01:24.9 & $-60$:50:49.2 & $98.34$ &  \\
shrds191 & 11:01:12.2 & $-60$:56:44.0 & G289.911$-$00.859 & Q & 11:01:01.6 & $-60$:54:29.4 & $67.53$ &  \\
 & & & G289.920$-$00.914 & Q & 11:00:54.5 & $-60$:57:42.5 & $51.52$ &  \\
 & & & G289.944$-$00.889 & C & 11:01:10.3 & $-60$:56:56.5 & $102.21$ &  \\
 & & & G289.966$-$00.962 & C & 11:01:05.4 & $-61$:01:27.8 & $173.48$ &  \\
 & & & G290.012$-$00.867 & C & 11:01:45.4 & $-60$:57:25.1 & $102.21$ &  \\
g290.012$-$ & 11:01:59.1 & $-60$:56:47.8 & G289.980$-$00.781 & C & 11:01:48.6 & $-60$:51:53.1 & $102.21$ &  \\
 & & & G290.012$-$00.867 & C & 11:01:45.4 & $-60$:57:25.1 & $102.21$ &  \\
shrds199 & 11:05:40.5 & $-62$:29:14.1 & G291.046$-$02.079 & C & 11:05:37.0 & $-62$:28:58.0 & $243.46$ &  \\
shrds1031g & 11:12:10.2 & $-60$:54:04.8 & G291.154$-$00.321 & G & 11:12:10.2 & $-60$:54:04.8 & $90.88$ &  \\
 & & & G291.186$-$00.274 & G & 11:12:33.5 & $-60$:52:12.0 & $90.88$ &  \\
 & & & G291.202$-$00.295 & G & 11:12:36.9 & $-60$:53:44.9 & $90.88$ &  \\
 & & & G291.214$-$00.246 & K & 11:12:51.5 & $-60$:51:14.8 & $245.72$ & CH87  \\
shrds1032 & 11:12:33.5 & $-60$:52:10.7 & G291.154$-$00.321 & G & 11:12:10.2 & $-60$:54:04.8 & $90.88$ &  \\
 & & & G291.186$-$00.274 & G & 11:12:33.5 & $-60$:52:12.0 & $90.88$ &  \\
 & & & G291.202$-$00.295 & G & 11:12:36.9 & $-60$:53:44.9 & $90.88$ &  \\
 & & & G291.214$-$00.246 & K & 11:12:51.5 & $-60$:51:14.8 & $245.72$ & CH87  \\
shrds1034 & 11:11:31.8 & $-61$:21:43.0 & G291.255$-$00.776 & G & 11:11:31.9 & $-61$:21:42.1 & $83.67$ &  \\
 & & & G291.281$-$00.726 & K & 11:11:53.5 & $-61$:19:28.2 & $446.49$ & CH87  \\
caswell3 & 11:11:53.4 & $-61$:19:00.5 & G291.255$-$00.776 & G & 11:11:31.9 & $-61$:21:42.1 & $83.67$ &  \\
 & & & G291.281$-$00.726 & K & 11:11:53.5 & $-61$:19:28.2 & $446.49$ & CH87  \\
ch52 & 11:11:57.1 & $-61$:18:51.9 & G291.255$-$00.776 & G & 11:11:31.9 & $-61$:21:42.1 & $83.67$ &  \\
 & & & G291.281$-$00.726 & K & 11:11:53.5 & $-61$:19:28.2 & $446.49$ & CH87  \\
 & & & G291.614$-$00.525 & K & 11:15:05.0 & $-61$:15:41.0 & $1125.19$ & CH87  \\
ch55 & 11:16:31.9 & $-61$:29:21.4 & G291.614$-$00.525 & K & 11:15:05.0 & $-61$:15:41.0 & $1125.19$ & CH87  \\
 & & & G291.863$-$00.682 & K & 11:16:33.1 & $-61$:29:50.0 & $155.35$ & CH87  \\
 & & & G291.947$-$00.910 & K & 11:16:31.4 & $-61$:44:25.4 & $920.14$ & CH87  \\
caswell4 & 11:16:33.7 & $-61$:29:57.3 & G291.614$-$00.525 & K & 11:15:05.0 & $-61$:15:41.0 & $1125.19$ & CH87  \\
 & & & G291.863$-$00.682 & K & 11:16:33.1 & $-61$:29:50.0 & $155.35$ & CH87  \\
 & & & G291.947$-$00.910 & K & 11:16:31.4 & $-61$:44:25.4 & $920.14$ & CH87  \\
ch57 & 11:24:48.3 & $-62$:13:30.3 & G292.917$-$00.973 & C & 11:24:04.8 & $-62$:08:01.7 & $212.57$ &  \\
 & & & G293.024$-$01.029 & K & 11:24:47.2 & $-62$:13:19.7 & $162.84$ & CH87  \\
 & & & G293.113$-$00.961 & C & 11:25:42.1 & $-62$:11:10.2 & $314.96$ &  \\
 & & & G293.232$-$00.659 & C & 11:27:29.6 & $-61$:56:18.9 & $1397.56$ &  \\
shrds207 & 11:25:41.9 & $-62$:11:13.4 & G293.024$-$01.029 & K & 11:24:47.2 & $-62$:13:19.7 & $162.84$ & CH87  \\
 & & & G293.113$-$00.961 & C & 11:25:42.1 & $-62$:11:10.2 & $314.96$ &  \\
 & & & G293.232$-$00.659 & C & 11:27:29.6 & $-61$:56:18.9 & $1397.56$ &  \\
shrds210 & 11:28:20.7 & $-62$:58:38.6 & G293.619$-$01.613 & G & 11:28:02.6 & $-62$:57:59.4 & $35.39$ &  \\
 & & & G293.620$-$01.638 & C & 11:27:58.8 & $-62$:59:27.3 & $274.30$ &  \\
 & & & G293.661$-$01.639 & G & 11:28:19.2 & $-63$:00:16.2 & $73.72$ &  \\
 & & & G293.683$-$01.590 & G & 11:28:38.5 & $-62$:57:52.6 & $38.56$ &  \\
shrds215 & 11:32:03.7 & $-62$:11:27.9 & G293.675$-$00.729 & C & 11:30:53.7 & $-62$:08:37.9 & $390.94$ &  \\
 & & & G293.824$-$00.761 & C & 11:32:01.7 & $-62$:13:10.6 & $64.68$ &  \\
 & & & G293.829$-$00.744 & C & 11:32:06.9 & $-62$:12:16.6 & $64.68$ &  \\
g293.936$-$ & 11:32:41.1 & $-62$:22:24.1 & G293.898$-$00.826 & C & 11:32:27.9 & $-62$:18:15.9 & $42.99$ &  \\
 & & & G293.936$-$00.873 & C & 11:32:39.4 & $-62$:21:37.2 & $75.25$ &  \\
 & & & G293.952$-$00.894 & C & 11:32:44.0 & $-62$:23:08.0 & $75.25$ &  \\
 & & & G293.967$-$00.984 & C & 11:32:37.5 & $-62$:28:30.3 & $120.38$ &  \\
 & & & G293.994$-$00.934 & C & 11:32:58.6 & $-62$:26:08.6 & $69.31$ &  \\
g293.994$-$ & 11:32:36.1 & $-62$:28:26.8 & G293.952$-$00.894 & C & 11:32:44.0 & $-62$:23:08.0 & $75.25$ &  \\
 & & & G293.967$-$00.984 & C & 11:32:37.5 & $-62$:28:30.3 & $120.38$ &  \\
 & & & G293.994$-$00.934 & C & 11:32:58.6 & $-62$:26:08.6 & $69.31$ &  \\
shrds219 & 11:32:37.2 & $-62$:28:02.7 & G293.952$-$00.894 & C & 11:32:44.0 & $-62$:23:08.0 & $75.25$ &  \\
 & & & G293.967$-$00.984 & C & 11:32:37.5 & $-62$:28:30.3 & $120.38$ &  \\
 & & & G293.994$-$00.934 & C & 11:32:58.6 & $-62$:26:08.6 & $69.31$ &  \\
shrds226 & 11:37:47.8 & $-62$:09:47.0 & G294.453$-$00.521 & C & 11:37:47.3 & $-62$:10:23.8 & $205.47$ &  \\
g295.748$-$ & 11:49:12.0 & $-62$:12:26.6 & G295.728$-$00.215 & K & 11:49:01.6 & $-62$:12:36.3 & $759.38$ & CH87  \\
 & & & G295.748$-$00.207 & C & 11:49:12.6 & $-62$:12:26.0 & $72.61$ &  \\
shrds242 & 12:02:14.6 & $-62$:35:53.4 & G297.312$-$00.295 & C & 12:02:14.8 & $-62$:37:41.5 & $212.36$ &  \\
shrds243 & 12:02:24.4 & $-62$:57:40.5 & G297.392$-$00.624 & C & 12:02:23.3 & $-62$:58:00.2 & $232.66$ &  \\
shrds244 & 12:04:28.4 & $-62$:21:16.9 & G297.455$-$00.010 & Q & 12:03:55.3 & $-62$:22:31.5 & $40.00$ &  \\
 & & & G297.519$-$00.031 & Q & 12:04:26.0 & $-62$:24:27.8 & $45.00$ &  \\
 & & & G297.570$-$00.036 & C & 12:04:51.5 & $-62$:25:17.8 & $302.36$ &  \\
shrds246 & 12:03:13.3 & $-63$:10:53.3 & G297.464$-$00.784 & Q & 12:02:44.7 & $-63$:08:15.0 & $45.62$ &  \\
 & & & G297.469$-$00.767 & Q & 12:02:49.1 & $-63$:07:17.3 & $52.25$ &  \\
 & & & G297.497$-$00.758 & K & 12:03:04.6 & $-63$:07:03.2 & $216.30$ & CH87  \\
 & & & G297.531$-$00.823 & C & 12:03:15.9 & $-63$:11:15.2 & $29.18$ &  \\
 & & & G297.535$-$00.832 & C & 12:03:17.1 & $-63$:11:52.1 & $26.43$ &  \\
 & & & G297.536$-$00.826 & C & 12:03:18.2 & $-63$:11:30.9 & $26.43$ &  \\
ch65 & 12:04:05.8 & $-63$:21:45.6 & G297.626$-$00.906 & C & 12:03:57.5 & $-63$:17:13.4 & $76.92$ &  \\
 & & & G297.651$-$00.973 & K & 12:04:04.1 & $-63$:21:27.5 & $171.37$ & CH87  \\
shrds249 & 12:08:26.2 & $-63$:11:13.3 & G298.108$-$00.740 & C & 12:08:26.0 & $-63$:12:26.5 & $182.35$ &  \\
 & & & G298.183$-$00.784 & K & 12:09:01.6 & $-63$:15:47.2 & $174.60$ & CH87  \\
caswell5 & 12:09:02.7 & $-63$:16:06.4 & G298.108$-$00.740 & C & 12:08:26.0 & $-63$:12:26.5 & $182.35$ &  \\
 & & & G298.183$-$00.784 & K & 12:09:01.6 & $-63$:15:47.2 & $174.60$ & CH87  \\
ch66 & 12:09:03.8 & $-63$:15:45.7 & G298.108$-$00.740 & C & 12:08:26.0 & $-63$:12:26.5 & $182.35$ &  \\
 & & & G298.183$-$00.784 & K & 12:09:01.6 & $-63$:15:47.2 & $174.60$ & CH87  \\
shrds1041 & 12:09:54.3 & $-62$:44:10.4 & G298.196$-$00.247 & G & 12:09:54.3 & $-62$:44:08.6 & $131.82$ &  \\
 & & & G298.205$-$00.142 & G & 12:10:07.8 & $-62$:38:00.0 & $153.57$ &  \\
 & & & G298.224$-$00.334 & K & 12:10:01.5 & $-62$:49:35.6 & $303.21$ & CH87  \\
 & & & G298.529$-$00.251 & K & 12:12:46.5 & $-62$:47:29.5 & $974.83$ & CH87  \\
ch67 & 12:10:03.8 & $-62$:49:27.3 & G298.196$-$00.247 & G & 12:09:54.3 & $-62$:44:08.6 & $131.82$ &  \\
 & & & G298.224$-$00.334 & K & 12:10:01.5 & $-62$:49:35.6 & $303.21$ & CH87  \\
 & & & G298.529$-$00.251 & K & 12:12:46.5 & $-62$:47:29.5 & $974.83$ & CH87  \\
g298.473+ & 12:12:50.0 & $-62$:25:54.3 & G298.473+00.104 & C & 12:12:45.3 & $-62$:25:54.8 & $166.06$ &  \\
shrds253 & 12:14:26.6 & $-62$:16:34.9 & G298.630+00.253 & C & 12:14:17.0 & $-62$:18:26.8 & $278.01$ &  \\
shrds256 & 12:15:17.5 & $-62$:23:36.4 & G298.630+00.253 & C & 12:14:17.0 & $-62$:18:26.8 & $278.01$ &  \\
 & & & G298.756+00.059 & Q & 12:15:07.3 & $-62$:31:03.3 & $204.69$ &  \\
 & & & G298.765+00.174 & C & 12:15:20.3 & $-62$:24:15.9 & $232.88$ &  \\
shrds258 & 12:15:50.6 & $-62$:27:21.3 & G298.756+00.059 & Q & 12:15:07.3 & $-62$:31:03.3 & $204.69$ &  \\
 & & & G298.765+00.174 & C & 12:15:20.3 & $-62$:24:15.9 & $232.88$ &  \\
 & & & G298.833+00.117 & C & 12:15:51.2 & $-62$:28:13.0 & $38.61$ &  \\
 & & & G298.834+00.127 & C & 12:15:52.4 & $-62$:27:38.6 & $38.61$ &  \\
 & & & G298.846+00.121 & C & 12:15:58.1 & $-62$:28:06.9 & $38.61$ &  \\
 & & & G298.878+00.192 & C & 12:16:19.6 & $-62$:24:10.9 & $58.09$ &  \\
shrds261 & 12:16:23.6 & $-62$:23:49.5 & G298.765+00.174 & C & 12:15:20.3 & $-62$:24:15.9 & $232.88$ &  \\
 & & & G298.878+00.192 & C & 12:16:19.6 & $-62$:24:10.9 & $58.09$ &  \\
 & & & G298.899+00.187 & C & 12:16:30.0 & $-62$:24:35.6 & $58.09$ &  \\
 & & & G298.903+00.218 & Q & 12:16:34.2 & $-62$:22:50.4 & $27.81$ &  \\
caswell6 & 12:19:56.6 & $-62$:55:29.8 & G299.290$-$00.289 & Q & 12:19:20.5 & $-62$:55:57.3 & $179.86$ &  \\
 & & & G299.326$-$00.311 & Q & 12:19:37.9 & $-62$:57:32.7 & $54.08$ &  \\
 & & & G299.336$-$00.329 & Q & 12:19:41.9 & $-62$:58:41.2 & $25.80$ &  \\
 & & & G299.349$-$00.267 & K & 12:19:52.7 & $-62$:55:06.6 & $140.00$ & CH87  \\
 & & & G299.399$-$00.235 & G & 12:20:20.9 & $-62$:53:33.5 & $102.39$ &  \\
ch71 & 12:20:00.7 & $-62$:54:38.8 & G299.290$-$00.289 & Q & 12:19:20.5 & $-62$:55:57.3 & $179.86$ &  \\
 & & & G299.326$-$00.311 & Q & 12:19:37.9 & $-62$:57:32.7 & $54.08$ &  \\
 & & & G299.336$-$00.329 & Q & 12:19:41.9 & $-62$:58:41.2 & $25.80$ &  \\
 & & & G299.349$-$00.267 & K & 12:19:52.7 & $-62$:55:06.6 & $140.00$ & CH87  \\
 & & & G299.399$-$00.235 & G & 12:20:20.9 & $-62$:53:33.5 & $102.39$ &  \\
shrds1046 & 12:20:26.4 & $-62$:53:54.9 & G299.349$-$00.267 & K & 12:19:52.7 & $-62$:55:06.6 & $140.00$ & CH87  \\
 & & & G299.399$-$00.235 & G & 12:20:20.9 & $-62$:53:33.5 & $102.39$ &  \\
shrds268 & 12:26:50.6 & $-62$:48:53.0 & G300.134$-$00.100 & C & 12:26:53.1 & $-62$:50:16.9 & $383.88$ &  \\
shrds271 & 12:28:48.0 & $-63$:02:09.7 & G300.084$-$00.485 & C & 12:26:07.1 & $-63$:12:59.6 & $1199.89$ &  \\
 & & & G300.344$-$00.219 & Q & 12:28:37.5 & $-62$:58:33.0 & $73.25$ &  \\
 & & & G300.369$-$00.288 & C & 12:28:47.5 & $-63$:02:45.8 & $163.06$ &  \\
 & & & G300.420$-$00.302 & C & 12:29:13.8 & $-63$:03:52.2 & $225.89$ &  \\
shrds273 & 12:29:26.8 & $-62$:55:04.6 & G300.424$-$00.153 & C & 12:29:22.6 & $-62$:55:00.5 & $166.65$ &  \\
 & & & G300.427$-$00.180 & C & 12:29:23.0 & $-62$:56:38.9 & $64.36$ &  \\
 & & & G300.455$-$00.190 & C & 12:29:37.3 & $-62$:57:23.4 & $63.12$ &  \\
 & & & G300.470$-$00.103 & Q & 12:29:49.0 & $-62$:52:15.5 & $79.25$ &  \\
 & & & G300.502$-$00.180 & K & 12:30:02.4 & $-62$:57:01.4 & $132.59$ & CH87  \\
ch73 & 12:34:47.2 & $-61$:38:48.7 & G300.965+01.162 & K & 12:34:51.8 & $-61$:38:43.9 & $111.33$ & CH87  \\
 & & & G300.983+01.117 & C & 12:34:59.4 & $-61$:41:31.6 & $88.54$ &  \\
caswell7 & 12:34:53.6 & $-61$:39:16.8 & G300.965+01.162 & K & 12:34:51.8 & $-61$:38:43.9 & $111.33$ & CH87  \\
 & & & G300.983+01.117 & C & 12:34:59.4 & $-61$:41:31.6 & $88.54$ &  \\
ch74 & 12:35:58.6 & $-61$:50:52.8 & G301.116+00.968 & K & 12:36:02.1 & $-61$:50:57.3 & $180.98$ & CH87  \\
caswell8 & 12:36:05.6 & $-61$:51:06.6 & G301.116+00.968 & K & 12:36:02.1 & $-61$:50:57.3 & $180.98$ & CH87  \\
shrds283 & 12:35:32.8 & $-63$:01:34.2 & G300.852$-$00.172 & C & 12:33:07.0 & $-62$:58:10.9 & $1171.26$ &  \\
 & & & G301.118$-$00.194 & C & 12:35:26.4 & $-63$:00:32.4 & $237.62$ &  \\
 & & & G301.138$-$00.227 & C & 12:35:35.9 & $-63$:02:34.7 & $54.79$ &  \\
shrds286 & 12:40:40.4 & $-62$:53:24.4 & G301.710$-$00.056 & C & 12:40:42.3 & $-62$:54:07.5 & $102.17$ &  \\
shrds1050g & 12:41:18.4 & $-61$:44:39.0 & G301.733+01.103 & G & 12:41:18.4 & $-61$:44:40.6 & $80.00$ &  \\
 & & & G301.996+00.947 & K & 12:43:29.2 & $-61$:54:33.5 & $1154.91$ & CH87  \\
shrds1051g & 12:41:55.0 & $-62$:04:01.7 & G301.817+00.784 & G & 12:41:55.0 & $-62$:04:00.2 & $127.31$ &  \\
 & & & G301.996+00.947 & K & 12:43:29.2 & $-61$:54:33.5 & $1154.91$ & CH87  \\
ch76 & 12:43:28.4 & $-62$:54:06.2 & G302.024$-$00.113 & Q & 12:43:26.7 & $-62$:58:13.6 & $88.01$ &  \\
 & & & G302.032$-$00.063 & K & 12:43:31.8 & $-62$:55:12.7 & $118.92$ & CH87  \\
 & & & G302.076+00.029 & C & 12:43:56.4 & $-62$:49:47.8 & $175.59$ &  \\
caswell9 & 12:43:34.9 & $-62$:55:16.0 & G302.024$-$00.113 & Q & 12:43:26.7 & $-62$:58:13.6 & $88.01$ &  \\
 & & & G302.032$-$00.063 & K & 12:43:31.8 & $-62$:55:12.7 & $118.92$ & CH87  \\
 & & & G302.076+00.029 & C & 12:43:56.4 & $-62$:49:47.8 & $175.59$ &  \\
shrds289 & 12:44:23.8 & $-63$:48:43.7 & G302.151$-$00.949 & C & 12:44:21.6 & $-63$:48:35.2 & $75.00$ &  \\
 & & & G302.155$-$00.917 & Q & 12:44:24.3 & $-63$:46:40.1 & $24.58$ &  \\
 & & & G302.209$-$00.912 & Q & 12:44:53.7 & $-63$:46:27.2 & $24.33$ &  \\
shrds291 & 12:45:23.2 & $-62$:51:49.1 & G302.160+00.064 & C & 12:44:41.5 & $-62$:47:48.5 & $154.40$ &  \\
 & & & G302.252+00.014 & C & 12:45:28.6 & $-62$:50:58.4 & $57.60$ &  \\
 & & & G302.270+00.073 & C & 12:45:38.8 & $-62$:47:28.7 & $326.82$ &  \\
shrds293 & 12:46:44.3 & $-62$:35:26.9 & G302.384+00.294 & Q & 12:46:40.8 & $-62$:34:21.4 & $31.52$ &  \\
 & & & G302.391+00.280 & C & 12:46:44.3 & $-62$:35:10.7 & $89.41$ &  \\
shrds294 & 12:47:02.2 & $-62$:58:35.3 & G302.436$-$00.106 & C & 12:47:04.3 & $-62$:58:23.8 & $119.22$ &  \\
 & & & G302.441$-$00.131 & Q & 12:47:06.8 & $-62$:59:53.2 & $34.25$ &  \\
 & & & G302.481$-$00.035 & C & 12:47:28.7 & $-62$:54:09.7 & $91.95$ &  \\
 & & & G302.582$-$00.083 & K & 12:48:21.6 & $-62$:57:08.0 & $470.39$ & CH87  \\
 & & & G302.631+00.030 & K & 12:48:48.1 & $-62$:50:24.6 & $860.88$ & CH87  \\
shrds295 & 12:47:32.9 & $-62$:54:12.3 & G302.436$-$00.106 & C & 12:47:04.3 & $-62$:58:23.8 & $119.22$ &  \\
 & & & G302.460$-$00.031 & Q & 12:47:17.6 & $-62$:53:55.5 & $42.80$ &  \\
 & & & G302.481$-$00.035 & C & 12:47:28.7 & $-62$:54:09.7 & $91.95$ &  \\
 & & & G302.582$-$00.083 & K & 12:48:21.6 & $-62$:57:08.0 & $470.39$ & CH87  \\
 & & & G302.631+00.030 & K & 12:48:48.1 & $-62$:50:24.6 & $860.88$ & CH87  \\
shrds296 & 12:47:34.0 & $-63$:38:00.7 & G302.453$-$00.740 & Q & 12:47:07.7 & $-63$:36:27.8 & $46.12$ &  \\
 & & & G302.503$-$00.762 & K & 12:47:34.5 & $-63$:37:49.4 & $251.74$ & CH87  \\
 & & & G302.614$-$00.756 & C & 12:48:34.5 & $-63$:37:33.1 & $847.45$ &  \\
shrds297 & 12:48:46.9 & $-63$:32:32.0 & G302.614$-$00.756 & C & 12:48:34.5 & $-63$:37:33.1 & $847.45$ &  \\
 & & & G302.636$-$00.672 & C & 12:48:46.9 & $-63$:32:29.3 & $159.77$ &  \\
 & & & G302.671$-$00.677 & Q & 12:49:05.7 & $-63$:32:48.9 & $38.05$ &  \\
ch79 & 12:50:21.8 & $-61$:33:55.7 & G302.805+01.287 & K & 12:50:22.3 & $-61$:35:02.6 & $197.30$ & CH87  \\
shrds299 & 12:50:20.7 & $-63$:43:03.0 & G302.614$-$00.756 & C & 12:48:34.5 & $-63$:37:33.1 & $847.45$ &  \\
 & & & G302.722$-$00.816 & C & 12:49:32.6 & $-63$:41:10.9 & $250.19$ &  \\
 & & & G302.816$-$00.844 & C & 12:50:23.5 & $-63$:42:52.5 & $82.94$ &  \\
shrds303 & 12:55:06.4 & $-63$:35:16.2 & G303.320$-$00.755 & Q & 12:54:55.9 & $-63$:37:26.2 & $41.81$ &  \\
 & & & G303.342$-$00.718 & C & 12:55:07.5 & $-63$:35:09.6 & $57.60$ &  \\
 & & & G303.445$-$00.745 & K & 12:56:03.3 & $-63$:36:40.1 & $435.56$ & CH87  \\
shrds305 & 12:55:33.4 & $-63$:50:06.4 & G303.384$-$00.965 & C & 12:55:32.3 & $-63$:49:57.5 & $81.00$ &  \\
shrds308 & 12:57:01.9 & $-63$:24:21.4 & G303.557$-$00.539 & C & 12:57:01.4 & $-63$:24:12.8 & $107.56$ &  \\
 & & & G303.593$-$00.631 & C & 12:57:21.8 & $-63$:29:41.4 & $142.57$ &  \\
shrds309 & 12:57:22.0 & $-63$:30:29.3 & G303.445$-$00.745 & K & 12:56:03.3 & $-63$:36:40.1 & $435.56$ & CH87  \\
 & & & G303.593$-$00.631 & C & 12:57:21.8 & $-63$:29:41.4 & $142.57$ &  \\
shrds326 & 13:00:39.9 & $-62$:53:16.5 & G303.893$-$00.055 & C & 12:59:52.9 & $-62$:54:37.4 & $554.10$ &  \\
 & & & G303.973$-$00.035 & C & 13:00:34.7 & $-62$:53:16.8 & $119.44$ &  \\
shrds329 & 13:00:57.8 & $-62$:33:48.4 & G303.896+00.407 & C & 12:59:46.6 & $-62$:26:54.9 & $419.30$ &  \\
 & & & G303.997+00.279 & C & 13:00:41.3 & $-62$:34:23.8 & $27.96$ &  \\
 & & & G304.018+00.277 & Q & 13:00:52.3 & $-62$:34:28.6 & $26.99$ &  \\
 & & & G304.034+00.290 & C & 13:01:00.4 & $-62$:33:39.6 & $109.06$ &  \\
 & & & G304.101+00.266 & Q & 13:01:35.8 & $-62$:34:57.7 & $22.80$ &  \\
shrds336 & 13:04:52.0 & $-62$:48:53.2 & G304.465$-$00.023 & C & 13:04:53.1 & $-62$:51:14.2 & $143.75$ &  \\
shrds338 & 13:05:31.3 & $-62$:29:57.5 & G304.557+00.329 & C & 13:05:31.3 & $-62$:29:53.5 & $71.13$ &  \\
shrds344 & 13:08:36.5 & $-62$:15:14.9 & G304.925+00.555 & C & 13:08:34.3 & $-62$:14:58.9 & $174.35$ &  \\
 & & & G305.056+00.372 & G & 13:09:48.4 & $-62$:25:23.5 & $558.38$ &  \\
ch86 & 13:12:35.2 & $-62$:35:34.4 & G305.233+00.110 & K & 13:11:30.4 & $-62$:40:18.5 & $678.69$ & CH87  \\
 & & & G305.272+00.164 & K & 13:11:48.5 & $-62$:36:52.6 & $90.88$ & CH87  \\
 & & & G305.352+00.222 & G & 13:12:27.6 & $-62$:33:00.3 & $55.11$ &  \\
 & & & G305.362+00.197 & K & 13:12:33.9 & $-62$:34:27.6 & $102.30$ & CH87  \\
 & & & G305.363+00.150 & K & 13:12:36.4 & $-62$:37:15.6 & $101.54$ & CH87  \\
 & & & G305.373+00.184 & G & 13:12:40.2 & $-62$:35:12.5 & $27.60$ &  \\
 & & & G305.503+00.214 & G & 13:13:46.3 & $-62$:32:43.0 & $770.46$ &  \\
shrds346 & 13:13:03.2 & $-63$:01:37.1 & G305.322$-$00.255 & K & 13:12:32.4 & $-63$:01:42.7 & $808.19$ & CH87  \\
 & & & G305.381$-$00.236 & Q & 13:13:02.7 & $-63$:00:16.9 & $45.30$ &  \\
 & & & G305.384$-$00.248 & C & 13:13:04.8 & $-63$:00:58.9 & $99.92$ &  \\
 & & & G305.439$-$00.232 & Q & 13:13:33.1 & $-62$:59:43.8 & $80.84$ &  \\
shrds350 & 13:16:12.5 & $-62$:26:49.6 & G305.789+00.138 & K & 13:16:18.4 & $-62$:35:43.6 & $321.19$ & CH87  \\
 & & & G305.789+00.280 & C & 13:16:11.3 & $-62$:27:15.4 & $128.28$ &  \\
ch93 & 13:21:21.0 & $-63$:02:10.0 & G306.268$-$00.333 & Q & 13:20:54.5 & $-63$:00:48.6 & $39.38$ &  \\
 & & & G306.286$-$00.344 & Q & 13:21:04.6 & $-63$:01:18.0 & $51.74$ &  \\
 & & & G306.321$-$00.358 & K & 13:21:23.9 & $-63$:01:55.2 & $104.14$ & CH87  \\
 & & & G306.323$-$00.332 & Q & 13:21:23.4 & $-63$:00:21.9 & $23.82$ &  \\
 & & & G306.345$-$00.326 & Q & 13:21:34.5 & $-62$:59:50.8 & $20.25$ &  \\
 & & & G306.361$-$00.291 & Q & 13:21:40.8 & $-62$:57:39.9 & $84.06$ &  \\
shrds364 & 13:32:31.8 & $-63$:06:06.8 & G307.559$-$00.585 & K & 13:32:30.1 & $-63$:05:14.0 & $119.68$ & CH87  \\
 & & & G307.571$-$00.620 & C & 13:32:39.2 & $-63$:07:09.2 & $72.79$ &  \\
 & & & G307.610$-$00.593 & C & 13:32:57.4 & $-63$:05:12.4 & $67.81$ &  \\
caswell10 & 13:32:32.1 & $-63$:05:33.7 & G307.559$-$00.585 & K & 13:32:30.1 & $-63$:05:14.0 & $119.68$ & CH87  \\
 & & & G307.571$-$00.620 & C & 13:32:39.2 & $-63$:07:09.2 & $72.79$ &  \\
 & & & G307.610$-$00.593 & C & 13:32:57.4 & $-63$:05:12.4 & $67.81$ &  \\
ch94 & 13:32:37.9 & $-63$:06:58.6 & G307.559$-$00.585 & K & 13:32:30.1 & $-63$:05:14.0 & $119.68$ & CH87  \\
 & & & G307.571$-$00.620 & C & 13:32:39.2 & $-63$:07:09.2 & $72.79$ &  \\
 & & & G307.610$-$00.593 & C & 13:32:57.4 & $-63$:05:12.4 & $67.81$ &  \\
shrds365 & 13:32:55.4 & $-63$:05:19.1 & G307.559$-$00.585 & K & 13:32:30.1 & $-63$:05:14.0 & $119.68$ & CH87  \\
 & & & G307.571$-$00.620 & C & 13:32:39.2 & $-63$:07:09.2 & $72.79$ &  \\
 & & & G307.610$-$00.593 & C & 13:32:57.4 & $-63$:05:12.4 & $67.81$ &  \\
shrds373 & 13:37:41.4 & $-64$:00:40.0 & G307.974$-$01.594 & C & 13:37:42.0 & $-64$:00:41.7 & $128.84$ &  \\
shrds374 & 13:32:36.9 & $-60$:27:27.8 & G308.002+02.020 & C & 13:32:41.8 & $-60$:26:40.9 & $140.66$ &  \\
g308.015$-$01 & 13:38:33.5 & $-64$:17:41.0 & G308.015$-$01.890 & C & 13:38:33.5 & $-64$:17:41.3 & $57.31$ &  \\
shrds377 & 13:37:20.1 & $-63$:28:21.1 & G307.972$-$01.102 & C & 13:36:53.7 & $-63$:31:38.8 & $64.86$ &  \\
 & & & G307.985$-$01.092 & Q & 13:36:59.6 & $-63$:30:55.9 & $20.24$ &  \\
 & & & G308.031$-$01.052 & C & 13:37:20.2 & $-63$:28:05.8 & $148.15$ &  \\
 & & & G308.033$-$01.053 & C & 13:37:21.4 & $-63$:28:07.6 & $52.02$ &  \\
g308.033$-$01 & 13:37:21.4 & $-63$:28:08.6 & G307.972$-$01.102 & C & 13:36:53.7 & $-63$:31:38.8 & $64.86$ &  \\
 & & & G307.985$-$01.092 & Q & 13:36:59.6 & $-63$:30:55.9 & $20.24$ &  \\
 & & & G308.031$-$01.052 & C & 13:37:20.2 & $-63$:28:05.8 & $148.15$ &  \\
 & & & G308.033$-$01.053 & C & 13:37:21.4 & $-63$:28:07.6 & $52.02$ &  \\
caswell11 & 13:36:46.9 & $-62$:49:38.9 & G308.056$-$00.397 & G & 13:36:32.7 & $-62$:49:07.5 & $34.19$ &  \\
 & & & G308.067$-$00.432 & Q & 13:36:41.1 & $-62$:51:03.9 & $25.79$ &  \\
 & & & G308.069$-$00.439 & Q & 13:36:42.8 & $-62$:51:29.7 & $19.86$ &  \\
 & & & G308.072$-$00.389 & G & 13:36:39.7 & $-62$:48:28.3 & $47.63$ &  \\
 & & & G308.079$-$00.406 & K & 13:36:44.9 & $-62$:49:23.3 & $131.95$ & CH87  \\
 & & & G308.096$-$00.326 & G & 13:36:46.4 & $-62$:44:31.9 & $324.14$ &  \\
ch96 & 13:36:54.1 & $-62$:50:50.6 & G308.056$-$00.397 & G & 13:36:32.7 & $-62$:49:07.5 & $34.19$ &  \\
 & & & G308.067$-$00.432 & Q & 13:36:41.1 & $-62$:51:03.9 & $25.79$ &  \\
 & & & G308.069$-$00.439 & Q & 13:36:42.8 & $-62$:51:29.7 & $19.86$ &  \\
 & & & G308.072$-$00.389 & G & 13:36:39.7 & $-62$:48:28.3 & $47.63$ &  \\
 & & & G308.079$-$00.406 & K & 13:36:44.9 & $-62$:49:23.3 & $131.95$ & CH87  \\
 & & & G308.096$-$00.326 & G & 13:36:46.4 & $-62$:44:31.9 & $324.14$ &  \\
shrds382 & 13:42:33.4 & $-62$:48:04.9 & G308.734$-$00.510 & C & 13:42:33.1 & $-62$:48:13.1 & $90.38$ &  \\
shrds1091 & 13:40:54.1 & $-61$:45:54.0 & G308.571+00.500 & G & 13:39:30.8 & $-61$:50:39.2 & $474.66$ &  \\
 & & & G308.713+00.646 & K & 13:40:27.7 & $-61$:40:27.2 & $477.49$ & CH87  \\
 & & & G308.747+00.547 & G & 13:40:54.1 & $-61$:45:53.7 & $100.40$ &  \\
shrds384 & 13:43:01.1 & $-62$:09:03.5 & G308.916+00.124 & C & 13:43:00.6 & $-62$:08:45.9 & $167.21$ &  \\
 & & & G309.075+00.172 & K & 13:44:15.6 & $-62$:04:03.4 & $489.31$ & CH87  \\
shrds385 & 13:45:19.4 & $-62$:25:23.8 & G309.151$-$00.215 & C & 13:45:35.0 & $-62$:25:50.7 & $191.04$ &  \\
shrds386 & 13:45:20.5 & $-62$:11:15.7 & G309.075+00.172 & K & 13:44:15.6 & $-62$:04:03.4 & $489.31$ & CH87  \\
 & & & G309.176$-$00.028 & C & 13:45:27.5 & $-62$:14:32.9 & $72.27$ &  \\
shrds387 & 13:46:21.4 & $-62$:23:07.3 & G309.151$-$00.215 & C & 13:45:35.0 & $-62$:25:50.7 & $191.04$ &  \\
 & & & G309.250$-$00.192 & C & 13:46:22.7 & $-62$:23:15.2 & $53.75$ &  \\
 & & & G309.272$-$00.224 & Q & 13:46:37.3 & $-62$:24:50.9 & $43.10$ &  \\
 & & & G309.297$-$00.409 & C & 13:47:10.6 & $-62$:35:23.0 & $608.45$ &  \\
shrds390 & 13:47:08.8 & $-62$:35:19.0 & G309.278$-$00.431 & Q & 13:47:03.3 & $-62$:36:52.7 & $45.46$ &  \\
 & & & G309.296$-$00.414 & C & 13:47:10.5 & $-62$:35:39.3 & $127.13$ &  \\
 & & & G309.297$-$00.409 & C & 13:47:10.6 & $-62$:35:23.0 & $608.45$ &  \\
shrds398 & 13:50:42.6 & $-61$:34:57.3 & G309.896+00.393 & K & 13:50:39.6 & $-61$:40:30.7 & $162.16$ & CH87  \\
 & & & G309.917+00.342 & K & 13:50:55.8 & $-61$:43:10.8 & $376.91$ & CH87  \\
 & & & G309.921+00.481 & C & 13:50:42.2 & $-61$:35:00.4 & $127.00$ &  \\
 & & & G310.004+00.502 & Q & 13:51:20.0 & $-61$:32:38.6 & $55.11$ &  \\
shrds403 & 13:54:48.3 & $-62$:10:06.8 & G310.168$-$00.132 & K & 13:53:56.8 & $-62$:07:18.6 & $244.78$ & CH87  \\
 & & & G310.182$-$00.247 & C & 13:54:17.9 & $-62$:13:46.8 & $121.90$ &  \\
 & & & G310.220$-$00.134 & Q & 13:54:22.9 & $-62$:06:39.0 & $38.22$ &  \\
 & & & G310.260$-$00.199 & C & 13:54:51.0 & $-62$:09:53.4 & $150.76$ &  \\
shrds407 & 13:57:01.8 & $-62$:07:11.2 & G310.519$-$00.220 & C & 13:57:02.5 & $-62$:07:15.5 & $95.54$ &  \\
 & & & G310.560$-$00.194 & C & 13:57:19.4 & $-62$:05:06.6 & $40.11$ &  \\
shrds409 & 13:58:37.3 & $-62$:17:39.7 & G310.578$-$00.456 & Q & 13:58:02.6 & $-62$:20:02.2 & $38.73$ &  \\
 & & & G310.630$-$00.421 & C & 13:58:24.0 & $-62$:17:14.3 & $111.39$ &  \\
 & & & G310.672$-$00.450 & C & 13:58:48.9 & $-62$:18:17.7 & $107.06$ &  \\
shrds411 & 13:58:39.3 & $-62$:09:54.1 & G310.688$-$00.314 & C & 13:58:38.8 & $-62$:10:09.3 & $59.66$ &  \\
 & & & G310.755$-$00.354 & Q & 13:59:17.4 & $-62$:11:25.4 & $48.38$ &  \\
shrds1095g & 13:59:29.3 & $-62$:14:03.2 & G310.755$-$00.354 & Q & 13:59:17.4 & $-62$:11:25.4 & $48.38$ &  \\
 & & & G310.766$-$00.403 & G & 13:59:29.3 & $-62$:14:04.7 & $39.64$ &  \\
 & & & G310.768$-$00.393 & Q & 13:59:29.0 & $-62$:13:28.5 & $18.35$ &  \\
 & & & G310.808$-$00.399 & K & 13:59:49.8 & $-62$:13:13.0 & $266.89$ & CH87  \\
shrds412 & 13:59:35.8 & $-61$:48:07.0 & G310.887+00.009 & C & 13:59:34.2 & $-61$:48:18.4 & $89.85$ &  \\
shrds1096 & 14:00:32.4 & $-62$:10:14.9 & G310.808$-$00.399 & K & 13:59:49.8 & $-62$:13:13.0 & $266.89$ & CH87  \\
 & & & G310.901$-$00.373 & G & 14:00:32.4 & $-62$:10:13.8 & $101.31$ &  \\
 & & & G310.961$-$00.384 & Q & 14:01:03.6 & $-62$:09:55.6 & $25.39$ &  \\
shrds413 & 14:01:20.0 & $-62$:08:02.0 & G310.961$-$00.384 & Q & 14:01:03.6 & $-62$:09:55.6 & $25.39$ &  \\
 & & & G311.003$-$00.355 & C & 14:01:20.4 & $-62$:07:32.7 & $122.03$ &  \\
 & & & G311.138$-$00.278 & K & 14:02:16.5 & $-62$:00:56.8 & $355.92$ & CH87  \\
shrds415 & 14:00:13.7 & $-61$:34:24.2 & G311.015+00.210 & C & 14:00:10.1 & $-61$:34:40.6 & $69.81$ &  \\
shrds418 & 14:02:05.6 & $-61$:59:04.1 & G311.137$-$00.235 & C & 14:02:09.9 & $-61$:58:26.3 & $38.58$ &  \\
 & & & G311.138$-$00.278 & K & 14:02:16.5 & $-62$:00:56.8 & $355.92$ & CH87  \\
shrds425 & 14:02:35.4 & $-61$:05:42.5 & G311.386+00.649 & Q & 14:02:10.3 & $-61$:03:19.6 & $42.78$ &  \\
 & & & G311.396+00.583 & C & 14:02:24.0 & $-61$:07:01.2 & $641.84$ &  \\
 & & & G311.425+00.598 & C & 14:02:35.8 & $-61$:05:39.9 & $62.23$ &  \\
shrds428 & 14:04:33.4 & $-61$:23:51.7 & G311.540+00.319 & Q & 14:04:09.1 & $-61$:19:51.2 & $57.65$ &  \\
 & & & G311.563+00.239 & C & 14:04:31.4 & $-61$:24:06.7 & $27.86$ &  \\
 & & & G311.575+00.239 & C & 14:04:37.2 & $-61$:23:54.0 & $28.95$ &  \\
 & & & G311.598+00.272 & Q & 14:04:43.6 & $-61$:21:35.5 & $21.67$ &  \\
 & & & G311.621+00.295 & K & 14:04:51.4 & $-61$:19:52.5 & $32.39$ & CH87  \\
 & & & G311.629+00.277 & Q & 14:04:57.8 & $-61$:20:47.1 & $15.65$ &  \\
 & & & G311.629+00.289 & K & 14:04:56.0 & $-61$:20:04.7 & $29.94$ & CH87  \\
shrds1101 & 14:06:41.8 & $-62$:11:26.0 & G311.551$-$00.584 & G & 14:06:23.5 & $-62$:11:38.7 & $82.97$ &  \\
 & & & G311.581$-$00.593 & G & 14:06:39.7 & $-62$:11:39.2 & $67.83$ &  \\
 & & & G311.597$-$00.635 & Q & 14:06:53.7 & $-62$:13:46.4 & $31.63$ &  \\
 & & & G311.606$-$00.638 & Q & 14:06:58.7 & $-62$:13:49.6 & $24.47$ &  \\
 & & & G311.639$-$00.627 & K & 14:07:13.4 & $-62$:12:38.3 & $262.25$ & CH87  \\
caswell12 & 14:04:54.0 & $-61$:19:53.5 & G311.575+00.239 & C & 14:04:37.2 & $-61$:23:54.0 & $28.95$ &  \\
 & & & G311.598+00.272 & Q & 14:04:43.6 & $-61$:21:35.5 & $21.67$ &  \\
 & & & G311.621+00.295 & K & 14:04:51.4 & $-61$:19:52.5 & $32.39$ & CH87  \\
 & & & G311.629+00.277 & Q & 14:04:57.8 & $-61$:20:47.1 & $15.65$ &  \\
 & & & G311.629+00.289 & K & 14:04:56.0 & $-61$:20:04.7 & $29.94$ & CH87  \\
 & & & G311.638+00.301 & Q & 14:04:58.7 & $-61$:19:15.7 & $31.72$ &  \\
ch110 & 14:04:57.9 & $-61$:21:15.4 & G311.563+00.239 & C & 14:04:31.4 & $-61$:24:06.7 & $27.86$ &  \\
 & & & G311.575+00.239 & C & 14:04:37.2 & $-61$:23:54.0 & $28.95$ &  \\
 & & & G311.598+00.272 & Q & 14:04:43.6 & $-61$:21:35.5 & $21.67$ &  \\
 & & & G311.621+00.295 & K & 14:04:51.4 & $-61$:19:52.5 & $32.39$ & CH87  \\
 & & & G311.629+00.277 & Q & 14:04:57.8 & $-61$:20:47.1 & $15.65$ &  \\
 & & & G311.629+00.289 & K & 14:04:56.0 & $-61$:20:04.7 & $29.94$ & CH87  \\
 & & & G311.638+00.301 & Q & 14:04:58.7 & $-61$:19:15.7 & $31.72$ &  \\
 & & & G311.645+00.207 & Q & 14:05:15.3 & $-61$:24:33.2 & $20.85$ &  \\
shrds432 & 14:07:05.5 & $-61$:58:08.0 & G311.644$-$00.379 & C & 14:06:39.2 & $-61$:58:18.4 & $35.54$ &  \\
 & & & G311.667$-$00.409 & C & 14:06:54.8 & $-61$:59:35.2 & $133.09$ &  \\
 & & & G311.673$-$00.323 & Q & 14:06:45.1 & $-61$:54:32.0 & $26.38$ &  \\
 & & & G311.696$-$00.392 & C & 14:07:06.6 & $-61$:58:09.1 & $22.15$ &  \\
shrds1103 & 14:07:50.4 & $-61$:49:56.9 & G311.809$-$00.309 & G & 14:07:49.4 & $-61$:51:23.4 & $253.20$ &  \\
 & & & G311.841$-$00.219 & K & 14:07:51.5 & $-61$:45:38.7 & $58.85$ & CH87  \\
 & & & G311.843$-$00.261 & Q & 14:07:58.8 & $-61$:48:02.3 & $27.33$ &  \\
 & & & G311.866$-$00.238 & K & 14:08:06.5 & $-61$:46:18.4 & $61.57$ & CH87  \\
 & & & G311.908$-$00.279 & G & 14:08:33.0 & $-61$:47:56.3 & $191.98$ &  \\
shrds435 & 14:07:02.3 & $-61$:30:29.1 & G311.747+00.164 & C & 14:06:10.6 & $-61$:25:19.2 & $275.81$ &  \\
 & & & G311.758+00.087 & Q & 14:06:26.9 & $-61$:29:31.6 & $39.51$ &  \\
 & & & G311.794+00.084 & Q & 14:06:44.6 & $-61$:29:04.5 & $36.03$ &  \\
 & & & G311.822+00.044 & C & 14:07:04.0 & $-61$:30:55.1 & $140.09$ &  \\
 & & & G311.893+00.086 & K & 14:07:31.9 & $-61$:27:13.9 & $186.05$ & CH87  \\
ch113 & 14:07:30.5 & $-61$:26:27.7 & G311.822+00.044 & C & 14:07:04.0 & $-61$:30:55.1 & $140.09$ &  \\
 & & & G311.893+00.086 & K & 14:07:31.9 & $-61$:27:13.9 & $186.05$ & CH87  \\
 & & & G311.919+00.204 & K & 14:07:27.2 & $-61$:20:00.3 & $156.17$ & CH87  \\
 & & & G311.991+00.219 & K & 14:07:59.5 & $-61$:17:53.4 & $363.99$ & CH87  \\
ch114 & 14:07:25.2 & $-61$:18:34.1 & G311.919+00.204 & K & 14:07:27.2 & $-61$:20:00.3 & $156.17$ & CH87  \\
 & & & G311.991+00.219 & K & 14:07:59.5 & $-61$:17:53.4 & $363.99$ & CH87  \\
shrds437 & 14:08:29.6 & $-61$:37:25.4 & G311.932$-$00.107 & Q & 14:08:19.1 & $-61$:37:38.3 & $17.61$ &  \\
 & & & G311.949$-$00.114 & C & 14:08:28.3 & $-61$:37:44.0 & $50.38$ &  \\
 & & & G311.963$-$00.037 & C & 14:08:23.7 & $-61$:33:04.2 & $212.94$ &  \\
 & & & G312.005$-$00.154 & Q & 14:09:01.4 & $-61$:39:03.9 & $30.42$ &  \\
shrds439 & 14:08:33.1 & $-61$:34:05.6 & G311.932$-$00.107 & Q & 14:08:19.1 & $-61$:37:38.3 & $17.61$ &  \\
 & & & G311.949$-$00.114 & C & 14:08:28.3 & $-61$:37:44.0 & $50.38$ &  \\
 & & & G311.963$-$00.037 & C & 14:08:23.7 & $-61$:33:04.2 & $212.94$ &  \\
shrds440 & 14:08:29.3 & $-61$:24:26.5 & G311.991+00.219 & K & 14:07:59.5 & $-61$:17:53.4 & $363.99$ & CH87  \\
 & & & G312.091+00.069 & C & 14:09:09.4 & $-61$:24:43.4 & $97.69$ &  \\
ch115 & 14:08:43.4 & $-61$:10:21.6 & G311.991+00.219 & K & 14:07:59.5 & $-61$:17:53.4 & $363.99$ & CH87  \\
 & & & G312.100+00.283 & Q & 14:08:42.2 & $-61$:12:18.6 & $16.78$ &  \\
 & & & G312.110+00.311 & K & 14:08:42.9 & $-61$:10:33.8 & $105.06$ & CH87  \\
shrds445 & 14:12:00.7 & $-61$:49:07.2 & G312.296$-$00.427 & C & 14:12:03.7 & $-61$:49:25.4 & $105.34$ &  \\
 & & & G312.307$-$00.364 & Q & 14:11:59.1 & $-61$:45:36.8 & $23.47$ &  \\
 & & & G312.317$-$00.429 & Q & 14:12:14.1 & $-61$:49:07.8 & $36.36$ &  \\
 & & & G312.325$-$00.357 & C & 14:12:06.7 & $-61$:44:52.1 & $102.00$ &  \\
 & & & G312.367$-$00.395 & C & 14:12:33.0 & $-61$:46:18.0 & $48.26$ &  \\
shrds450 & 14:11:38.1 & $-61$:26:02.2 & G312.388$-$00.057 & C & 14:11:50.7 & $-61$:26:36.5 & $86.37$ &  \\
shrds454 & 14:13:30.1 & $-61$:35:53.9 & G312.527$-$00.266 & C & 14:13:29.6 & $-61$:35:55.2 & $46.03$ &  \\
 & & & G312.548$-$00.280 & C & 14:13:42.0 & $-61$:36:22.0 & $42.89$ &  \\
shrds456 & 14:12:40.8 & $-61$:06:35.1 & G312.591+00.210 & C & 14:12:46.1 & $-61$:07:36.0 & $129.29$ &  \\
 & & & G312.620+00.280 & Q & 14:12:49.1 & $-61$:03:04.9 & $34.68$ &  \\
shrds458 & 14:13:14.4 & $-61$:16:52.6 & G312.536+00.064 & C & 14:12:42.6 & $-61$:16:58.4 & $46.95$ &  \\
 & & & G312.598+00.048 & C & 14:13:14.4 & $-61$:16:42.3 & $47.17$ &  \\
 & & & G312.675+00.048 & C & 14:13:51.0 & $-61$:15:16.6 & $109.78$ &  \\
shrds459 & 14:18:44.6 & $-63$:07:07.0 & G312.614$-$01.902 & C & 14:18:44.4 & $-63$:07:13.6 & $66.50$ &  \\
shrds462 & 14:14:10.1 & $-61$:16:07.4 & G312.675+00.048 & C & 14:13:51.0 & $-61$:15:16.6 & $109.78$ &  \\
 & & & G312.706+00.012 & C & 14:14:11.3 & $-61$:16:43.5 & $95.87$ &  \\
 & & & G312.764+00.067 & C & 14:14:30.2 & $-61$:12:31.1 & $80.22$ &  \\
shrds463 & 14:14:33.7 & $-61$:12:39.3 & G312.675+00.048 & C & 14:13:51.0 & $-61$:15:16.6 & $109.78$ &  \\
 & & & G312.706+00.012 & C & 14:14:11.3 & $-61$:16:43.5 & $95.87$ &  \\
 & & & G312.764+00.067 & C & 14:14:30.2 & $-61$:12:31.1 & $80.22$ &  \\
shrds465 & 14:17:20.5 & $-61$:37:53.4 & G312.877$-$00.460 & Q & 14:16:48.5 & $-61$:40:19.5 & $55.90$ &  \\
 & & & G312.888$-$00.447 & C & 14:16:51.6 & $-61$:39:21.8 & $116.14$ &  \\
 & & & G312.979$-$00.432 & C & 14:17:32.7 & $-61$:36:45.0 & $201.29$ &  \\
shrds468 & 14:20:18.3 & $-61$:31:40.3 & G313.315$-$00.462 & C & 14:20:17.4 & $-61$:31:45.0 & $87.48$ &  \\
shrds479 & 14:23:52.6 & $-61$:08:18.0 & G313.851$-$00.243 & C & 14:23:51.8 & $-61$:08:22.1 & $70.58$ &  \\
shrds1111 & 14:25:16.8 & $-60$:21:17.9 & G314.220+00.477 & G & 14:24:37.5 & $-60$:20:10.0 & $315.97$ &  \\
 & & & G314.239+00.428 & K & 14:24:54.4 & $-60$:22:28.4 & $130.62$ & CH87  \\
 & & & G314.257+00.379 & Q & 14:25:11.0 & $-60$:24:50.8 & $21.12$ &  \\
 & & & G314.288+00.431 & G & 14:25:16.7 & $-60$:21:16.4 & $20.41$ &  \\
 & & & G314.303+00.416 & G & 14:25:26.1 & $-60$:21:48.2 & $13.19$ &  \\
 & & & G314.323+00.384 & C & 14:25:40.2 & $-60$:23:11.5 & $74.62$ &  \\
g314.593$-$01 & 14:33:18.0 & $-61$:58:09.8 & G314.593$-$01.427 & C & 14:33:18.0 & $-61$:58:10.1 & $57.33$ &  \\
ch121 & 14:35:07.1 & $-60$:37:41.7 & G315.286$-$00.270 & Q & 14:34:54.8 & $-60$:38:08.0 & $19.89$ &  \\
 & & & G315.296$-$00.235 & Q & 14:34:52.5 & $-60$:35:56.3 & $33.22$ &  \\
 & & & G315.297$-$00.319 & Q & 14:35:08.9 & $-60$:40:33.2 & $29.56$ &  \\
 & & & G315.306$-$00.182 & Q & 14:34:47.1 & $-60$:32:48.1 & $81.84$ &  \\
 & & & G315.312$-$00.272 & K & 14:35:06.7 & $-60$:37:35.6 & $115.43$ & CH87  \\
 & & & G315.327$-$00.230 & Q & 14:35:05.6 & $-60$:34:57.1 & $14.51$ &  \\
 & & & G315.328$-$00.225 & Q & 14:35:05.1 & $-60$:34:39.3 & $16.44$ &  \\
 & & & G315.330$-$00.221 & G & 14:35:05.2 & $-60$:34:22.6 & $77.36$ &  \\
 & & & G315.341$-$00.320 & G & 14:35:29.1 & $-60$:39:36.9 & $120.50$ &  \\
 & & & G315.363$-$00.235 & G & 14:35:22.6 & $-60$:34:21.5 & $77.50$ &  \\
 & & & G315.378$-$00.186 & G & 14:35:20.2 & $-60$:31:20.7 & $167.10$ &  \\
shrds501 & 14:41:42.4 & $-60$:32:11.7 & G316.093$-$00.511 & C & 14:41:43.2 & $-60$:31:59.4 & $64.98$ &  \\
 & & & G316.141$-$00.506 & K & 14:42:03.5 & $-60$:30:31.8 & $112.14$ & CH87  \\
ch122 & 14:42:07.4 & $-60$:29:24.8 & G316.093$-$00.511 & C & 14:41:43.2 & $-60$:31:59.4 & $64.98$ &  \\
 & & & G316.141$-$00.506 & K & 14:42:03.5 & $-60$:30:31.8 & $112.14$ & CH87  \\
ch124 & 14:45:21.0 & $-59$:48:14.3 & G316.796$-$00.056 & K & 14:45:19.6 & $-59$:49:33.2 & $311.80$ & CH87  \\
 & & & G316.875+00.041 & G & 14:45:34.0 & $-59$:42:16.0 & $238.42$ &  \\
 & & & G317.030+00.028 & K & 14:46:43.4 & $-59$:39:01.3 & $1463.64$ & CH87  \\
shrds512 & 14:50:17.6 & $-60$:30:33.7 & G317.059$-$00.937 & C & 14:50:18.0 & $-60$:30:23.5 & $83.48$ &  \\
shrds513 & 14:52:25.7 & $-60$:29:41.6 & G317.294$-$01.041 & C & 14:52:22.9 & $-60$:29:40.3 & $84.43$ &  \\
shrds1122 & 14:49:09.7 & $-59$:25:07.2 & G317.030+00.028 & K & 14:46:43.4 & $-59$:39:01.3 & $1463.64$ & CH87  \\
 & & & G317.405+00.091 & G & 14:49:10.3 & $-59$:25:49.4 & $154.34$ &  \\
shrds518 & 14:51:44.4 & $-59$:57:50.6 & G317.426$-$00.561 & C & 14:51:36.4 & $-60$:00:24.1 & $71.65$ &  \\
 & & & G317.431$-$00.522 & C & 14:51:30.2 & $-59$:58:09.6 & $63.03$ &  \\
 & & & G317.458$-$00.533 & C & 14:51:44.2 & $-59$:58:02.5 & $33.15$ &  \\
 & & & G317.466$-$00.524 & C & 14:51:45.6 & $-59$:57:20.1 & $33.15$ &  \\
 & & & G317.475$-$00.586 & Q & 14:52:02.7 & $-60$:00:24.0 & $19.40$ &  \\
 & & & G317.487$-$00.564 & Q & 14:52:03.2 & $-59$:58:54.9 & $21.81$ &  \\
 & & & G317.498$-$00.576 & Q & 14:52:10.4 & $-59$:59:14.9 & $55.76$ &  \\
 & & & G317.517$-$00.629 & C & 14:52:30.0 & $-60$:01:36.0 & $190.27$ &  \\
 & & & G317.528$-$00.535 & Q & 14:52:14.6 & $-59$:56:16.7 & $14.92$ &  \\
shrds521 & 14:51:26.3 & $-59$:40:04.6 & G317.570$-$00.257 & C & 14:51:33.2 & $-59$:40:12.7 & $419.51$ &  \\
 & & & G317.577$-$00.169 & C & 14:51:17.7 & $-59$:35:18.2 & $103.19$ &  \\
shrds528 & 14:53:07.3 & $-59$:20:54.5 & G317.818$-$00.059 & Q & 14:52:36.2 & $-59$:22:54.4 & $20.16$ &  \\
 & & & G317.829$-$00.015 & Q & 14:52:31.7 & $-59$:20:17.2 & $41.79$ &  \\
 & & & G317.870$-$00.008 & C & 14:52:47.3 & $-59$:18:46.9 & $132.43$ &  \\
 & & & G317.881$-$00.068 & Q & 14:53:04.7 & $-59$:21:43.0 & $21.92$ &  \\
 & & & G317.889$-$00.065 & C & 14:53:07.5 & $-59$:21:20.6 & $17.29$ &  \\
 & & & G317.891$-$00.052 & C & 14:53:05.5 & $-59$:20:33.8 & $32.77$ &  \\
 & & & G317.891$-$00.059 & C & 14:53:07.0 & $-59$:20:58.0 & $23.82$ &  \\
ch129 & 14:55:43.5 & $-59$:37:48.1 & G318.059$-$00.450 & K & 14:55:41.9 & $-59$:37:16.5 & $100.16$ & CH87  \\
caswell13 & 14:55:41.9 & $-59$:37:01.6 & G318.059$-$00.450 & K & 14:55:41.9 & $-59$:37:16.5 & $100.16$ & CH87  \\
shrds1126 & 14:57:29.3 & $-59$:40:43.0 & G318.141$-$00.697 & G & 14:57:10.8 & $-59$:48:09.7 & $522.52$ &  \\
 & & & G318.233$-$00.605 & G & 14:57:29.2 & $-59$:40:42.7 & $131.16$ &  \\
shrds532 & 14:57:33.3 & $-59$:26:20.8 & G318.351$-$00.398 & C & 14:57:33.0 & $-59$:26:24.6 & $65.34$ &  \\
shrds535 & 14:59:30.0 & $-59$:06:41.4 & G318.726$-$00.222 & C & 14:59:30.0 & $-59$:06:33.3 & $71.19$ &  \\
shrds536 & 14:59:35.1 & $-59$:01:18.2 & G318.726$-$00.222 & C & 14:59:30.0 & $-59$:06:33.3 & $71.19$ &  \\
 & & & G318.774$-$00.150 & C & 14:59:33.8 & $-59$:01:22.1 & $61.84$ &  \\
ch131 & 15:00:36.9 & $-58$:59:07.9 & G318.915$-$00.165 & K & 15:00:35.0 & $-58$:58:10.3 & $96.33$ & CH87  \\
 & & & G318.948$-$00.199 & Q & 15:00:55.9 & $-58$:58:58.5 & $65.50$ &  \\
shrds1129 & 15:03:02.3 & $-58$:55:23.3 & G319.188$-$00.329 & G & 15:03:03.2 & $-58$:58:57.0 & $463.22$ &  \\
 & & & G319.293$-$00.426 & G & 15:04:07.8 & $-59$:00:56.9 & $410.57$ &  \\
shrds1131 & 15:03:41.5 & $-58$:35:05.1 & G319.397$-$00.006 & K & 15:03:15.5 & $-58$:35:55.5 & $128.64$ & CH87  \\
 & & & G319.453$-$00.022 & G & 15:03:41.6 & $-58$:35:06.7 & $80.54$ &  \\
ch134 & 15:03:34.2 & $-57$:41:19.8 & G319.884+00.793 & K & 15:03:32.9 & $-57$:39:46.9 & $202.83$ & CH87  \\
 & & & G320.016+00.742 & C & 15:04:36.0 & $-57$:38:38.8 & $296.75$ &  \\
shrds1133g & 15:09:36.8 & $-58$:45:21.9 & G320.037$-$00.551 & G & 15:09:36.8 & $-58$:45:21.8 & $63.84$ &  \\
 & & & G320.104$-$00.511 & K & 15:09:54.0 & $-58$:41:14.1 & $259.79$ & CH87  \\
shrds1134g & 15:09:38.0 & $-58$:35:32.3 & G320.104$-$00.511 & K & 15:09:54.0 & $-58$:41:14.1 & $259.79$ & CH87  \\
 & & & G320.116$-$00.429 & G & 15:09:39.6 & $-58$:36:36.3 & $136.30$ &  \\
 & & & G320.147$-$00.411 & G & 15:09:47.9 & $-58$:34:46.6 & $60.22$ &  \\
ch136 & 15:05:21.2 & $-57$:32:38.2 & G320.016+00.742 & C & 15:04:36.0 & $-57$:38:38.8 & $296.75$ &  \\
 & & & G320.098+00.744 & Q & 15:05:07.6 & $-57$:36:07.3 & $50.66$ &  \\
 & & & G320.163+00.797 & K & 15:05:21.3 & $-57$:31:26.9 & $186.23$ & CH87  \\
shrds1137 & 15:05:22.3 & $-57$:26:33.5 & G320.148+00.873 & Q & 15:04:59.2 & $-57$:27:53.1 & $70.60$ &  \\
 & & & G320.163+00.797 & K & 15:05:21.3 & $-57$:31:26.9 & $186.23$ & CH87  \\
 & & & G320.205+00.867 & G & 15:05:22.2 & $-57$:26:32.4 & $64.41$ &  \\
 & & & G320.236+00.938 & C & 15:05:18.7 & $-57$:21:54.2 & $233.29$ &  \\
shrds1139 & 15:09:30.1 & $-58$:19:44.5 & G320.190$-$00.172 & G & 15:09:09.7 & $-58$:21:05.1 & $171.42$ &  \\
 & & & G320.236$-$00.099 & G & 15:09:11.0 & $-58$:15:53.6 & $168.90$ &  \\
 & & & G320.240$-$00.176 & G & 15:09:30.2 & $-58$:19:45.8 & $83.56$ &  \\
 & & & G320.278$-$00.157 & G & 15:09:41.0 & $-58$:17:39.1 & $151.48$ &  \\
 & & & G320.278$-$00.217 & G & 15:09:54.8 & $-58$:20:45.6 & $106.02$ &  \\
 & & & G320.311$-$00.176 & K & 15:09:58.4 & $-58$:17:38.1 & $91.96$ & CH87  \\
shrds1140 & 15:09:09.2 & $-58$:14:53.4 & G320.190$-$00.172 & G & 15:09:09.7 & $-58$:21:05.1 & $171.42$ &  \\
 & & & G320.236$-$00.099 & G & 15:09:11.0 & $-58$:15:53.6 & $168.90$ &  \\
 & & & G320.249$-$00.043 & Q & 15:09:03.3 & $-58$:12:37.2 & $14.34$ &  \\
 & & & G320.278$-$00.157 & G & 15:09:41.0 & $-58$:17:39.1 & $151.48$ &  \\
 & & & G320.298$-$00.101 & Q & 15:09:35.9 & $-58$:14:08.6 & $22.26$ &  \\
ch138 & 15:10:11.2 & $-58$:27:30.3 & G320.232$-$00.286 & G & 15:09:52.6 & $-58$:25:43.9 & $27.56$ &  \\
 & & & G320.248$-$00.278 & Q & 15:09:57.0 & $-58$:24:48.5 & $47.25$ &  \\
 & & & G320.255$-$00.326 & K & 15:10:10.8 & $-58$:27:03.5 & $270.21$ & CH87  \\
 & & & G320.331$-$00.307 & C & 15:10:36.5 & $-58$:23:47.2 & $65.06$ &  \\
ch139 & 15:10:08.1 & $-58$:19:06.9 & G320.240$-$00.176 & G & 15:09:30.2 & $-58$:19:45.8 & $83.56$ &  \\
 & & & G320.255$-$00.326 & K & 15:10:10.8 & $-58$:27:03.5 & $270.21$ & CH87  \\
 & & & G320.278$-$00.157 & G & 15:09:41.0 & $-58$:17:39.1 & $151.48$ &  \\
 & & & G320.278$-$00.217 & G & 15:09:54.8 & $-58$:20:45.6 & $106.02$ &  \\
 & & & G320.311$-$00.176 & K & 15:09:58.4 & $-58$:17:38.1 & $91.96$ & CH87  \\
 & & & G320.322$-$00.257 & Q & 15:10:21.3 & $-58$:21:27.4 & $58.54$ &  \\
 & & & G320.343$-$00.180 & K & 15:10:11.8 & $-58$:16:51.9 & $76.12$ & CH87  \\
 & & & G320.346$-$00.215 & K & 15:10:21.1 & $-58$:18:34.0 & $85.52$ & CH87  \\
 & & & G320.349$-$00.223 & Q & 15:10:24.1 & $-58$:18:54.1 & $23.20$ &  \\
shrds552 & 15:10:35.1 & $-58$:23:42.9 & G320.255$-$00.326 & K & 15:10:10.8 & $-58$:27:03.5 & $270.21$ & CH87  \\
 & & & G320.322$-$00.257 & Q & 15:10:21.3 & $-58$:21:27.4 & $58.54$ &  \\
 & & & G320.331$-$00.307 & C & 15:10:36.5 & $-58$:23:47.2 & $65.06$ &  \\
 & & & G320.346$-$00.215 & K & 15:10:21.1 & $-58$:18:34.0 & $85.52$ & CH87  \\
 & & & G320.426$-$00.270 & C & 15:11:05.2 & $-58$:18:57.1 & $135.56$ &  \\
shrds555 & 15:09:32.4 & $-57$:59:25.2 & G320.354+00.114 & Q & 15:09:08.7 & $-58$:01:18.2 & $23.67$ &  \\
 & & & G320.357+00.153 & K & 15:09:00.9 & $-57$:59:10.2 & $69.99$ & CH87  \\
 & & & G320.376+00.172 & K & 15:09:04.0 & $-57$:57:37.3 & $70.15$ & CH87  \\
 & & & G320.399+00.162 & K & 15:09:15.4 & $-57$:57:28.0 & $50.48$ & CH87  \\
 & & & G320.407+00.134 & K & 15:09:24.8 & $-57$:58:39.2 & $135.25$ & CH87  \\
 & & & G320.419+00.114 & C & 15:09:34.0 & $-57$:59:19.5 & $36.61$ &  \\
 & & & G320.423+00.101 & C & 15:09:38.6 & $-57$:59:52.8 & $36.61$ &  \\
 & & & G320.431+00.114 & Q & 15:09:38.7 & $-57$:58:56.8 & $20.62$ &  \\
shrds1144g & 15:10:17.6 & $-57$:40:44.0 & G320.590+00.190 & G & 15:10:23.2 & $-57$:50:10.9 & $435.24$ &  \\
 & & & G320.663+00.336 & G & 15:10:18.2 & $-57$:40:24.8 & $138.30$ &  \\
 & & & G320.692+00.185 & K & 15:11:04.0 & $-57$:47:20.8 & $341.06$ & CH87  \\
shrds559 & 15:10:49.2 & $-57$:45:04.1 & G320.590+00.190 & G & 15:10:23.2 & $-57$:50:10.9 & $435.24$ &  \\
 & & & G320.663+00.336 & G & 15:10:18.2 & $-57$:40:24.8 & $138.30$ &  \\
 & & & G320.675+00.246 & C & 15:10:43.5 & $-57$:44:44.0 & $42.28$ &  \\
 & & & G320.692+00.185 & K & 15:11:04.0 & $-57$:47:20.8 & $341.06$ & CH87  \\
 & & & G320.782+00.258 & G & 15:11:22.1 & $-57$:40:50.1 & $147.82$ &  \\
 & & & G320.799+00.187 & G & 15:11:44.9 & $-57$:43:57.6 & $216.02$ &  \\
shrds1146 & 15:11:22.2 & $-57$:40:22.3 & G320.692+00.185 & K & 15:11:04.0 & $-57$:47:20.8 & $341.06$ & CH87  \\
 & & & G320.778+00.241 & G & 15:11:24.5 & $-57$:41:50.2 & $37.97$ &  \\
 & & & G320.782+00.258 & G & 15:11:22.1 & $-57$:40:50.1 & $147.82$ &  \\
 & & & G320.799+00.187 & G & 15:11:44.9 & $-57$:43:57.6 & $216.02$ &  \\
shrds1147 & 15:11:46.1 & $-57$:44:20.2 & G320.692+00.185 & K & 15:11:04.0 & $-57$:47:20.8 & $341.06$ & CH87  \\
 & & & G320.778+00.241 & G & 15:11:24.5 & $-57$:41:50.2 & $37.97$ &  \\
 & & & G320.782+00.258 & G & 15:11:22.1 & $-57$:40:50.1 & $147.82$ &  \\
 & & & G320.799+00.187 & G & 15:11:44.9 & $-57$:43:57.6 & $216.02$ &  \\
shrds561 & 15:15:33.5 & $-58$:23:30.4 & G320.884$-$00.641 & C & 15:15:32.3 & $-58$:23:50.0 & $138.34$ &  \\
 & & & G321.061$-$00.763 & C & 15:17:10.7 & $-58$:24:28.7 & $533.84$ &  \\
ch142 & 15:16:03.2 & $-58$:12:47.5 & G320.956$-$00.505 & G & 15:15:27.8 & $-58$:14:36.4 & $79.44$ &  \\
 & & & G321.015$-$00.527 & K & 15:15:56.0 & $-58$:13:53.7 & $242.38$ & CH87  \\
 & & & G321.109$-$00.414 & G & 15:16:05.4 & $-58$:05:08.8 & $372.62$ &  \\
 & & & G321.115$-$00.546 & K & 15:16:39.4 & $-58$:11:43.6 & $251.12$ & CH87  \\
shrds563 & 15:15:34.2 & $-57$:57:32.0 & G321.109$-$00.414 & G & 15:16:05.4 & $-58$:05:08.8 & $372.62$ &  \\
 & & & G321.114$-$00.273 & C & 15:15:33.9 & $-57$:57:48.7 & $106.72$ &  \\
ch144 & 15:13:49.4 & $-56$:25:57.8 & G321.725+01.169 & K & 15:13:52.3 & $-56$:24:52.4 & $175.12$ & CH87  \\
caswell14 & 15:13:49.9 & $-56$:24:48.0 & G321.725+01.169 & K & 15:13:52.3 & $-56$:24:52.4 & $175.12$ & CH87  \\
ch145 & 15:18:38.0 & $-56$:39:45.6 & G322.036+00.625 & G & 15:17:51.8 & $-56$:42:51.3 & $386.37$ &  \\
 & & & G322.162+00.625 & K & 15:18:38.4 & $-56$:38:50.1 & $174.22$ & CH87  \\
 & & & G322.220+00.504 & G & 15:19:28.2 & $-56$:43:07.6 & $480.22$ &  \\
caswell15 & 15:18:39.2 & $-56$:39:00.9 & G322.036+00.625 & G & 15:17:51.8 & $-56$:42:51.3 & $386.37$ &  \\
 & & & G322.162+00.625 & K & 15:18:38.4 & $-56$:38:50.1 & $174.22$ & CH87  \\
 & & & G322.220+00.504 & G & 15:19:28.2 & $-56$:43:07.6 & $480.22$ &  \\
shrds1151 & 15:18:54.7 & $-56$:41:42.9 & G322.036+00.625 & G & 15:17:51.8 & $-56$:42:51.3 & $386.37$ &  \\
 & & & G322.162+00.625 & K & 15:18:38.4 & $-56$:38:50.1 & $174.22$ & CH87  \\
 & & & G322.220+00.504 & G & 15:19:28.2 & $-56$:43:07.6 & $480.22$ &  \\
shrds574 & 15:25:47.3 & $-57$:08:54.6 & G322.706$-$00.330 & C & 15:25:47.5 & $-57$:09:09.9 & $77.40$ &  \\
shrds584 & 15:27:47.0 & $-55$:48:26.9 & G323.680+00.631 & C & 15:27:45.6 & $-55$:48:41.3 & $145.60$ &  \\
shrds589 & 15:31:05.0 & $-56$:06:45.4 & G323.895+00.116 & C & 15:31:06.5 & $-56$:06:51.3 & $65.66$ &  \\
shrds590 & 15:31:34.3 & $-56$:10:12.1 & G323.895+00.116 & C & 15:31:06.5 & $-56$:06:51.3 & $65.66$ &  \\
 & & & G323.915+00.026 & C & 15:31:35.9 & $-56$:10:37.7 & $69.12$ &  \\
 & & & G323.936$-$00.038 & C & 15:31:59.0 & $-56$:13:00.6 & $217.18$ &  \\
 & & & G323.942+00.042 & Q & 15:31:41.3 & $-56$:08:52.4 & $20.48$ &  \\
 & & & G323.973+00.057 & K & 15:31:48.6 & $-56$:07:05.0 & $48.91$ & CH87  \\
 & & & G324.025+00.089 & C & 15:31:59.1 & $-56$:03:43.3 & $205.50$ &  \\
ch149 & 15:32:52.9 & $-55$:57:00.3 & G324.135+00.236 & K & 15:32:01.5 & $-55$:52:42.6 & $386.29$ & CH87  \\
 & & & G324.201+00.117 & K & 15:32:54.0 & $-55$:56:16.6 & $156.60$ & CH87  \\
caswell16 & 15:32:53.5 & $-55$:56:17.2 & G324.135+00.236 & K & 15:32:01.5 & $-55$:52:42.6 & $386.29$ & CH87  \\
 & & & G324.201+00.117 & K & 15:32:54.0 & $-55$:56:16.6 & $156.60$ & CH87  \\
shrds599 & 15:40:11.1 & $-56$:06:11.9 & G324.924$-$00.569 & K & 15:39:58.2 & $-56$:04:10.5 & $78.75$ & CH87  \\
 & & & G324.931$-$00.621 & C & 15:40:13.9 & $-56$:06:25.5 & $52.01$ &  \\
shrds1161 & 15:45:59.0 & $-55$:14:43.9 & G326.036$-$00.497 & G & 15:45:56.3 & $-55$:20:18.2 & $251.91$ &  \\
 & & & G326.065$-$00.393 & G & 15:45:39.1 & $-55$:14:18.5 & $234.61$ &  \\
 & & & G326.474$-$00.292 & K & 15:47:28.1 & $-54$:54:25.4 & $1252.65$ & CH87  \\
ch152 & 15:40:49.3 & $-54$:03:01.0 & G326.270+00.783 & K & 15:41:49.8 & $-54$:10:48.2 & $949.79$ & CH87  \\
ch154 & 15:42:13.4 & $-53$:58:22.4 & G326.270+00.783 & K & 15:41:49.8 & $-54$:10:48.2 & $949.79$ & CH87  \\
 & & & G326.446+00.901 & K & 15:42:18.0 & $-53$:58:46.2 & $178.99$ & CH87  \\
caswell17 & 15:42:18.3 & $-53$:58:25.8 & G326.270+00.783 & K & 15:41:49.8 & $-54$:10:48.2 & $949.79$ & CH87  \\
 & & & G326.446+00.901 & K & 15:42:18.0 & $-53$:58:46.2 & $178.99$ & CH87  \\
shrds609 & 15:47:49.7 & $-54$:58:44.7 & G326.467$-$00.382 & C & 15:47:49.1 & $-54$:58:55.6 & $32.43$ &  \\
 & & & G326.473$-$00.378 & C & 15:47:50.0 & $-54$:58:30.9 & $32.43$ &  \\
 & & & G326.474$-$00.292 & K & 15:47:28.1 & $-54$:54:25.4 & $1252.65$ & CH87  \\
ch156 & 15:44:40.3 & $-54$:06:26.4 & G326.628+00.612 & Q & 15:44:28.9 & $-54$:05:56.7 & $33.84$ &  \\
 & & & G326.643+00.514 & K & 15:44:58.2 & $-54$:10:02.0 & $524.91$ & CH87  \\
 & & & G326.657+00.588 & G & 15:44:44.2 & $-54$:06:00.3 & $118.28$ &  \\
 & & & G326.728+00.616 & G & 15:45:00.3 & $-54$:02:06.2 & $118.28$ &  \\
shrds1163 & 15:44:44.2 & $-54$:05:60.0 & G326.628+00.612 & Q & 15:44:28.9 & $-54$:05:56.7 & $33.84$ &  \\
 & & & G326.643+00.514 & K & 15:44:58.2 & $-54$:10:02.0 & $524.91$ & CH87  \\
 & & & G326.657+00.588 & G & 15:44:44.2 & $-54$:06:00.3 & $118.28$ &  \\
 & & & G326.728+00.616 & G & 15:45:00.3 & $-54$:02:06.2 & $118.28$ &  \\
shrds1164 & 15:45:00.4 & $-54$:02:06.9 & G326.643+00.514 & K & 15:44:58.2 & $-54$:10:02.0 & $524.91$ & CH87  \\
 & & & G326.657+00.588 & G & 15:44:44.2 & $-54$:06:00.3 & $118.28$ &  \\
 & & & G326.728+00.616 & G & 15:45:00.3 & $-54$:02:06.2 & $118.28$ &  \\
 & & & G326.780+00.669 & Q & 15:45:03.7 & $-53$:57:38.8 & $77.14$ &  \\
shrds618 & 15:50:56.6 & $-54$:28:23.6 & G326.900$-$00.347 & K & 15:50:01.1 & $-54$:41:05.8 & $683.04$ & CH87  \\
 & & & G327.078+00.050 & K & 15:49:16.2 & $-54$:15:49.6 & $1049.93$ & CH87  \\
 & & & G327.128$-$00.371 & Q & 15:51:21.2 & $-54$:33:40.7 & $189.24$ &  \\
 & & & G327.139$-$00.261 & C & 15:50:56.1 & $-54$:28:06.8 & $91.80$ &  \\
shrds1167 & 15:52:33.1 & $-54$:43:42.6 & G327.172$-$00.527 & G & 15:52:15.9 & $-54$:39:14.4 & $546.34$ &  \\
caswell18 & 15:53:02.8 & $-54$:35:13.8 & G327.172$-$00.527 & G & 15:52:15.9 & $-54$:39:14.4 & $546.34$ &  \\
 & & & G327.263$-$00.500 & Q & 15:52:38.1 & $-54$:34:32.4 & $39.35$ &  \\
 & & & G327.267$-$00.557 & Q & 15:52:54.3 & $-54$:37:02.3 & $24.74$ &  \\
 & & & G327.269$-$00.572 & Q & 15:52:59.1 & $-54$:37:41.3 & $21.21$ &  \\
 & & & G327.273$-$00.578 & Q & 15:53:01.8 & $-54$:37:47.8 & $21.21$ &  \\
 & & & G327.285$-$00.576 & K & 15:53:05.2 & $-54$:37:15.0 & $45.22$ & CH87  \\
 & & & G327.287$-$00.589 & Q & 15:53:09.1 & $-54$:37:45.7 & $21.21$ &  \\
 & & & G327.295$-$00.562 & Q & 15:53:04.8 & $-54$:36:14.1 & $24.74$ &  \\
 & & & G327.296$-$00.595 & Q & 15:53:13.6 & $-54$:37:41.5 & $21.21$ &  \\
 & & & G327.300$-$00.548 & K & 15:53:02.6 & $-54$:35:22.3 & $276.04$ & CH87  \\
 & & & G327.454$-$00.633 & G & 15:54:14.3 & $-54$:33:27.3 & $633.52$ &  \\
ch162 & 15:53:03.7 & $-54$:34:20.8 & G327.172$-$00.527 & G & 15:52:15.9 & $-54$:39:14.4 & $546.34$ &  \\
 & & & G327.263$-$00.500 & Q & 15:52:38.1 & $-54$:34:32.4 & $39.35$ &  \\
 & & & G327.267$-$00.557 & Q & 15:52:54.3 & $-54$:37:02.3 & $24.74$ &  \\
 & & & G327.269$-$00.572 & Q & 15:52:59.1 & $-54$:37:41.3 & $21.21$ &  \\
 & & & G327.273$-$00.578 & Q & 15:53:01.8 & $-54$:37:47.8 & $21.21$ &  \\
 & & & G327.285$-$00.576 & K & 15:53:05.2 & $-54$:37:15.0 & $45.22$ & CH87  \\
 & & & G327.287$-$00.589 & Q & 15:53:09.1 & $-54$:37:45.7 & $21.21$ &  \\
 & & & G327.295$-$00.562 & Q & 15:53:04.8 & $-54$:36:14.1 & $24.74$ &  \\
 & & & G327.296$-$00.595 & Q & 15:53:13.6 & $-54$:37:41.5 & $21.21$ &  \\
 & & & G327.300$-$00.548 & K & 15:53:02.6 & $-54$:35:22.3 & $276.04$ & CH87  \\
 & & & G327.454$-$00.633 & G & 15:54:14.3 & $-54$:33:27.3 & $633.52$ &  \\
shrds1168 & 15:53:24.1 & $-54$:35:34.5 & G327.172$-$00.527 & G & 15:52:15.9 & $-54$:39:14.4 & $546.34$ &  \\
 & & & G327.267$-$00.557 & Q & 15:52:54.3 & $-54$:37:02.3 & $24.74$ &  \\
 & & & G327.269$-$00.572 & Q & 15:52:59.1 & $-54$:37:41.3 & $21.21$ &  \\
 & & & G327.273$-$00.578 & Q & 15:53:01.8 & $-54$:37:47.8 & $21.21$ &  \\
 & & & G327.285$-$00.576 & K & 15:53:05.2 & $-54$:37:15.0 & $45.22$ & CH87  \\
 & & & G327.287$-$00.589 & Q & 15:53:09.1 & $-54$:37:45.7 & $21.21$ &  \\
 & & & G327.295$-$00.562 & Q & 15:53:04.8 & $-54$:36:14.1 & $24.74$ &  \\
 & & & G327.296$-$00.595 & Q & 15:53:13.6 & $-54$:37:41.5 & $21.21$ &  \\
 & & & G327.300$-$00.548 & K & 15:53:02.6 & $-54$:35:22.3 & $276.04$ & CH87  \\
 & & & G327.454$-$00.633 & G & 15:54:14.3 & $-54$:33:27.3 & $633.52$ &  \\
shrds621 & 15:49:19.2 & $-53$:45:46.0 & G327.400+00.444 & C & 15:49:18.7 & $-53$:45:17.7 & $38.48$ &  \\
 & & & G327.401+00.483 & C & 15:49:09.2 & $-53$:43:26.5 & $133.68$ &  \\
shrds628 & 15:54:40.2 & $-54$:11:34.6 & G327.651$-$00.334 & K & 15:53:58.4 & $-54$:12:05.8 & $130.56$ & CH87  \\
 & & & G327.708$-$00.392 & C & 15:54:31.5 & $-54$:12:35.0 & $48.00$ &  \\
 & & & G327.735$-$00.396 & C & 15:54:41.1 & $-54$:11:44.1 & $70.14$ &  \\
 & & & G327.757$-$00.331 & Q & 15:54:31.2 & $-54$:07:54.9 & $33.22$ &  \\
 & & & G327.770$-$00.346 & K & 15:54:39.1 & $-54$:08:05.1 & $122.34$ & CH87  \\
 & & & G327.773$-$00.344 & Q & 15:54:39.4 & $-54$:07:52.0 & $18.27$ &  \\
shrds634 & 15:54:09.6 & $-53$:56:55.1 & G327.838$-$00.140 & C & 15:54:06.8 & $-53$:55:57.7 & $92.59$ &  \\
 & & & G327.889$-$00.045 & C & 15:53:58.3 & $-53$:49:37.9 & $358.62$ &  \\
 & & & G327.910$-$00.155 & C & 15:54:33.4 & $-53$:53:55.0 & $65.63$ &  \\
shrds635 & 15:53:30.4 & $-53$:48:13.2 & G327.824+00.117 & K & 15:52:56.1 & $-53$:44:35.0 & $236.65$ & CH87  \\
 & & & G327.848+00.016 & C & 15:53:29.5 & $-53$:48:20.4 & $31.11$ &  \\
 & & & G327.889$-$00.045 & C & 15:53:58.3 & $-53$:49:37.9 & $358.62$ &  \\
shrds639 & 15:53:14.4 & $-53$:39:22.6 & G327.824+00.117 & K & 15:52:56.1 & $-53$:44:35.0 & $236.65$ & CH87  \\
 & & & G327.852+00.189 & Q & 15:52:46.3 & $-53$:40:09.8 & $14.49$ &  \\
 & & & G327.857+00.189 & Q & 15:52:48.0 & $-53$:40:00.4 & $7.62$ &  \\
 & & & G327.867+00.173 & Q & 15:52:55.1 & $-53$:40:20.1 & $43.33$ &  \\
 & & & G327.885+00.147 & Q & 15:53:07.4 & $-53$:40:51.1 & $17.56$ &  \\
 & & & G327.916+00.154 & C & 15:53:15.3 & $-53$:39:21.1 & $60.03$ &  \\
shrds638 & 15:57:00.2 & $-54$:19:17.0 & G327.878$-$00.727 & C & 15:56:53.5 & $-54$:21:28.8 & $130.53$ &  \\
 & & & G327.927$-$00.694 & C & 15:57:00.0 & $-54$:18:02.9 & $409.18$ &  \\
shrds640 & 15:54:15.9 & $-53$:44:28.6 & G327.889$-$00.045 & C & 15:53:58.3 & $-53$:49:37.9 & $358.62$ &  \\
 & & & G327.979$-$00.006 & C & 15:54:16.4 & $-53$:44:23.6 & $42.05$ &  \\
 & & & G327.991$-$00.087 & K & 15:54:41.1 & $-53$:47:39.8 & $182.72$ & CH87  \\
shrds643 & 15:53:18.7 & $-53$:27:40.4 & G328.043+00.298 & C & 15:53:18.1 & $-53$:27:50.9 & $94.13$ &  \\
 & & & G328.118+00.374 & Q & 15:53:22.1 & $-53$:21:29.2 & $313.54$ &  \\
shrds644 & 15:54:20.6 & $-53$:37:07.7 & G328.062+00.076 & C & 15:54:21.1 & $-53$:37:24.6 & $48.00$ &  \\
 & & & G328.117+00.108 & C & 15:54:30.1 & $-53$:33:51.1 & $106.92$ &  \\
shrds647 & 15:54:31.1 & $-53$:33:39.2 & G328.062+00.076 & C & 15:54:21.1 & $-53$:37:24.6 & $48.00$ &  \\
 & & & G328.117+00.108 & C & 15:54:30.1 & $-53$:33:51.1 & $106.92$ &  \\
 & & & G328.146+00.185 & C & 15:54:19.1 & $-53$:29:08.5 & $48.00$ &  \\
shrds646 & 15:52:33.3 & $-53$:11:54.2 & G328.069+00.573 & Q & 15:52:16.2 & $-53$:14:04.9 & $19.38$ &  \\
 & & & G328.073+00.580 & C & 15:52:15.6 & $-53$:13:35.9 & $31.14$ &  \\
 & & & G328.075+00.590 & Q & 15:52:13.7 & $-53$:13:03.6 & $23.16$ &  \\
 & & & G328.117+00.570 & C & 15:52:32.0 & $-53$:12:25.9 & $89.18$ &  \\
 & & & G328.165+00.587 & C & 15:52:42.6 & $-53$:09:49.2 & $21.95$ &  \\
shrds648 & 15:54:15.9 & $-53$:28:45.1 & G328.117+00.108 & C & 15:54:30.1 & $-53$:33:51.1 & $106.92$ &  \\
 & & & G328.146+00.185 & C & 15:54:19.1 & $-53$:29:08.5 & $48.00$ &  \\
shrds651 & 15:57:24.0 & $-53$:58:12.3 & G328.029$-$00.488 & C & 15:56:37.7 & $-54$:04:39.7 & $375.62$ &  \\
 & & & G328.193$-$00.479 & C & 15:57:26.7 & $-53$:57:56.0 & $142.02$ &  \\
 & & & G328.193$-$00.569 & C & 15:57:50.3 & $-54$:02:01.9 & $116.42$ &  \\
shrds652 & 15:57:49.8 & $-54$:02:13.5 & G328.162$-$00.614 & C & 15:57:52.5 & $-54$:05:17.9 & $175.83$ &  \\
 & & & G328.193$-$00.479 & C & 15:57:26.7 & $-53$:57:56.0 & $142.02$ &  \\
 & & & G328.193$-$00.569 & C & 15:57:50.3 & $-54$:02:01.9 & $116.42$ &  \\
 & & & G328.224$-$00.582 & C & 15:58:03.4 & $-54$:01:26.0 & $92.84$ &  \\
 & & & G328.240$-$00.545 & C & 15:57:58.7 & $-53$:59:07.9 & $15.89$ &  \\
 & & & G328.248$-$00.532 & Q & 15:57:57.6 & $-53$:58:11.9 & $12.99$ &  \\
 & & & G328.253$-$00.531 & Q & 15:57:59.1 & $-53$:57:59.5 & $18.54$ &  \\
 & & & G328.279$-$00.559 & K & 15:58:14.5 & $-53$:58:15.5 & $98.15$ & CH87  \\
shrds656 & 15:53:55.5 & $-53$:14:13.5 & G328.118+00.374 & Q & 15:53:22.1 & $-53$:21:29.2 & $313.54$ &  \\
 & & & G328.250+00.403 & C & 15:53:55.6 & $-53$:15:05.3 & $82.45$ &  \\
 & & & G328.286+00.464 & K & 15:53:51.3 & $-53$:10:55.2 & $96.13$ & CH87  \\
 & & & G328.314+00.360 & C & 15:54:26.4 & $-53$:14:38.5 & $49.35$ &  \\
 & & & G328.320+00.383 & Q & 15:54:22.3 & $-53$:13:20.4 & $50.27$ &  \\
 & & & G328.320+00.435 & K & 15:54:09.2 & $-53$:10:57.7 & $105.14$ & CH87  \\
ch168 & 15:54:02.8 & $-53$:10:45.1 & G328.250+00.403 & C & 15:53:55.6 & $-53$:15:05.3 & $82.45$ &  \\
 & & & G328.286+00.464 & K & 15:53:51.3 & $-53$:10:55.2 & $96.13$ & CH87  \\
 & & & G328.320+00.383 & Q & 15:54:22.3 & $-53$:13:20.4 & $50.27$ &  \\
 & & & G328.320+00.435 & K & 15:54:09.2 & $-53$:10:57.7 & $105.14$ & CH87  \\
shrds657 & 15:54:24.8 & $-53$:14:38.7 & G328.250+00.403 & C & 15:53:55.6 & $-53$:15:05.3 & $82.45$ &  \\
 & & & G328.314+00.360 & C & 15:54:26.4 & $-53$:14:38.5 & $49.35$ &  \\
 & & & G328.320+00.383 & Q & 15:54:22.3 & $-53$:13:20.4 & $50.27$ &  \\
 & & & G328.320+00.435 & K & 15:54:09.2 & $-53$:10:57.7 & $105.14$ & CH87  \\
shrds659 & 15:58:35.4 & $-53$:55:39.6 & G328.277$-$00.530 & Q & 15:58:06.3 & $-53$:57:00.6 & $20.19$ &  \\
 & & & G328.279$-$00.559 & K & 15:58:14.5 & $-53$:58:15.5 & $98.15$ & CH87  \\
 & & & G328.294$-$00.536 & Q & 15:58:12.9 & $-53$:56:35.4 & $42.10$ &  \\
 & & & G328.315$-$00.594 & K & 15:58:34.8 & $-53$:58:25.7 & $93.40$ & CH87  \\
 & & & G328.355$-$00.485 & Q & 15:58:18.4 & $-53$:51:53.7 & $28.96$ &  \\
 & & & G328.356$-$00.559 & C & 15:58:38.3 & $-53$:55:14.7 & $96.57$ &  \\
ch171 & 15:55:48.6 & $-52$:42:47.1 & G328.809+00.634 & K & 15:55:48.4 & $-52$:43:02.1 & $101.65$ & CH87  \\
shrds668 & 15:58:34.0 & $-53$:11:45.8 & G328.807$-$00.078 & K & 15:58:50.9 & $-53$:15:44.8 & $131.59$ & CH87  \\
 & & & G328.819$-$00.004 & C & 15:58:35.2 & $-53$:11:52.3 & $72.03$ &  \\
shrds669 & 15:56:47.5 & $-52$:40:27.7 & G328.945+00.570 & C & 15:56:45.9 & $-52$:40:43.9 & $118.31$ &  \\
 & & & G328.946+00.551 & Q & 15:56:51.1 & $-52$:41:34.3 & $39.15$ &  \\
 & & & G328.982+00.572 & Q & 15:56:56.5 & $-52$:39:11.9 & $20.84$ &  \\
 & & & G328.996+00.602 & C & 15:56:53.0 & $-52$:37:15.8 & $113.16$ &  \\
shrds670 & 15:58:12.1 & $-52$:55:01.6 & G328.961+00.248 & C & 15:58:13.1 & $-52$:54:49.9 & $79.82$ &  \\
 & & & G328.962+00.207 & C & 15:58:24.1 & $-52$:56:40.6 & $88.35$ &  \\
shrds674 & 16:00:45.6 & $-53$:17:38.5 & G329.005$-$00.291 & C & 16:00:46.8 & $-53$:17:39.6 & $92.78$ &  \\
shrds677 & 16:00:19.9 & $-52$:49:24.7 & G329.265+00.046 & C & 16:00:37.3 & $-52$:52:10.2 & $63.90$ &  \\
 & & & G329.266+00.111 & C & 16:00:20.8 & $-52$:49:11.9 & $120.72$ &  \\
 & & & G329.338+00.147 & K & 16:00:32.9 & $-52$:44:42.5 & $77.26$ & CH87  \\
 & & & G329.340+00.121 & K & 16:00:40.3 & $-52$:45:48.9 & $57.86$ & CH87  \\
shrds679 & 16:00:52.1 & $-52$:43:23.1 & G329.338+00.147 & K & 16:00:32.9 & $-52$:44:42.5 & $77.26$ & CH87  \\
 & & & G329.340+00.121 & K & 16:00:40.3 & $-52$:45:48.9 & $57.86$ & CH87  \\
 & & & G329.389+00.135 & C & 16:00:51.4 & $-52$:43:15.9 & $56.06$ &  \\
 & & & G329.408+00.163 & Q & 16:00:49.9 & $-52$:41:16.3 & $29.35$ &  \\
 & & & G329.460+00.174 & C & 16:01:02.7 & $-52$:38:43.9 & $66.34$ &  \\
shrds683 & 16:03:29.5 & $-53$:09:30.8 & G329.388$-$00.447 & Q & 16:03:23.7 & $-53$:09:37.5 & $49.35$ &  \\
 & & & G329.389$-$00.473 & Q & 16:03:30.9 & $-53$:10:45.2 & $24.10$ &  \\
 & & & G329.390$-$00.486 & C & 16:03:34.6 & $-53$:11:17.5 & $82.00$ &  \\
 & & & G329.398$-$00.458 & C & 16:03:29.6 & $-53$:09:42.9 & $33.58$ &  \\
 & & & G329.407$-$00.458 & Q & 16:03:32.3 & $-53$:09:21.5 & $26.43$ &  \\
shrds684 & 16:02:17.4 & $-52$:55:32.9 & G329.389$-$00.072 & C & 16:01:45.4 & $-52$:52:39.5 & $296.56$ &  \\
 & & & G329.422$-$00.160 & C & 16:02:18.2 & $-52$:55:18.9 & $82.84$ &  \\
shrds685 & 15:59:33.0 & $-52$:23:38.9 & G329.445+00.504 & C & 15:59:33.1 & $-52$:24:18.8 & $65.82$ &  \\
 & & & G329.464+00.504 & Q & 15:59:38.8 & $-52$:23:35.1 & $18.65$ &  \\
shrds686 & 16:01:02.3 & $-52$:38:51.6 & G329.389+00.135 & C & 16:00:51.4 & $-52$:43:15.9 & $56.06$ &  \\
 & & & G329.408+00.163 & Q & 16:00:49.9 & $-52$:41:16.3 & $29.35$ &  \\
 & & & G329.454+00.236 & Q & 16:00:44.8 & $-52$:36:09.2 & $24.37$ &  \\
 & & & G329.460+00.174 & C & 16:01:02.7 & $-52$:38:43.9 & $66.34$ &  \\
 & & & G329.465+00.207 & K & 16:00:55.6 & $-52$:37:01.8 & $16.53$ & CH87  \\
 & & & G329.465+00.235 & Q & 16:00:48.4 & $-52$:35:46.1 & $19.91$ &  \\
 & & & G329.470+00.205 & K & 16:00:57.5 & $-52$:36:54.4 & $18.04$ & CH87  \\
 & & & G329.472+00.214 & K & 16:00:55.7 & $-52$:36:25.2 & $55.04$ & CH87  \\
 & & & G329.475+00.226 & Q & 16:00:53.6 & $-52$:35:46.0 & $25.73$ &  \\
 & & & G329.567+00.242 & C & 16:01:17.0 & $-52$:31:26.4 & $262.44$ &  \\
shrds687 & 15:58:16.0 & $-52$:07:44.6 & G329.474+00.839 & C & 15:58:16.2 & $-52$:07:52.6 & $67.31$ &  \\
shrds690 & 16:02:13.4 & $-52$:38:37.6 & G329.530+00.093 & Q & 16:01:44.6 & $-52$:39:38.6 & $19.52$ &  \\
 & & & G329.601+00.059 & C & 16:02:14.4 & $-52$:38:21.2 & $86.30$ &  \\
 & & & G329.649+00.094 & Q & 16:02:19.7 & $-52$:34:53.8 & $41.30$ &  \\
ch174 & 16:04:51.9 & $-52$:25:35.6 & G329.976$-$00.002 & Q & 16:04:21.4 & $-52$:26:13.6 & $121.39$ &  \\
 & & & G330.039$-$00.058 & K & 16:04:54.6 & $-52$:26:13.9 & $142.10$ & CH87  \\
shrds697 & 16:00:50.2 & $-51$:42:50.2 & G329.804+00.917 & C & 15:59:34.4 & $-51$:51:29.2 & $941.87$ &  \\
 & & & G330.049+00.899 & C & 16:00:50.9 & $-51$:42:41.4 & $99.60$ &  \\
 & & & G330.121+00.687 & C & 16:02:06.0 & $-51$:49:28.0 & $786.92$ &  \\
shrds1171 & 16:09:50.8 & $-52$:15:28.8 & G330.673$-$00.388 & K & 16:09:26.3 & $-52$:15:23.7 & $113.85$ & CH87  \\
 & & & G330.738$-$00.449 & G & 16:10:01.1 & $-52$:15:25.3 & $148.18$ &  \\
 & & & G330.775$-$00.398 & G & 16:09:58.3 & $-52$:11:41.1 & $358.22$ &  \\
shrds1172 & 16:09:58.4 & $-52$:09:50.3 & G330.738$-$00.449 & G & 16:10:01.1 & $-52$:15:25.3 & $148.18$ &  \\
 & & & G330.775$-$00.398 & G & 16:09:58.3 & $-52$:11:41.1 & $358.22$ &  \\
 & & & G330.873$-$00.369 & K & 16:10:18.8 & $-52$:06:24.5 & $98.86$ & CH87  \\
 & & & G330.986$-$00.433 & G & 16:11:08.1 & $-52$:04:36.2 & $572.96$ &  \\
ch177 & 16:10:14.6 & $-52$:07:13.1 & G330.775$-$00.398 & G & 16:09:58.3 & $-52$:11:41.1 & $358.22$ &  \\
 & & & G330.873$-$00.369 & K & 16:10:18.8 & $-52$:06:24.5 & $98.86$ & CH87  \\
 & & & G330.986$-$00.433 & G & 16:11:08.1 & $-52$:04:36.2 & $572.96$ &  \\
shrds709 & 16:09:52.7 & $-51$:54:38.6 & G330.954$-$00.181 & C & 16:09:52.2 & $-51$:54:49.5 & $66.43$ &  \\
 & & & G330.966$-$00.190 & Q & 16:09:58.1 & $-51$:54:45.0 & $28.84$ &  \\
 & & & G331.020$-$00.143 & K & 16:10:01.2 & $-51$:50:29.5 & $228.96$ & CH87  \\
shrds710 & 16:11:27.7 & $-52$:01:46.7 & G330.986$-$00.433 & G & 16:11:08.1 & $-52$:04:36.2 & $572.96$ &  \\
 & & & G331.056$-$00.437 & C & 16:11:29.1 & $-52$:01:55.1 & $75.67$ &  \\
 & & & G331.127$-$00.481 & C & 16:12:01.3 & $-52$:00:58.6 & $64.02$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds711 & 16:10:37.5 & $-51$:52:55.2 & G330.986$-$00.433 & G & 16:11:08.1 & $-52$:04:36.2 & $572.96$ &  \\
 & & & G331.020$-$00.143 & K & 16:10:01.2 & $-51$:50:29.5 & $228.96$ & CH87  \\
 & & & G331.057$-$00.229 & C & 16:10:34.3 & $-51$:52:45.0 & $79.53$ &  \\
 & & & G331.120$-$00.248 & C & 16:10:57.3 & $-51$:51:00.3 & $231.19$ &  \\
 & & & G331.121$-$00.169 & C & 16:10:36.8 & $-51$:47:30.0 & $103.18$ &  \\
 & & & G331.129$-$00.243 & C & 16:10:58.5 & $-51$:50:25.5 & $44.24$ &  \\
ch179 & 16:12:03.1 & $-52$:02:46.2 & G330.986$-$00.433 & G & 16:11:08.1 & $-52$:04:36.2 & $572.96$ &  \\
 & & & G331.056$-$00.437 & C & 16:11:29.1 & $-52$:01:55.1 & $75.67$ &  \\
 & & & G331.087$-$00.518 & Q & 16:11:59.6 & $-52$:04:12.2 & $26.40$ &  \\
 & & & G331.119$-$00.496 & C & 16:12:02.9 & $-52$:01:57.0 & $28.63$ &  \\
 & & & G331.123$-$00.530 & K & 16:12:13.0 & $-52$:03:15.4 & $143.49$ & CH87  \\
 & & & G331.127$-$00.481 & C & 16:12:01.3 & $-52$:00:58.6 & $64.02$ &  \\
 & & & G331.146$-$00.480 & Q & 16:12:06.3 & $-52$:00:08.1 & $37.79$ &  \\
 & & & G331.157$-$00.462 & Q & 16:12:04.6 & $-51$:58:53.2 & $30.64$ &  \\
 & & & G331.172$-$00.460 & C & 16:12:08.5 & $-51$:58:12.7 & $104.39$ &  \\
 & & & G331.182$-$00.541 & Q & 16:12:32.9 & $-52$:01:20.0 & $56.22$ &  \\
 & & & G331.256$-$00.480 & C & 16:12:37.7 & $-51$:55:38.3 & $348.58$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds714 & 16:10:44.9 & $-51$:48:35.4 & G331.020$-$00.143 & K & 16:10:01.2 & $-51$:50:29.5 & $228.96$ & CH87  \\
 & & & G331.057$-$00.229 & C & 16:10:34.3 & $-51$:52:45.0 & $79.53$ &  \\
 & & & G331.093$-$00.131 & Q & 16:10:18.7 & $-51$:46:58.0 & $27.91$ &  \\
 & & & G331.108$-$00.124 & Q & 16:10:21.3 & $-51$:46:03.7 & $21.33$ &  \\
 & & & G331.120$-$00.248 & C & 16:10:57.3 & $-51$:51:00.3 & $231.19$ &  \\
 & & & G331.121$-$00.169 & C & 16:10:36.8 & $-51$:47:30.0 & $103.18$ &  \\
 & & & G331.129$-$00.243 & C & 16:10:58.5 & $-51$:50:25.5 & $44.24$ &  \\
shrds717 & 16:12:07.5 & $-52$:01:43.9 & G330.986$-$00.433 & G & 16:11:08.1 & $-52$:04:36.2 & $572.96$ &  \\
 & & & G331.087$-$00.518 & Q & 16:11:59.6 & $-52$:04:12.2 & $26.40$ &  \\
 & & & G331.119$-$00.496 & C & 16:12:02.9 & $-52$:01:57.0 & $28.63$ &  \\
 & & & G331.123$-$00.530 & K & 16:12:13.0 & $-52$:03:15.4 & $143.49$ & CH87  \\
 & & & G331.127$-$00.481 & C & 16:12:01.3 & $-52$:00:58.6 & $64.02$ &  \\
 & & & G331.146$-$00.480 & Q & 16:12:06.3 & $-52$:00:08.1 & $37.79$ &  \\
 & & & G331.157$-$00.462 & Q & 16:12:04.6 & $-51$:58:53.2 & $30.64$ &  \\
 & & & G331.172$-$00.460 & C & 16:12:08.5 & $-51$:58:12.7 & $104.39$ &  \\
 & & & G331.182$-$00.541 & Q & 16:12:32.9 & $-52$:01:20.0 & $56.22$ &  \\
 & & & G331.195$-$00.469 & Q & 16:12:17.4 & $-51$:57:39.8 & $37.79$ &  \\
 & & & G331.256$-$00.480 & C & 16:12:37.7 & $-51$:55:38.3 & $348.58$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds716 & 16:10:58.7 & $-51$:50:22.0 & G331.057$-$00.229 & C & 16:10:34.3 & $-51$:52:45.0 & $79.53$ &  \\
 & & & G331.120$-$00.248 & C & 16:10:57.3 & $-51$:51:00.3 & $231.19$ &  \\
 & & & G331.121$-$00.169 & C & 16:10:36.8 & $-51$:47:30.0 & $103.18$ &  \\
 & & & G331.129$-$00.243 & C & 16:10:58.5 & $-51$:50:25.5 & $44.24$ &  \\
shrds720 & 16:11:41.7 & $-51$:55:59.7 & G330.986$-$00.433 & G & 16:11:08.1 & $-52$:04:36.2 & $572.96$ &  \\
 & & & G331.156$-$00.391 & C & 16:11:45.6 & $-51$:55:50.4 & $141.66$ &  \\
 & & & G331.157$-$00.462 & Q & 16:12:04.6 & $-51$:58:53.2 & $30.64$ &  \\
 & & & G331.172$-$00.460 & C & 16:12:08.5 & $-51$:58:12.7 & $104.39$ &  \\
 & & & G331.256$-$00.480 & C & 16:12:37.7 & $-51$:55:38.3 & $348.58$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds719 & 16:09:25.0 & $-51$:33:09.0 & G331.127+00.127 & Q & 16:09:20.9 & $-51$:34:13.2 & $15.86$ &  \\
 & & & G331.137+00.112 & Q & 16:09:27.6 & $-51$:34:28.6 & $26.70$ &  \\
 & & & G331.145+00.133 & C & 16:09:24.2 & $-51$:33:11.5 & $38.91$ &  \\
 & & & G331.150+00.115 & Q & 16:09:30.4 & $-51$:33:48.1 & $27.54$ &  \\
shrds721 & 16:12:08.2 & $-51$:58:20.4 & G330.986$-$00.433 & G & 16:11:08.1 & $-52$:04:36.2 & $572.96$ &  \\
 & & & G331.119$-$00.496 & C & 16:12:02.9 & $-52$:01:57.0 & $28.63$ &  \\
 & & & G331.123$-$00.530 & K & 16:12:13.0 & $-52$:03:15.4 & $143.49$ & CH87  \\
 & & & G331.127$-$00.481 & C & 16:12:01.3 & $-52$:00:58.6 & $64.02$ &  \\
 & & & G331.146$-$00.480 & Q & 16:12:06.3 & $-52$:00:08.1 & $37.79$ &  \\
 & & & G331.156$-$00.391 & C & 16:11:45.6 & $-51$:55:50.4 & $141.66$ &  \\
 & & & G331.157$-$00.462 & Q & 16:12:04.6 & $-51$:58:53.2 & $30.64$ &  \\
 & & & G331.172$-$00.460 & C & 16:12:08.5 & $-51$:58:12.7 & $104.39$ &  \\
 & & & G331.182$-$00.541 & Q & 16:12:32.9 & $-52$:01:20.0 & $56.22$ &  \\
 & & & G331.195$-$00.469 & Q & 16:12:17.4 & $-51$:57:39.8 & $37.79$ &  \\
 & & & G331.256$-$00.480 & C & 16:12:37.7 & $-51$:55:38.3 & $348.58$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds1174 & 16:05:52.9 & $-50$:48:03.2 & G331.249+01.071 & G & 16:05:52.4 & $-50$:47:20.8 & $209.94$ &  \\
 & & & G331.344+01.055 & K & 16:06:23.2 & $-50$:44:14.1 & $251.85$ & CH87  \\
ch180 & 16:11:20.6 & $-51$:42:38.1 & G331.259$-$00.188 & K & 16:11:20.9 & $-51$:42:41.8 & $154.19$ & CH87  \\
 & & & G331.322$-$00.176 & C & 16:11:35.7 & $-51$:39:36.4 & $89.77$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds723 & 16:09:46.3 & $-51$:24:57.9 & G331.280+00.191 & C & 16:09:47.4 & $-51$:25:09.1 & $78.06$ &  \\
ch181 & 16:12:15.8 & $-51$:46:57.6 & G331.256$-$00.480 & C & 16:12:37.7 & $-51$:55:38.3 & $348.58$ &  \\
 & & & G331.334$-$00.389 & Q & 16:12:35.4 & $-51$:48:25.8 & $39.81$ &  \\
 & & & G331.338$-$00.365 & K & 16:12:30.3 & $-51$:47:14.1 & $208.23$ & CH87  \\
 & & & G331.341$-$00.268 & C & 16:12:05.4 & $-51$:42:52.0 & $164.41$ &  \\
 & & & G331.384$-$00.358 & G & 16:12:41.4 & $-51$:45:01.6 & $58.81$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds725 & 16:11:34.4 & $-51$:39:34.2 & G331.259$-$00.188 & K & 16:11:20.9 & $-51$:42:41.8 & $154.19$ & CH87  \\
 & & & G331.300$-$00.071 & C & 16:11:01.8 & $-51$:35:54.1 & $174.29$ &  \\
 & & & G331.322$-$00.176 & C & 16:11:35.7 & $-51$:39:36.4 & $89.77$ &  \\
 & & & G331.341$-$00.268 & C & 16:12:05.4 & $-51$:42:52.0 & $164.41$ &  \\
 & & & G331.367$-$00.143 & Q & 16:11:39.6 & $-51$:36:18.1 & $20.91$ &  \\
 & & & G331.398$-$00.182 & C & 16:11:58.6 & $-51$:36:43.9 & $37.32$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
ch182 & 16:11:01.6 & $-51$:31:11.7 & G331.300$-$00.071 & C & 16:11:01.8 & $-51$:35:54.1 & $174.29$ &  \\
 & & & G331.352+00.023 & Q & 16:10:51.7 & $-51$:29:37.4 & $35.97$ &  \\
 & & & G331.361$-$00.019 & K & 16:11:05.2 & $-51$:31:05.3 & $151.43$ & CH87  \\
 & & & G331.382+00.004 & G & 16:11:05.3 & $-51$:29:14.8 & $50.62$ &  \\
 & & & G331.412+00.011 & C & 16:11:11.9 & $-51$:27:43.3 & $60.32$ &  \\
shrds1175g & 16:06:02.7 & $-50$:39:43.5 & G331.344+01.055 & K & 16:06:23.2 & $-50$:44:14.1 & $251.85$ & CH87  \\
 & & & G331.359+01.158 & G & 16:06:01.3 & $-50$:39:02.4 & $124.17$ &  \\
shrds729 & 16:11:10.4 & $-51$:27:27.9 & G331.352+00.023 & Q & 16:10:51.7 & $-51$:29:37.4 & $35.97$ &  \\
 & & & G331.361$-$00.019 & K & 16:11:05.2 & $-51$:31:05.3 & $151.43$ & CH87  \\
 & & & G331.382+00.004 & G & 16:11:05.3 & $-51$:29:14.8 & $50.62$ &  \\
 & & & G331.412+00.011 & C & 16:11:11.9 & $-51$:27:43.3 & $60.32$ &  \\
 & & & G331.580$-$00.022 & G & 16:12:07.9 & $-51$:22:17.5 & $396.57$ &  \\
shrds731 & 16:12:50.8 & $-51$:43:36.4 & G331.338$-$00.365 & K & 16:12:30.3 & $-51$:47:14.1 & $208.23$ & CH87  \\
 & & & G331.378$-$00.386 & Q & 16:12:47.1 & $-51$:46:30.1 & $35.02$ &  \\
 & & & G331.384$-$00.358 & G & 16:12:41.4 & $-51$:45:01.6 & $58.81$ &  \\
 & & & G331.417$-$00.354 & C & 16:12:49.5 & $-51$:43:29.1 & $43.64$ &  \\
 & & & G331.427$-$00.372 & C & 16:12:57.2 & $-51$:43:52.0 & $35.35$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds732 & 16:12:41.1 & $-51$:37:26.9 & G331.436$-$00.259 & Q & 16:12:29.8 & $-51$:38:33.9 & $29.27$ &  \\
 & & & G331.468$-$00.262 & C & 16:12:39.7 & $-51$:37:23.6 & $62.68$ &  \\
 & & & G331.538$-$00.308 & C & 16:13:11.4 & $-51$:36:30.2 & $53.77$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds734 & 16:13:49.0 & $-51$:46:04.3 & G331.500$-$00.491 & C & 16:13:49.4 & $-51$:46:02.6 & $37.44$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds733 & 16:12:09.6 & $-51$:29:41.6 & G331.475$-$00.138 & Q & 16:12:08.7 & $-51$:31:39.0 & $26.16$ &  \\
 & & & G331.485$-$00.123 & Q & 16:12:07.7 & $-51$:30:36.5 & $26.16$ &  \\
 & & & G331.491$-$00.116 & C & 16:12:07.5 & $-51$:30:03.1 & $17.33$ &  \\
 & & & G331.520$-$00.076 & K & 16:12:05.1 & $-51$:27:05.6 & $153.20$ & CH87  \\
 & & & G331.546$-$00.154 & Q & 16:12:33.0 & $-51$:29:27.2 & $26.16$ &  \\
 & & & G331.559$-$00.128 & C & 16:12:29.7 & $-51$:27:46.3 & $60.73$ &  \\
 & & & G331.580$-$00.022 & G & 16:12:07.9 & $-51$:22:17.5 & $396.57$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
ch185 & 16:12:02.6 & $-51$:26:56.4 & G331.485$-$00.123 & Q & 16:12:07.7 & $-51$:30:36.5 & $26.16$ &  \\
 & & & G331.491$-$00.116 & C & 16:12:07.5 & $-51$:30:03.1 & $17.33$ &  \\
 & & & G331.520$-$00.076 & K & 16:12:05.1 & $-51$:27:05.6 & $153.20$ & CH87  \\
 & & & G331.559$-$00.128 & C & 16:12:29.7 & $-51$:27:46.3 & $60.73$ &  \\
 & & & G331.580$-$00.022 & G & 16:12:07.9 & $-51$:22:17.5 & $396.57$ &  \\
shrds735 & 16:13:11.1 & $-51$:36:21.4 & G331.468$-$00.262 & C & 16:12:39.7 & $-51$:37:23.6 & $62.68$ &  \\
 & & & G331.538$-$00.308 & C & 16:13:11.4 & $-51$:36:30.2 & $53.77$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds736 & 16:12:27.2 & $-51$:27:37.0 & G331.485$-$00.123 & Q & 16:12:07.7 & $-51$:30:36.5 & $26.16$ &  \\
 & & & G331.491$-$00.116 & C & 16:12:07.5 & $-51$:30:03.1 & $17.33$ &  \\
 & & & G331.520$-$00.076 & K & 16:12:05.1 & $-51$:27:05.6 & $153.20$ & CH87  \\
 & & & G331.546$-$00.154 & Q & 16:12:33.0 & $-51$:29:27.2 & $26.16$ &  \\
 & & & G331.559$-$00.128 & C & 16:12:29.7 & $-51$:27:46.3 & $60.73$ &  \\
 & & & G331.580$-$00.022 & G & 16:12:07.9 & $-51$:22:17.5 & $396.57$ &  \\
 & & & G331.604$-$00.110 & C & 16:12:37.6 & $-51$:25:07.5 & $44.04$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
shrds737 & 16:11:40.7 & $-51$:18:48.1 & G331.560+00.091 & C & 16:11:32.4 & $-51$:18:07.5 & $81.91$ &  \\
 & & & G331.580$-$00.022 & G & 16:12:07.9 & $-51$:22:17.5 & $396.57$ &  \\
shrds738 & 16:12:37.0 & $-51$:25:12.2 & G331.520$-$00.076 & K & 16:12:05.1 & $-51$:27:05.6 & $153.20$ & CH87  \\
 & & & G331.546$-$00.154 & Q & 16:12:33.0 & $-51$:29:27.2 & $26.16$ &  \\
 & & & G331.559$-$00.128 & C & 16:12:29.7 & $-51$:27:46.3 & $60.73$ &  \\
 & & & G331.580$-$00.022 & G & 16:12:07.9 & $-51$:22:17.5 & $396.57$ &  \\
 & & & G331.604$-$00.110 & C & 16:12:37.6 & $-51$:25:07.5 & $44.04$ &  \\
 & & & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
 & & & G331.667$-$00.093 & C & 16:12:50.9 & $-51$:21:49.7 & $99.01$ &  \\
shrds741 & 16:11:48.0 & $-51$:12:28.4 & G331.580$-$00.022 & G & 16:12:07.9 & $-51$:22:17.5 & $396.57$ &  \\
 & & & G331.653+00.128 & C & 16:11:49.0 & $-51$:12:43.9 & $105.12$ &  \\
 & & & G331.689+00.162 & Q & 16:11:50.2 & $-51$:09:46.0 & $52.54$ &  \\
shrds743 & 16:13:06.7 & $-51$:17:32.0 & G331.580$-$00.022 & G & 16:12:07.9 & $-51$:22:17.5 & $396.57$ &  \\
 & & & G331.667$-$00.093 & C & 16:12:50.9 & $-51$:21:49.7 & $99.01$ &  \\
 & & & G331.744$-$00.068 & C & 16:13:05.7 & $-51$:17:32.4 & $74.29$ &  \\
 & & & G331.786$-$00.133 & Q & 16:13:34.6 & $-51$:18:39.4 & $45.01$ &  \\
 & & & G331.797$-$00.148 & C & 16:13:41.8 & $-51$:18:52.5 & $146.95$ &  \\
 & & & G331.834$-$00.002 & C & 16:13:13.5 & $-51$:10:57.2 & $160.99$ &  \\
shrds744 & 16:12:35.4 & $-51$:11:16.4 & G331.760+00.064 & C & 16:12:35.7 & $-51$:11:08.7 & $109.70$ &  \\
 & & & G331.834$-$00.002 & C & 16:13:13.5 & $-51$:10:57.2 & $160.99$ &  \\
shrds745 & 16:13:50.2 & $-51$:18:42.2 & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
 & & & G331.786$-$00.133 & Q & 16:13:34.6 & $-51$:18:39.4 & $45.01$ &  \\
 & & & G331.797$-$00.148 & C & 16:13:41.8 & $-51$:18:52.5 & $146.95$ &  \\
 & & & G331.865$-$00.122 & C & 16:13:53.8 & $-51$:14:55.2 & $45.57$ &  \\
shrds746 & 16:13:11.1 & $-51$:11:41.8 & G331.760+00.064 & C & 16:12:35.7 & $-51$:11:08.7 & $109.70$ &  \\
 & & & G331.834$-$00.002 & C & 16:13:13.5 & $-51$:10:57.2 & $160.99$ &  \\
 & & & G331.864+00.059 & C & 16:13:06.0 & $-51$:07:05.2 & $38.12$ &  \\
shrds752 & 16:12:04.5 & $-50$:39:19.3 & G332.062+00.509 & C & 16:12:03.5 & $-50$:39:14.2 & $49.71$ &  \\
 & & & G332.070+00.500 & Q & 16:12:08.2 & $-50$:39:19.7 & $91.35$ &  \\
shrds753 & 16:16:20.5 & $-51$:18:15.7 & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
 & & & G332.092$-$00.422 & C & 16:16:16.1 & $-51$:18:30.4 & $81.56$ &  \\
 & & & G332.145$-$00.452 & K & 16:16:38.8 & $-51$:17:35.9 & $236.28$ & CH87  \\
ch186 & 16:16:38.2 & $-51$:17:15.1 & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
 & & & G332.092$-$00.422 & C & 16:16:16.1 & $-51$:18:30.4 & $81.56$ &  \\
 & & & G332.145$-$00.452 & K & 16:16:38.8 & $-51$:17:35.9 & $236.28$ & CH87  \\
shrds756 & 16:15:45.9 & $-50$:56:10.5 & G332.233$-$00.052 & Q & 16:15:17.2 & $-50$:56:39.8 & $42.34$ &  \\
 & & & G332.275$-$00.004 & C & 16:15:16.0 & $-50$:52:49.0 & $249.52$ &  \\
 & & & G332.291$-$00.092 & C & 16:15:43.7 & $-50$:55:58.7 & $30.27$ &  \\
 & & & G332.293$-$00.106 & C & 16:15:47.8 & $-50$:56:29.5 & $44.35$ &  \\
 & & & G332.340$-$00.115 & C & 16:16:03.1 & $-50$:54:55.8 & $39.68$ &  \\
 & & & G332.353$-$00.118 & Q & 16:16:07.4 & $-50$:54:30.7 & $16.20$ &  \\
 & & & G332.356$-$00.122 & Q & 16:16:09.5 & $-50$:54:35.5 & $16.20$ &  \\
shrds759 & 16:17:57.9 & $-51$:15:06.5 & G331.628$-$00.926 & C & 16:16:22.2 & $-51$:59:36.5 & $2790.92$ &  \\
 & & & G332.293$-$00.536 & C & 16:17:42.0 & $-51$:15:02.6 & $52.55$ &  \\
 & & & G332.311$-$00.567 & C & 16:17:55.4 & $-51$:15:39.3 & $112.54$ &  \\
 & & & G332.394$-$00.668 & C & 16:18:45.1 & $-51$:16:29.3 & $437.84$ &  \\
shrds763 & 16:15:32.1 & $-50$:44:22.5 & G332.382+00.080 & C & 16:15:23.4 & $-50$:44:44.9 & $93.10$ &  \\
 & & & G332.415+00.053 & C & 16:15:39.6 & $-50$:44:33.5 & $228.79$ &  \\
shrds764 & 16:18:06.0 & $-51$:08:30.4 & G332.394$-$00.668 & C & 16:18:45.1 & $-51$:16:29.3 & $437.84$ &  \\
 & & & G332.412$-$00.505 & C & 16:18:06.6 & $-51$:08:45.5 & $58.14$ &  \\
shrds766 & 16:15:52.6 & $-50$:44:01.1 & G332.382+00.080 & C & 16:15:23.4 & $-50$:44:44.9 & $93.10$ &  \\
 & & & G332.415+00.053 & C & 16:15:39.6 & $-50$:44:33.5 & $228.79$ &  \\
shrds767 & 16:16:50.1 & $-50$:53:10.9 & G332.395$-$00.182 & C & 16:16:35.9 & $-50$:55:31.8 & $115.71$ &  \\
 & & & G332.450$-$00.177 & C & 16:16:49.8 & $-50$:53:02.9 & $62.53$ &  \\
 & & & G332.469$-$00.132 & Q & 16:16:42.9 & $-50$:50:17.2 & $26.76$ &  \\
shrds770 & 16:15:26.3 & $-50$:29:58.2 & G332.551+00.257 & C & 16:15:23.3 & $-50$:30:04.3 & $103.94$ &  \\
shrds771 & 16:19:10.1 & $-51$:03:56.9 & G332.555$-$00.602 & Q & 16:19:11.5 & $-51$:06:53.9 & $21.35$ &  \\
 & & & G332.585$-$00.561 & C & 16:19:08.6 & $-51$:03:52.7 & $71.86$ &  \\
 & & & G332.620$-$00.570 & Q & 16:19:20.6 & $-51$:02:47.5 & $62.23$ &  \\
 & & & G332.657$-$00.622 & K & 16:19:44.7 & $-51$:03:29.0 & $218.84$ & CH87  \\
 & & & G332.762$-$00.595 & K & 16:20:06.0 & $-50$:57:53.9 & $411.03$ & CH87  \\
shrds1181 & 16:19:54.6 & $-51$:07:06.0 & G332.601$-$00.727 & C & 16:19:57.5 & $-51$:10:17.3 & $75.07$ &  \\
 & & & G332.633$-$00.683 & G & 16:19:54.5 & $-51$:07:05.0 & $78.31$ &  \\
 & & & G332.657$-$00.622 & K & 16:19:44.7 & $-51$:03:29.0 & $218.84$ & CH87  \\
 & & & G332.762$-$00.595 & K & 16:20:06.0 & $-50$:57:53.9 & $411.03$ & CH87  \\
shrds773 & 16:18:49.5 & $-50$:45:22.5 & G332.767$-$00.309 & C & 16:18:50.9 & $-50$:45:25.7 & $50.78$ &  \\
 & & & G332.786$-$00.242 & C & 16:18:38.2 & $-50$:41:45.5 & $50.78$ &  \\
shrds774 & 16:17:32.1 & $-50$:32:17.0 & G332.718$-$00.053 & Q & 16:17:30.0 & $-50$:36:30.3 & $25.20$ &  \\
 & & & G332.733$-$00.028 & Q & 16:17:27.3 & $-50$:34:46.6 & $19.89$ &  \\
 & & & G332.766$-$00.006 & C & 16:17:30.7 & $-50$:32:29.5 & $86.11$ &  \\
shrds775 & 16:18:39.0 & $-50$:41:42.6 & G332.767$-$00.309 & C & 16:18:50.9 & $-50$:45:25.7 & $50.78$ &  \\
 & & & G332.786$-$00.242 & C & 16:18:38.2 & $-50$:41:45.5 & $50.78$ &  \\
ch190 & 16:20:05.0 & $-50$:55:26.5 & G332.762$-$00.595 & K & 16:20:06.0 & $-50$:57:53.9 & $411.03$ & CH87  \\
 & & & G332.823$-$00.550 & C & 16:20:10.4 & $-50$:53:23.5 & $44.76$ &  \\
 & & & G332.833$-$00.569 & C & 16:20:18.1 & $-50$:53:46.6 & $44.76$ &  \\
 & & & G332.840$-$00.543 & C & 16:20:13.1 & $-50$:52:22.3 & $44.76$ &  \\
 & & & G332.861$-$00.573 & C & 16:20:26.9 & $-50$:52:46.9 & $74.41$ &  \\
shrds777 & 16:20:11.3 & $-50$:53:32.3 & G332.762$-$00.595 & K & 16:20:06.0 & $-50$:57:53.9 & $411.03$ & CH87  \\
 & & & G332.823$-$00.550 & C & 16:20:10.4 & $-50$:53:23.5 & $44.76$ &  \\
 & & & G332.833$-$00.569 & C & 16:20:18.1 & $-50$:53:46.6 & $44.76$ &  \\
 & & & G332.840$-$00.543 & C & 16:20:13.1 & $-50$:52:22.3 & $44.76$ &  \\
 & & & G332.861$-$00.573 & C & 16:20:26.9 & $-50$:52:46.9 & $74.41$ &  \\
shrds782 & 16:10:37.4 & $-49$:05:46.7 & G332.815+01.874 & Q & 16:09:42.9 & $-49$:08:29.5 & $497.00$ &  \\
 & & & G332.957+01.793 & C & 16:10:41.5 & $-49$:06:18.6 & $145.46$ &  \\
 & & & G333.053+01.748 & C & 16:11:18.3 & $-49$:04:20.4 & $551.13$ &  \\
 & & & G333.093+01.966 & K & 16:10:34.7 & $-48$:53:07.7 & $739.74$ & CH87  \\
ch191 & 16:15:00.5 & $-49$:49:10.8 & G332.964+00.771 & K & 16:15:02.0 & $-49$:50:39.2 & $72.92$ & CH87  \\
 & & & G332.978+00.773 & K & 16:15:05.3 & $-49$:49:59.9 & $235.37$ & CH87  \\
 & & & G333.005+00.770 & Q & 16:15:13.3 & $-49$:48:59.5 & $20.64$ &  \\
 & & & G333.008+00.723 & Q & 16:15:26.1 & $-49$:50:53.9 & $24.81$ &  \\
 & & & G333.016+00.739 & Q & 16:15:24.1 & $-49$:49:52.1 & $24.81$ &  \\
 & & & G333.016+00.761 & G & 16:15:18.5 & $-49$:48:55.6 & $36.97$ &  \\
 & & & G333.019+00.747 & Q & 16:15:23.0 & $-49$:49:25.1 & $24.81$ &  \\
 & & & G333.045+00.731 & Q & 16:15:34.1 & $-49$:49:02.2 & $90.26$ &  \\
shrds784 & 16:14:33.4 & $-49$:43:33.6 & G332.987+00.902 & C & 16:14:34.6 & $-49$:44:01.1 & $92.86$ &  \\
shrds785 & 16:21:14.8 & $-50$:49:25.2 & G332.990$-$00.619 & C & 16:21:13.9 & $-50$:49:16.2 & $167.80$ &  \\
 & & & G333.045$-$00.564 & Q & 16:21:13.9 & $-50$:44:35.7 & $41.86$ &  \\
shrds786 & 16:18:57.0 & $-50$:23:52.6 & G332.978$-$00.074 & C & 16:18:45.7 & $-50$:26:30.5 & $258.54$ &  \\
 & & & G333.029$-$00.066 & C & 16:18:57.3 & $-50$:24:00.7 & $38.95$ &  \\
 & & & G333.052+00.033 & C & 16:18:37.5 & $-50$:18:48.7 & $118.05$ &  \\
 & & & G333.173$-$00.068 & K & 16:19:36.4 & $-50$:18:02.2 & $279.46$ & CH87  \\
shrds788 & 16:18:37.4 & $-50$:18:42.6 & G332.978$-$00.074 & C & 16:18:45.7 & $-50$:26:30.5 & $258.54$ &  \\
 & & & G333.052+00.033 & C & 16:18:37.5 & $-50$:18:48.7 & $118.05$ &  \\
shrds789 & 16:21:00.8 & $-50$:39:26.7 & G333.011$-$00.441 & K & 16:20:32.0 & $-50$:40:49.3 & $137.51$ & W70  \\
 & & & G333.049$-$00.463 & Q & 16:20:48.1 & $-50$:40:08.9 & $24.59$ &  \\
 & & & G333.067$-$00.447 & G & 16:20:48.7 & $-50$:38:42.9 & $17.21$ &  \\
 & & & G333.068$-$00.443 & G & 16:20:47.8 & $-50$:38:28.7 & $17.21$ &  \\
 & & & G333.074$-$00.482 & C & 16:20:59.7 & $-50$:39:52.6 & $160.23$ &  \\
 & & & G333.080$-$00.413 & Q & 16:20:43.2 & $-50$:36:43.1 & $22.09$ &  \\
 & & & G333.085$-$00.479 & G & 16:21:02.0 & $-50$:39:18.5 & $57.40$ &  \\
 & & & G333.095$-$00.460 & G & 16:20:59.6 & $-50$:38:03.8 & $52.76$ &  \\
 & & & G333.108$-$00.507 & G & 16:21:15.5 & $-50$:39:29.6 & $72.40$ &  \\
 & & & G333.129$-$00.439 & K & 16:21:03.1 & $-50$:35:44.4 & $112.55$ & CH87  \\
shrds792 & 16:19:41.5 & $-50$:21:46.4 & G333.113$-$00.141 & C & 16:19:39.6 & $-50$:23:41.1 & $108.36$ &  \\
 & & & G333.164$-$00.100 & Q & 16:19:42.6 & $-50$:19:48.9 & $26.22$ &  \\
 & & & G333.173$-$00.068 & K & 16:19:36.4 & $-50$:18:02.2 & $279.46$ & CH87  \\
shrds793 & 16:20:41.7 & $-50$:30:36.6 & G333.093$-$00.370 & C & 16:20:35.1 & $-50$:34:18.9 & $59.61$ &  \\
 & & & G333.107$-$00.398 & Q & 16:20:46.3 & $-50$:34:55.6 & $30.41$ &  \\
 & & & G333.134$-$00.390 & Q & 16:20:51.3 & $-50$:33:25.1 & $41.90$ &  \\
 & & & G333.149$-$00.338 & C & 16:20:41.6 & $-50$:30:35.8 & $111.64$ &  \\
 & & & G333.211$-$00.394 & G & 16:21:13.0 & $-50$:30:20.2 & $100.49$ &  \\
 & & & G333.215$-$00.298 & G & 16:20:48.7 & $-50$:26:06.6 & $305.73$ &  \\
shrds794 & 16:19:23.8 & $-50$:09:03.9 & G333.255+00.065 & C & 16:19:23.5 & $-50$:08:55.9 & $120.14$ &  \\
 & & & G333.265+00.041 & C & 16:19:32.5 & $-50$:09:32.3 & $24.73$ &  \\
ch194 & 16:21:28.7 & $-50$:25:57.7 & G333.211$-$00.394 & G & 16:21:13.0 & $-50$:30:20.2 & $100.49$ &  \\
 & & & G333.215$-$00.298 & G & 16:20:48.7 & $-50$:26:06.6 & $305.73$ &  \\
 & & & G333.227$-$00.405 & Q & 16:21:20.3 & $-50$:30:08.9 & $20.04$ &  \\
 & & & G333.245$-$00.487 & G & 16:21:46.9 & $-50$:32:50.6 & $322.19$ &  \\
 & & & G333.267$-$00.439 & Q & 16:21:40.0 & $-50$:29:53.0 & $47.98$ &  \\
 & & & G333.286$-$00.374 & Q & 16:21:27.8 & $-50$:26:19.9 & $17.99$ &  \\
 & & & G333.288$-$00.399 & K & 16:21:34.9 & $-50$:27:17.5 & $86.78$ & CH87  \\
 & & & G333.312$-$00.362 & K & 16:21:31.6 & $-50$:24:43.1 & $79.88$ & CH87  \\
 & & & G333.314$-$00.350 & Q & 16:21:28.9 & $-50$:24:07.0 & $22.30$ &  \\
 & & & G333.326$-$00.355 & Q & 16:21:33.5 & $-50$:23:50.4 & $29.33$ &  \\
shrds796 & 16:10:15.9 & $-48$:30:32.5 & G333.315+02.273 & C & 16:10:18.1 & $-48$:30:35.3 & $145.46$ &  \\
shrds799 & 16:21:19.3 & $-50$:09:40.1 & G333.467$-$00.159 & C & 16:21:18.9 & $-50$:09:31.3 & $93.89$ &  \\
 & & & G333.508$-$00.138 & G & 16:21:24.2 & $-50$:06:52.8 & $203.31$ &  \\
shrds800 & 16:22:03.6 & $-50$:12:51.3 & G333.497$-$00.275 & C & 16:21:57.6 & $-50$:13:10.1 & $110.65$ &  \\
 & & & G333.531$-$00.303 & G & 16:22:14.1 & $-50$:12:55.6 & $85.86$ &  \\
 & & & G333.534$-$00.383 & C & 16:22:36.0 & $-50$:16:09.9 & $238.34$ &  \\
 & & & G333.563$-$00.216 & G & 16:21:59.4 & $-50$:07:52.0 & $52.26$ &  \\
 & & & G333.568$-$00.317 & Q & 16:22:27.7 & $-50$:11:57.4 & $28.74$ &  \\
 & & & G333.594$-$00.291 & G & 16:22:27.5 & $-50$:09:43.7 & $267.88$ &  \\
 & & & G333.627$-$00.199 & K & 16:22:11.8 & $-50$:04:25.5 & $270.66$ & CH87  \\
shrds801 & 16:22:36.0 & $-50$:16:29.7 & G333.531$-$00.303 & G & 16:22:14.1 & $-50$:12:55.6 & $85.86$ &  \\
 & & & G333.534$-$00.383 & C & 16:22:36.0 & $-50$:16:09.9 & $238.34$ &  \\
 & & & G333.594$-$00.291 & G & 16:22:27.5 & $-50$:09:43.7 & $267.88$ &  \\
shrds802 & 16:20:45.2 & $-49$:55:54.4 & G333.575+00.098 & Q & 16:20:39.7 & $-49$:54:00.1 & $28.51$ &  \\
 & & & G333.580+00.058 & C & 16:20:51.6 & $-49$:55:30.4 & $292.98$ &  \\
 & & & G333.586+00.071 & Q & 16:20:50.0 & $-49$:54:43.2 & $28.51$ &  \\
 & & & G333.603$-$00.009 & Q & 16:21:15.3 & $-49$:57:22.5 & $74.06$ &  \\
caswell19 & 16:22:10.7 & $-50$:05:56.3 & G333.508$-$00.138 & G & 16:21:24.2 & $-50$:06:52.8 & $203.31$ &  \\
 & & & G333.563$-$00.216 & G & 16:21:59.4 & $-50$:07:52.0 & $52.26$ &  \\
 & & & G333.593$-$00.090 & K & 16:21:34.1 & $-50$:01:15.2 & $205.38$ & W70  \\
 & & & G333.594$-$00.291 & G & 16:22:27.5 & $-50$:09:43.7 & $267.88$ &  \\
 & & & G333.627$-$00.199 & K & 16:22:11.8 & $-50$:04:25.5 & $270.66$ & CH87  \\
 & & & G333.668$-$00.122 & G & 16:22:02.2 & $-49$:59:24.7 & $199.35$ &  \\
ch196 & 16:22:09.9 & $-50$:05:33.4 & G333.508$-$00.138 & G & 16:21:24.2 & $-50$:06:52.8 & $203.31$ &  \\
 & & & G333.563$-$00.216 & G & 16:21:59.4 & $-50$:07:52.0 & $52.26$ &  \\
 & & & G333.593$-$00.090 & K & 16:21:34.1 & $-50$:01:15.2 & $205.38$ & W70  \\
 & & & G333.594$-$00.291 & G & 16:22:27.5 & $-50$:09:43.7 & $267.88$ &  \\
 & & & G333.627$-$00.199 & K & 16:22:11.8 & $-50$:04:25.5 & $270.66$ & CH87  \\
 & & & G333.668$-$00.122 & G & 16:22:02.2 & $-49$:59:24.7 & $199.35$ &  \\
shrds1200 & 16:21:53.5 & $-49$:58:00.3 & G333.593$-$00.090 & K & 16:21:34.1 & $-50$:01:15.2 & $205.38$ & W70  \\
 & & & G333.618$-$00.037 & Q & 16:21:26.6 & $-49$:57:55.6 & $66.35$ &  \\
 & & & G333.627$-$00.199 & K & 16:22:11.8 & $-50$:04:25.5 & $270.66$ & CH87  \\
 & & & G333.668$-$00.122 & G & 16:22:02.2 & $-49$:59:24.7 & $199.35$ &  \\
 & & & G333.719$-$00.027 & C & 16:21:50.8 & $-49$:53:14.6 & $45.71$ &  \\
shrds803 & 16:20:09.0 & $-49$:36:11.6 & G333.725+00.364 & C & 16:20:10.0 & $-49$:36:21.7 & $100.75$ &  \\
 & & & G333.757+00.360 & C & 16:20:19.4 & $-49$:35:09.9 & $61.03$ &  \\
shrds804 & 16:23:41.0 & $-50$:09:24.5 & G333.681$-$00.441 & K & 16:23:30.3 & $-50$:12:21.1 & $65.97$ & CH87  \\
 & & & G333.683$-$00.512 & K & 16:23:49.7 & $-50$:15:15.3 & $240.72$ & CH87  \\
 & & & G333.733$-$00.429 & C & 16:23:40.8 & $-50$:09:37.3 & $59.53$ &  \\
shrds806 & 16:22:30.4 & $-49$:39:12.3 & G333.962+00.063 & C & 16:22:30.8 & $-49$:39:06.1 & $67.49$ &  \\
 & & & G334.022+00.106 & C & 16:22:35.1 & $-49$:34:42.5 & $119.37$ &  \\
shrds807 & 16:22:28.8 & $-49$:35:02.8 & G333.962+00.063 & C & 16:22:30.8 & $-49$:39:06.1 & $67.49$ &  \\
 & & & G334.022+00.106 & C & 16:22:35.1 & $-49$:34:42.5 & $119.37$ &  \\
 & & & G334.106+00.109 & C & 16:22:56.4 & $-49$:31:02.5 & $130.21$ &  \\
shrds810 & 16:22:57.3 & $-49$:31:51.1 & G334.022+00.106 & C & 16:22:35.1 & $-49$:34:42.5 & $119.37$ &  \\
 & & & G334.106+00.109 & C & 16:22:56.4 & $-49$:31:02.5 & $130.21$ &  \\
 & & & G334.221+00.065 & K & 16:23:37.9 & $-49$:27:59.8 & $293.86$ & CH87  \\
shrds811 & 16:22:59.9 & $-49$:23:34.6 & G334.202+00.193 & C & 16:22:59.4 & $-49$:23:23.8 & $83.82$ &  \\
 & & & G334.221+00.065 & K & 16:23:37.9 & $-49$:27:59.8 & $293.86$ & CH87  \\
shrds814 & 16:24:14.8 & $-49$:23:32.9 & G334.221+00.065 & K & 16:23:37.9 & $-49$:27:59.8 & $293.86$ & CH87  \\
 & & & G334.341+00.045 & C & 16:24:14.2 & $-49$:23:42.3 & $52.80$ &  \\
shrds815 & 16:27:00.5 & $-49$:44:53.7 & G334.400$-$00.523 & C & 16:26:60.0 & $-49$:44:58.9 & $61.63$ &  \\
 & & & G334.440$-$00.575 & Q & 16:27:24.2 & $-49$:45:25.2 & $18.39$ &  \\
 & & & G334.444$-$00.504 & C & 16:27:06.1 & $-49$:42:15.5 & $238.15$ &  \\
shrds817 & 16:25:43.8 & $-49$:31:25.1 & G334.412$-$00.230 & Q & 16:25:45.1 & $-49$:32:13.0 & $26.94$ &  \\
 & & & G334.420$-$00.217 & C & 16:25:43.7 & $-49$:31:19.2 & $43.46$ &  \\
 & & & G334.422$-$00.251 & C & 16:25:53.2 & $-49$:32:39.5 & $50.95$ &  \\
 & & & G334.468$-$00.229 & C & 16:25:59.1 & $-49$:29:44.3 & $230.19$ &  \\
shrds818 & 16:23:20.6 & $-49$:07:59.5 & G334.427+00.331 & C & 16:23:21.6 & $-49$:07:59.0 & $53.25$ &  \\
shrds822 & 16:25:24.9 & $-49$:19:47.3 & G334.525$-$00.047 & C & 16:25:25.7 & $-49$:19:40.1 & $49.98$ &  \\
g334.591$-$01.105 & 16:30:25.6 & $-50$:00:46.9 & G334.591$-$01.105 & C & 16:30:25.7 & $-50$:00:47.6 & $50.34$ &  \\
shrds824 & 16:30:25.3 & $-50$:00:44.4 & G334.591$-$01.105 & C & 16:30:25.7 & $-50$:00:47.6 & $50.34$ &  \\
shrds825 & 16:23:50.9 & $-48$:54:05.4 & G334.571+00.471 & C & 16:23:22.1 & $-48$:55:54.6 & $306.26$ &  \\
 & & & G334.646+00.442 & C & 16:23:48.9 & $-48$:53:56.1 & $111.90$ &  \\
shrds826 & 16:27:04.0 & $-49$:23:30.0 & G334.659$-$00.286 & C & 16:27:03.3 & $-49$:23:53.1 & $99.81$ &  \\
ch201 & 16:28:58.7 & $-49$:37:17.7 & G334.721$-$00.653 & K & 16:28:57.1 & $-49$:36:28.2 & $105.60$ & CH87  \\
caswell20 & 16:28:57.8 & $-49$:36:29.5 & G334.721$-$00.653 & K & 16:28:57.1 & $-49$:36:28.2 & $105.60$ & CH87  \\
shrds828 & 16:26:26.5 & $-49$:07:28.5 & G334.698$-$00.090 & K & 16:26:21.7 & $-49$:14:03.7 & $157.89$ & CH87  \\
 & & & G334.774$-$00.023 & C & 16:26:23.3 & $-49$:07:58.3 & $122.72$ &  \\
shrds833 & 16:27:20.5 & $-49$:00:19.6 & G334.976$-$00.047 & C & 16:27:21.2 & $-49$:00:16.9 & $50.82$ &  \\
shrds834 & 16:27:55.1 & $-49$:02:23.0 & G335.006$-$00.143 & C & 16:27:53.9 & $-49$:02:56.3 & $93.49$ &  \\
 & & & G335.013$-$00.170 & Q & 16:28:03.0 & $-49$:03:47.3 & $24.61$ &  \\
 & & & G335.058$-$00.130 & Q & 16:28:03.8 & $-49$:00:10.6 & $82.54$ &  \\
shrds835 & 16:29:02.9 & $-49$:00:13.8 & G335.141$-$00.261 & Q & 16:28:59.3 & $-49$:01:59.1 & $54.78$ &  \\
 & & & G335.168$-$00.240 & C & 16:29:00.7 & $-48$:59:57.9 & $105.60$ &  \\
shrds836 & 16:29:48.2 & $-49$:04:53.0 & G335.195$-$00.385 & C & 16:29:45.8 & $-49$:04:46.2 & $51.78$ &  \\
 & & & G335.223$-$00.345 & Q & 16:29:42.3 & $-49$:01:54.1 & $35.82$ &  \\
shrds837 & 16:26:50.1 & $-48$:25:52.4 & G335.326+00.409 & C & 16:26:50.2 & $-48$:26:08.2 & $100.48$ &  \\
shrds840 & 16:29:09.4 & $-48$:35:38.0 & G335.469+00.027 & C & 16:29:05.9 & $-48$:35:49.5 & $104.49$ &  \\
 & & & G335.499$-$00.142 & C & 16:29:57.9 & $-48$:41:30.6 & $355.16$ &  \\
shrds841 & 16:30:34.2 & $-48$:40:54.4 & G335.499$-$00.142 & C & 16:29:57.9 & $-48$:41:30.6 & $355.16$ &  \\
 & & & G335.510$-$00.244 & Q & 16:30:27.7 & $-48$:45:15.5 & $34.41$ &  \\
 & & & G335.579$-$00.209 & C & 16:30:35.5 & $-48$:40:46.8 & $78.30$ &  \\
shrds843 & 16:35:05.9 & $-48$:45:57.4 & G336.026$-$00.817 & C & 16:35:08.3 & $-48$:45:59.5 & $85.16$ &  \\
shrds845 & 16:32:07.9 & $-48$:12:16.8 & G336.086$-$00.074 & C & 16:32:05.8 & $-48$:13:05.8 & $89.61$ &  \\
 & & & G336.097+00.005 & C & 16:31:47.6 & $-48$:09:21.7 & $219.40$ &  \\
shrds849 & 16:38:36.0 & $-48$:55:10.4 & G336.295$-$01.341 & C & 16:38:36.0 & $-48$:55:06.1 & $119.47$ &  \\
 & & & G336.317$-$01.223 & C & 16:38:09.1 & $-48$:49:26.1 & $370.94$ &  \\
shrds852 & 16:32:52.1 & $-47$:57:20.0 & G336.367$-$00.003 & C & 16:32:55.9 & $-47$:57:50.8 & $34.76$ &  \\
 & & & G336.446$-$00.198 & K & 16:34:06.3 & $-48$:02:17.8 & $623.89$ & CH87  \\
 & & & G336.455+00.042 & K & 16:33:05.4 & $-47$:52:07.5 & $197.00$ & CH87  \\
shrds853 & 16:34:13.1 & $-48$:06:11.8 & G336.410$-$00.257 & C & 16:34:13.2 & $-48$:06:18.0 & $22.51$ &  \\
 & & & G336.418$-$00.249 & K & 16:34:13.1 & $-48$:05:38.0 & $105.60$ & CH87  \\
 & & & G336.446$-$00.198 & K & 16:34:06.3 & $-48$:02:17.8 & $623.89$ & CH87  \\
caswell21 & 16:40:00.3 & $-48$:51:37.3 & G336.491$-$01.474 & K & 16:39:59.6 & $-48$:51:40.6 & $93.15$ & CH87  \\
 & & & G336.524$-$01.466 & Q & 16:40:05.4 & $-48$:49:52.8 & $49.50$ &  \\
 & & & G336.551$-$01.422 & Q & 16:39:59.9 & $-48$:46:55.3 & $49.29$ &  \\
 & & & G336.789$-$01.726 & G & 16:42:20.5 & $-48$:48:17.3 & $1540.11$ &  \\
ch209 & 16:40:06.2 & $-48$:50:47.9 & G336.491$-$01.474 & K & 16:39:59.6 & $-48$:51:40.6 & $93.15$ & CH87  \\
 & & & G336.524$-$01.466 & Q & 16:40:05.4 & $-48$:49:52.8 & $49.50$ &  \\
 & & & G336.551$-$01.422 & Q & 16:39:59.9 & $-48$:46:55.3 & $49.29$ &  \\
 & & & G336.789$-$01.726 & G & 16:42:20.5 & $-48$:48:17.3 & $1540.11$ &  \\
shrds854 & 16:33:06.5 & $-47$:45:54.5 & G336.455+00.042 & K & 16:33:05.4 & $-47$:52:07.5 & $197.00$ & CH87  \\
 & & & G336.518+00.119 & C & 16:33:00.7 & $-47$:46:13.5 & $186.70$ &  \\
 & & & G336.585+00.019 & C & 16:33:43.2 & $-47$:47:21.7 & $132.52$ &  \\
shrds855 & 16:40:00.1 & $-48$:46:56.9 & G336.491$-$01.474 & K & 16:39:59.6 & $-48$:51:40.6 & $93.15$ & CH87  \\
 & & & G336.524$-$01.466 & Q & 16:40:05.4 & $-48$:49:52.8 & $49.50$ &  \\
 & & & G336.551$-$01.422 & Q & 16:39:59.9 & $-48$:46:55.3 & $49.29$ &  \\
 & & & G336.789$-$01.726 & G & 16:42:20.5 & $-48$:48:17.3 & $1540.11$ &  \\
shrds857 & 16:33:43.4 & $-47$:47:04.5 & G336.518+00.119 & C & 16:33:00.7 & $-47$:46:13.5 & $186.70$ &  \\
 & & & G336.585+00.019 & C & 16:33:43.2 & $-47$:47:21.7 & $132.52$ &  \\
 & & & G336.753+00.097 & K & 16:34:03.4 & $-47$:36:47.2 & $410.12$ & CH87  \\
shrds1204 & 16:34:38.4 & $-47$:49:37.9 & G336.446$-$00.198 & K & 16:34:06.3 & $-48$:02:17.8 & $623.89$ & CH87  \\
 & & & G336.652$-$00.117 & C & 16:34:35.0 & $-47$:49:54.9 & $95.46$ &  \\
 & & & G336.689$-$00.085 & Q & 16:34:35.7 & $-47$:47:00.3 & $23.48$ &  \\
 & & & G336.694$-$00.095 & Q & 16:34:39.6 & $-47$:47:12.1 & $23.91$ &  \\
 & & & G336.700$-$00.076 & Q & 16:34:36.0 & $-47$:46:09.5 & $28.49$ &  \\
 & & & G336.703$-$00.099 & Q & 16:34:42.7 & $-47$:46:57.1 & $16.67$ &  \\
shrds1205 & 16:33:28.2 & $-47$:30:14.0 & G336.753+00.097 & K & 16:34:03.4 & $-47$:36:47.2 & $410.12$ & CH87  \\
 & & & G336.766+00.243 & C & 16:33:28.3 & $-47$:30:14.7 & $50.68$ &  \\
shrds1209 & 16:34:22.4 & $-47$:28:38.3 & G336.753+00.097 & K & 16:34:03.4 & $-47$:36:47.2 & $410.12$ & CH87  \\
 & & & G336.874+00.139 & G & 16:34:21.4 & $-47$:29:42.6 & $143.62$ &  \\
 & & & G336.888+00.057 & G & 16:34:46.3 & $-47$:32:25.7 & $105.60$ &  \\
 & & & G336.922+00.062 & G & 16:34:53.2 & $-47$:30:44.4 & $89.08$ &  \\
shrds1212 & 16:34:59.4 & $-47$:33:38.5 & G336.753+00.097 & K & 16:34:03.4 & $-47$:36:47.2 & $410.12$ & CH87  \\
 & & & G336.854$-$00.018 & G & 16:34:57.9 & $-47$:36:59.8 & $146.00$ &  \\
 & & & G336.879+00.000 & Q & 16:34:59.0 & $-47$:35:08.4 & $31.27$ &  \\
 & & & G336.888+00.057 & G & 16:34:46.3 & $-47$:32:25.7 & $105.60$ &  \\
 & & & G336.900$-$00.033 & C & 16:35:12.9 & $-47$:35:34.4 & $26.38$ &  \\
 & & & G336.915$-$00.026 & Q & 16:35:14.6 & $-47$:34:36.8 & $21.44$ &  \\
 & & & G336.922+00.062 & G & 16:34:53.2 & $-47$:30:44.4 & $89.08$ &  \\
shrds862 & 16:35:19.9 & $-47$:30:23.5 & G336.915$-$00.026 & Q & 16:35:14.6 & $-47$:34:36.8 & $21.44$ &  \\
 & & & G336.922+00.062 & G & 16:34:53.2 & $-47$:30:44.4 & $89.08$ &  \\
 & & & G336.969$-$00.013 & Q & 16:35:24.1 & $-47$:31:41.2 & $17.32$ &  \\
 & & & G336.970$-$00.051 & Q & 16:35:34.5 & $-47$:33:12.5 & $33.59$ &  \\
 & & & G336.978$-$00.007 & C & 16:35:24.8 & $-47$:31:03.6 & $11.58$ &  \\
 & & & G336.986$-$00.006 & C & 16:35:26.3 & $-47$:30:38.6 & $17.58$ &  \\
 & & & G336.990$-$00.021 & C & 16:35:31.4 & $-47$:31:06.3 & $28.51$ &  \\
 & & & G336.994$-$00.028 & C & 16:35:34.0 & $-47$:31:11.4 & $17.99$ &  \\
 & & & G337.001$-$00.030 & Q & 16:35:36.3 & $-47$:30:57.9 & $22.86$ &  \\
 & & & G337.046+00.030 & Q & 16:35:31.4 & $-47$:26:33.9 & $23.82$ &  \\
 & & & G337.046$-$00.001 & Q & 16:35:39.5 & $-47$:27:48.8 & $27.56$ &  \\
shrds864 & 16:36:09.3 & $-47$:37:06.3 & G336.919$-$00.188 & K & 16:35:58.0 & $-47$:40:58.7 & $191.21$ & W70  \\
 & & & G336.984$-$00.183 & C & 16:36:12.4 & $-47$:37:54.5 & $45.19$ &  \\
shrds865 & 16:34:01.1 & $-47$:16:20.6 & G337.004+00.322 & C & 16:34:05.2 & $-47$:16:34.0 & $53.15$ &  \\
shrds866 & 16:40:38.8 & $-48$:15:55.3 & G337.009$-$01.159 & C & 16:40:38.8 & $-48$:15:54.8 & $67.82$ &  \\
shrds867 & 16:40:02.7 & $-48$:04:15.4 & G337.091$-$00.965 & C & 16:40:06.0 & $-48$:04:30.0 & $159.35$ &  \\
 & & & G337.113$-$01.049 & C & 16:40:34.1 & $-48$:06:48.8 & $104.74$ &  \\
shrds868 & 16:40:34.0 & $-48$:06:52.5 & G337.091$-$00.965 & C & 16:40:06.0 & $-48$:04:30.0 & $159.35$ &  \\
 & & & G337.113$-$01.049 & C & 16:40:34.1 & $-48$:06:48.8 & $104.74$ &  \\
shrds869 & 16:36:19.5 & $-47$:24:14.3 & G337.097$-$00.045 & Q & 16:36:03.2 & $-47$:27:19.2 & $33.08$ &  \\
 & & & G337.138+00.008 & Q & 16:35:59.0 & $-47$:23:20.6 & $33.77$ &  \\
 & & & G337.170$-$00.059 & C & 16:36:24.2 & $-47$:24:37.8 & $35.25$ &  \\
 & & & G337.177$-$00.062 & C & 16:36:26.8 & $-47$:24:28.1 & $28.86$ &  \\
 & & & G337.188$-$00.060 & C & 16:36:28.8 & $-47$:23:52.8 & $28.86$ &  \\
 & & & G337.195$-$00.060 & C & 16:36:30.5 & $-47$:23:34.5 & $28.86$ &  \\
shrds870 & 16:37:07.3 & $-47$:25:14.9 & G337.253$-$00.165 & C & 16:37:12.0 & $-47$:25:14.6 & $59.25$ &  \\
 & & & G337.260$-$00.150 & Q & 16:37:09.6 & $-47$:24:18.1 & $13.94$ &  \\
 & & & G337.281$-$00.163 & C & 16:37:18.1 & $-47$:23:54.9 & $30.12$ &  \\
 & & & G337.285$-$00.113 & C & 16:37:05.9 & $-47$:21:43.0 & $57.15$ &  \\
 & & & G337.304$-$00.142 & C & 16:37:17.9 & $-47$:22:01.1 & $85.64$ &  \\
shrds871 & 16:36:02.5 & $-47$:12:36.5 & G337.286+00.113 & C & 16:36:07.0 & $-47$:12:34.0 & $105.60$ &  \\
 & & & G337.327+00.053 & Q & 16:36:32.4 & $-47$:13:10.3 & $57.30$ &  \\
shrds875 & 16:38:51.0 & $-47$:26:44.7 & G337.367$-$00.402 & Q & 16:38:41.6 & $-47$:29:40.1 & $22.37$ &  \\
 & & & G337.377$-$00.389 & Q & 16:38:40.6 & $-47$:28:42.6 & $22.37$ &  \\
 & & & G337.392$-$00.401 & Q & 16:38:47.2 & $-47$:28:30.4 & $22.37$ &  \\
 & & & G337.404$-$00.404 & C & 16:38:50.9 & $-47$:28:06.2 & $38.72$ &  \\
 & & & G337.412$-$00.401 & Q & 16:38:51.9 & $-47$:27:36.8 & $22.37$ &  \\
 & & & G337.428$-$00.401 & C & 16:38:55.7 & $-47$:26:53.3 & $58.62$ &  \\
 & & & G337.439$-$00.397 & Q & 16:38:57.3 & $-47$:26:15.0 & $22.37$ &  \\
 & & & G337.453$-$00.363 & C & 16:38:51.6 & $-47$:24:15.4 & $95.16$ &  \\
 & & & G337.496$-$00.258 & K & 16:38:33.9 & $-47$:18:06.8 & $335.50$ & CH87  \\
shrds878 & 16:39:39.2 & $-47$:28:37.3 & G337.487$-$00.534 & C & 16:39:44.8 & $-47$:29:32.7 & $83.82$ &  \\
 & & & G337.515$-$00.543 & Q & 16:39:53.8 & $-47$:28:39.6 & $136.45$ &  \\
ch214 & 16:38:58.6 & $-47$:17:40.0 & G337.496$-$00.258 & K & 16:38:33.9 & $-47$:18:06.8 & $335.50$ & CH87  \\
 & & & G337.595$-$00.366 & Q & 16:39:25.9 & $-47$:18:01.9 & $31.35$ &  \\
shrds879 & 16:42:33.1 & $-47$:47:06.2 & G337.474$-$01.054 & Q & 16:42:00.8 & $-47$:50:48.9 & $168.07$ &  \\
 & & & G337.580$-$01.081 & Q & 16:42:32.9 & $-47$:47:04.7 & $86.88$ &  \\
shrds880 & 16:38:08.0 & $-47$:04:57.8 & G337.583$-$00.044 & C & 16:37:58.2 & $-47$:05:38.8 & $95.77$ &  \\
 & & & G337.584$-$00.069 & Q & 16:38:05.2 & $-47$:06:37.9 & $26.51$ &  \\
 & & & G337.608$-$00.047 & Q & 16:38:05.1 & $-47$:04:40.7 & $29.22$ &  \\
 & & & G337.617$-$00.065 & C & 16:38:11.7 & $-47$:04:58.5 & $49.58$ &  \\
 & & & G337.652$-$00.050 & K & 16:38:16.2 & $-47$:02:50.0 & $197.83$ & CH87  \\
shrds881 & 16:37:49.0 & $-46$:58:30.3 & G337.593+00.096 & Q & 16:37:24.0 & $-46$:59:35.3 & $22.03$ &  \\
 & & & G337.652$-$00.050 & K & 16:38:16.2 & $-47$:02:50.0 & $197.83$ & CH87  \\
 & & & G337.664+00.049 & C & 16:37:53.1 & $-46$:58:19.5 & $102.49$ &  \\
 & & & G337.709+00.091 & C & 16:37:52.8 & $-46$:54:38.5 & $68.90$ &  \\
 & & & G337.754+00.057 & C & 16:38:12.2 & $-46$:53:59.2 & $203.32$ &  \\
shrds883 & 16:38:50.0 & $-47$:06:57.2 & G337.652$-$00.050 & K & 16:38:16.2 & $-47$:02:50.0 & $197.83$ & CH87  \\
 & & & G337.653$-$00.180 & Q & 16:38:50.6 & $-47$:08:00.5 & $19.92$ &  \\
 & & & G337.658$-$00.162 & C & 16:38:46.9 & $-47$:07:01.8 & $93.26$ &  \\
 & & & G337.660$-$00.183 & Q & 16:38:53.0 & $-47$:07:47.9 & $19.92$ &  \\
 & & & G337.665$-$00.176 & C & 16:38:52.4 & $-47$:07:18.4 & $19.92$ &  \\
 & & & G337.671$-$00.195 & Q & 16:38:58.7 & $-47$:07:47.4 & $19.92$ &  \\
shrds884 & 16:39:38.9 & $-47$:12:36.1 & G337.684$-$00.343 & C & 16:39:40.7 & $-47$:13:06.7 & $162.52$ &  \\
shrds885 & 16:38:25.5 & $-47$:00:33.2 & G337.652$-$00.050 & K & 16:38:16.2 & $-47$:02:50.0 & $197.83$ & CH87  \\
 & & & G337.696$-$00.070 & Q & 16:38:31.6 & $-47$:01:38.7 & $28.34$ &  \\
 & & & G337.705$-$00.059 & C & 16:38:31.0 & $-47$:00:49.2 & $67.52$ &  \\
 & & & G337.754+00.057 & C & 16:38:12.2 & $-46$:53:59.2 & $203.32$ &  \\
shrds886 & 16:37:57.9 & $-46$:55:01.6 & G337.664+00.049 & C & 16:37:53.1 & $-46$:58:19.5 & $102.49$ &  \\
 & & & G337.709+00.091 & C & 16:37:52.8 & $-46$:54:38.5 & $68.90$ &  \\
 & & & G337.754+00.057 & C & 16:38:12.2 & $-46$:53:59.2 & $203.32$ &  \\
shrds888 & 16:38:23.4 & $-46$:53:03.2 & G337.754+00.057 & C & 16:38:12.2 & $-46$:53:59.2 & $203.32$ &  \\
 & & & G337.827+00.056 & C & 16:38:29.6 & $-46$:50:46.3 & $135.53$ &  \\
shrds1218 & 16:38:32.2 & $-46$:47:09.0 & G337.827+00.056 & C & 16:38:29.6 & $-46$:50:46.3 & $135.53$ &  \\
 & & & G337.877+00.091 & C & 16:38:32.2 & $-46$:47:08.6 & $27.41$ &  \\
shrds1233 & 16:39:33.8 & $-46$:55:26.4 & G337.876$-$00.133 & C & 16:39:30.4 & $-46$:56:07.4 & $137.56$ &  \\
 & & & G337.920$-$00.158 & Q & 16:39:47.4 & $-46$:55:09.8 & $35.87$ &  \\
 & & & G337.926$-$00.133 & Q & 16:39:42.2 & $-46$:53:53.7 & $16.13$ &  \\
 & & & G338.003$-$00.121 & K & 16:39:57.0 & $-46$:49:58.3 & $276.32$ & CH87  \\
ch216 & 16:41:18.0 & $-47$:06:31.3 & G337.922$-$00.463 & K & 16:41:08.1 & $-47$:07:11.5 & $108.99$ & CH87  \\
 & & & G337.957$-$00.474 & K & 16:41:19.2 & $-47$:06:03.4 & $265.42$ & CH87  \\
shrds890 & 16:38:58.4 & $-46$:42:18.8 & G337.996+00.081 & C & 16:39:02.6 & $-46$:42:13.2 & $67.80$ &  \\
 & & & G338.009+00.016 & C & 16:39:22.4 & $-46$:44:13.0 & $101.02$ &  \\
shrds891 & 16:40:02.0 & $-46$:51:07.3 & G337.920$-$00.158 & Q & 16:39:47.4 & $-46$:55:09.8 & $35.87$ &  \\
 & & & G337.926$-$00.133 & Q & 16:39:42.2 & $-46$:53:53.7 & $16.13$ &  \\
 & & & G337.986$-$00.144 & Q & 16:39:59.0 & $-46$:51:37.9 & $19.35$ &  \\
 & & & G338.002$-$00.149 & C & 16:40:04.1 & $-46$:51:07.2 & $19.35$ &  \\
 & & & G338.003$-$00.121 & K & 16:39:57.0 & $-46$:49:58.3 & $276.32$ & CH87  \\
 & & & G338.114$-$00.193 & K & 16:40:41.8 & $-46$:47:51.6 & $271.53$ & CH87  \\
shrds892 & 16:39:21.1 & $-46$:44:00.4 & G337.996+00.081 & C & 16:39:02.6 & $-46$:42:13.2 & $67.80$ &  \\
 & & & G338.003$-$00.121 & K & 16:39:57.0 & $-46$:49:58.3 & $276.32$ & CH87  \\
 & & & G338.009+00.016 & C & 16:39:22.4 & $-46$:44:13.0 & $101.02$ &  \\
 & & & G338.075+00.016 & K & 16:39:38.0 & $-46$:41:17.4 & $75.12$ & CH87  \\
shrds1219 & 16:39:58.1 & $-46$:45:05.0 & G338.003$-$00.121 & K & 16:39:57.0 & $-46$:49:58.3 & $276.32$ & CH87  \\
 & & & G338.066$-$00.069 & C & 16:39:58.1 & $-46$:45:04.3 & $35.88$ &  \\
 & & & G338.075+00.016 & K & 16:39:38.0 & $-46$:41:17.4 & $75.12$ & CH87  \\
 & & & G338.080$-$00.028 & Q & 16:39:50.6 & $-46$:42:48.6 & $34.89$ &  \\
 & & & G338.114$-$00.193 & K & 16:40:41.8 & $-46$:47:51.6 & $271.53$ & CH87  \\
shrds893 & 16:39:38.7 & $-46$:39:37.6 & G338.009+00.016 & C & 16:39:22.4 & $-46$:44:13.0 & $101.02$ &  \\
 & & & G338.075+00.016 & K & 16:39:38.0 & $-46$:41:17.4 & $75.12$ & CH87  \\
 & & & G338.080$-$00.028 & Q & 16:39:50.6 & $-46$:42:48.6 & $34.89$ &  \\
 & & & G338.106+00.020 & C & 16:39:44.1 & $-46$:39:43.5 & $50.45$ &  \\
shrds894 & 16:42:01.7 & $-46$:47:02.3 & G338.263$-$00.364 & C & 16:42:01.2 & $-46$:47:54.5 & $35.26$ &  \\
 & & & G338.271$-$00.293 & Q & 16:41:44.4 & $-46$:44:45.2 & $25.86$ &  \\
 & & & G338.289$-$00.373 & C & 16:42:09.5 & $-46$:47:04.9 & $59.11$ &  \\
 & & & G338.328$-$00.291 & Q & 16:41:57.1 & $-46$:42:06.7 & $54.93$ &  \\
shrds896 & 16:41:06.8 & $-46$:32:35.6 & G338.360$-$00.095 & C & 16:41:12.8 & $-46$:32:52.2 & $94.24$ &  \\
 & & & G338.364$-$00.020 & C & 16:40:54.3 & $-46$:29:44.5 & $54.03$ &  \\
 & & & G338.374$-$00.152 & C & 16:41:31.1 & $-46$:34:31.1 & $34.37$ &  \\
 & & & G338.430+00.048 & K & 16:40:51.8 & $-46$:24:04.2 & $346.56$ & CH87  \\
caswell22 & 16:41:51.7 & $-46$:35:04.5 & G338.344$-$00.159 & Q & 16:41:26.0 & $-46$:36:08.9 & $34.37$ &  \\
 & & & G338.374$-$00.152 & C & 16:41:31.1 & $-46$:34:31.1 & $34.37$ &  \\
 & & & G338.405$-$00.203 & K & 16:41:51.7 & $-46$:35:09.4 & $63.49$ & CH87  \\
 & & & G338.430$-$00.214 & Q & 16:42:00.2 & $-46$:34:26.3 & $38.72$ &  \\
 & & & G338.446$-$00.261 & Q & 16:42:16.3 & $-46$:35:34.8 & $21.21$ &  \\
 & & & G338.450$-$00.250 & Q & 16:42:14.3 & $-46$:34:57.8 & $21.21$ &  \\
 & & & G338.461$-$00.217 & Q & 16:42:08.1 & $-46$:33:09.7 & $43.86$ &  \\
 & & & G338.462$-$00.262 & C & 16:42:20.3 & $-46$:34:54.6 & $138.65$ &  \\
ch221 & 16:42:01.4 & $-46$:36:27.3 & G338.405$-$00.203 & K & 16:41:51.7 & $-46$:35:09.4 & $63.49$ & CH87  \\
 & & & G338.430$-$00.214 & Q & 16:42:00.2 & $-46$:34:26.3 & $38.72$ &  \\
 & & & G338.446$-$00.261 & Q & 16:42:16.3 & $-46$:35:34.8 & $21.21$ &  \\
 & & & G338.450$-$00.250 & Q & 16:42:14.3 & $-46$:34:57.8 & $21.21$ &  \\
 & & & G338.461$-$00.217 & Q & 16:42:08.1 & $-46$:33:09.7 & $43.86$ &  \\
 & & & G338.462$-$00.262 & C & 16:42:20.3 & $-46$:34:54.6 & $138.65$ &  \\
shrds898 & 16:42:16.2 & $-46$:35:05.8 & G338.405$-$00.203 & K & 16:41:51.7 & $-46$:35:09.4 & $63.49$ & CH87  \\
 & & & G338.430$-$00.214 & Q & 16:42:00.2 & $-46$:34:26.3 & $38.72$ &  \\
 & & & G338.446$-$00.261 & Q & 16:42:16.3 & $-46$:35:34.8 & $21.21$ &  \\
 & & & G338.450$-$00.250 & Q & 16:42:14.3 & $-46$:34:57.8 & $21.21$ &  \\
 & & & G338.461$-$00.217 & Q & 16:42:08.1 & $-46$:33:09.7 & $43.86$ &  \\
 & & & G338.462$-$00.262 & C & 16:42:20.3 & $-46$:34:54.6 & $138.65$ &  \\
shrds899 & 16:42:09.7 & $-46$:25:15.8 & G338.565$-$00.151 & C & 16:42:14.7 & $-46$:25:50.8 & $155.02$ &  \\
shrds900 & 16:41:28.9 & $-46$:18:11.8 & G338.430+00.048 & K & 16:40:51.8 & $-46$:24:04.2 & $346.56$ & CH87  \\
 & & & G338.576+00.020 & C & 16:41:32.7 & $-46$:18:36.6 & $135.11$ &  \\
 & & & G338.596$-$00.007 & Q & 16:41:44.3 & $-46$:18:46.5 & $31.74$ &  \\
shrds901 & 16:41:09.7 & $-46$:10:52.9 & G338.628+00.145 & C & 16:41:12.1 & $-46$:11:19.0 & $88.43$ &  \\
shrds1223 & 16:39:42.0 & $-45$:47:21.8 & G338.706+00.645 & K & 16:39:20.5 & $-45$:47:52.8 & $181.86$ & CH87  \\
 & & & G338.861+00.597 & G & 16:40:08.4 & $-45$:42:52.2 & $460.33$ &  \\
shrds904 & 16:43:56.7 & $-46$:20:15.1 & G338.837$-$00.318 & C & 16:44:00.9 & $-46$:20:09.4 & $118.21$ &  \\
shrds905 & 16:40:51.7 & $-45$:51:18.6 & G338.816+00.403 & C & 16:40:48.2 & $-45$:52:36.9 & $135.03$ &  \\
 & & & G338.848+00.412 & Q & 16:40:53.1 & $-45$:50:48.6 & $18.21$ &  \\
 & & & G338.851+00.405 & C & 16:40:55.5 & $-45$:50:56.0 & $18.21$ &  \\
 & & & G338.861+00.597 & G & 16:40:08.4 & $-45$:42:52.2 & $460.33$ &  \\
 & & & G338.896+00.384 & Q & 16:41:11.2 & $-45$:49:44.6 & $18.61$ &  \\
 & & & G338.901+00.348 & Q & 16:41:21.7 & $-45$:50:57.5 & $67.95$ &  \\
 & & & G338.904+00.393 & Q & 16:41:10.7 & $-45$:49:02.3 & $18.61$ &  \\
 & & & G338.926+00.392 & C & 16:41:16.1 & $-45$:48:05.9 & $80.90$ &  \\
shrds1225 & 16:40:29.0 & $-45$:44:17.0 & G338.861+00.597 & G & 16:40:08.4 & $-45$:42:52.2 & $460.33$ &  \\
 & & & G338.883+00.537 & G & 16:40:28.9 & $-45$:44:16.1 & $82.68$ &  \\
 & & & G338.906+00.557 & Q & 16:40:28.9 & $-45$:42:26.1 & $25.33$ &  \\
 & & & G338.911+00.615 & K & 16:40:15.1 & $-45$:39:53.3 & $226.25$ & CH87  \\
 & & & G338.915+00.547 & Q & 16:40:33.6 & $-45$:42:25.8 & $25.33$ &  \\
 & & & G338.921+00.549 & Q & 16:40:34.3 & $-45$:42:03.6 & $27.09$ &  \\
 & & & G338.925+00.563 & Q & 16:40:31.6 & $-45$:41:19.5 & $25.33$ &  \\
shrds906 & 16:41:12.3 & $-45$:48:14.3 & G338.816+00.403 & C & 16:40:48.2 & $-45$:52:36.9 & $135.03$ &  \\
 & & & G338.848+00.412 & Q & 16:40:53.1 & $-45$:50:48.6 & $18.21$ &  \\
 & & & G338.851+00.405 & C & 16:40:55.5 & $-45$:50:56.0 & $18.21$ &  \\
 & & & G338.896+00.384 & Q & 16:41:11.2 & $-45$:49:44.6 & $18.61$ &  \\
 & & & G338.901+00.348 & Q & 16:41:21.7 & $-45$:50:57.5 & $67.95$ &  \\
 & & & G338.904+00.393 & Q & 16:41:10.7 & $-45$:49:02.3 & $18.61$ &  \\
 & & & G338.917+00.382 & Q & 16:41:16.6 & $-45$:48:53.5 & $23.22$ &  \\
 & & & G338.926+00.392 & C & 16:41:16.1 & $-45$:48:05.9 & $80.90$ &  \\
ch225 & 16:43:20.0 & $-46$:07:20.8 & G338.934$-$00.067 & K & 16:43:17.1 & $-46$:05:53.2 & $241.13$ & CH87  \\
 & & & G338.957$-$00.032 & Q & 16:43:13.2 & $-46$:03:27.7 & $24.65$ &  \\
shrds908 & 16:43:30.2 & $-45$:55:08.6 & G339.103+00.008 & C & 16:43:35.8 & $-45$:55:15.6 & $110.44$ &  \\
 & & & G339.158+00.009 & Q & 16:43:47.9 & $-45$:52:43.2 & $25.91$ &  \\
shrds909 & 16:42:55.3 & $-45$:48:58.4 & G339.094+00.208 & Q & 16:42:41.8 & $-45$:47:47.3 & $36.60$ &  \\
 & & & G339.106+00.152 & C & 16:42:59.1 & $-45$:49:28.5 & $52.91$ &  \\
 & & & G339.233+00.243 & K & 16:43:04.1 & $-45$:40:07.0 & $484.34$ & CH87  \\
shrds910 & 16:47:00.5 & $-46$:24:45.9 & G339.169$-$00.698 & C & 16:46:56.1 & $-46$:19:52.1 & $584.29$ &  \\
shrds913 & 16:42:59.8 & $-45$:39:56.8 & G339.216+00.263 & C & 16:42:55.2 & $-45$:40:07.4 & $52.80$ &  \\
 & & & G339.233+00.243 & K & 16:43:04.1 & $-45$:40:07.0 & $484.34$ & CH87  \\
shrds1228 & 16:44:06.9 & $-45$:49:04.5 & G339.211+00.038 & C & 16:43:52.3 & $-45$:49:11.0 & $140.03$ &  \\
 & & & G339.233$-$00.011 & Q & 16:44:10.2 & $-45$:50:08.1 & $35.40$ &  \\
 & & & G339.240+00.008 & C & 16:44:06.8 & $-45$:49:03.7 & $35.40$ &  \\
 & & & G339.299$-$00.020 & Q & 16:44:27.3 & $-45$:47:28.5 & $35.40$ &  \\
shrds915 & 16:46:50.3 & $-46$:11:50.5 & G339.147$-$00.600 & C & 16:46:25.2 & $-46$:17:03.1 & $284.17$ &  \\
 & & & G339.169$-$00.698 & C & 16:46:56.1 & $-46$:19:52.1 & $584.29$ &  \\
 & & & G339.275$-$00.607 & C & 16:46:55.9 & $-46$:11:28.9 & $117.65$ &  \\
shrds917 & 16:44:11.8 & $-45$:31:34.3 & G339.478+00.181 & C & 16:44:15.2 & $-45$:31:26.9 & $73.00$ &  \\
shrds918 & 16:44:37.1 & $-45$:34:31.5 & G339.478+00.181 & C & 16:44:15.2 & $-45$:31:26.9 & $73.00$ &  \\
 & & & G339.486+00.087 & C & 16:44:41.5 & $-45$:34:47.6 & $88.04$ &  \\
shrds919 & 16:46:59.2 & $-45$:50:33.7 & G339.531$-$00.417 & Q & 16:47:03.3 & $-45$:52:20.3 & $46.76$ &  \\
 & & & G339.548$-$00.385 & C & 16:46:58.7 & $-45$:50:23.9 & $52.32$ &  \\
 & & & G339.553$-$00.401 & C & 16:47:03.9 & $-45$:50:47.1 & $191.03$ &  \\
shrds920 & 16:44:05.6 & $-45$:23:39.2 & G339.556+00.282 & C & 16:44:06.7 & $-45$:23:58.5 & $82.94$ &  \\
shrds921 & 16:44:59.2 & $-45$:30:01.5 & G339.584+00.084 & C & 16:45:04.0 & $-45$:30:25.9 & $98.68$ &  \\
 & & & G339.590+00.083 & Q & 16:45:05.8 & $-45$:30:13.2 & $20.23$ &  \\
 & & & G339.596+00.079 & Q & 16:45:08.1 & $-45$:30:05.6 & $18.41$ &  \\
shrds922 & 16:44:30.2 & $-45$:18:39.6 & G339.676+00.283 & C & 16:44:33.1 & $-45$:18:28.2 & $57.87$ &  \\
 & & & G339.699+00.302 & Q & 16:44:33.3 & $-45$:16:40.7 & $21.20$ &  \\
g339.716$-$01.119 & 16:50:50.0 & $-46$:10:57.6 & G339.639$-$01.061 & Q & 16:50:17.5 & $-46$:12:17.9 & $172.04$ &  \\
 & & & G339.716$-$01.119 & C & 16:50:50.1 & $-46$:10:58.7 & $43.34$ &  \\
 & & & G339.717$-$01.102 & C & 16:50:45.9 & $-46$:10:17.8 & $45.09$ &  \\
 & & & G339.717$-$01.211 & C & 16:51:15.0 & $-46$:14:27.8 & $141.60$ &  \\
 & & & G339.723$-$01.119 & C & 16:50:51.8 & $-46$:10:40.0 & $33.95$ &  \\
g339.717$-$01.102 & 16:50:45.9 & $-46$:10:18.0 & G339.639$-$01.061 & Q & 16:50:17.5 & $-46$:12:17.9 & $172.04$ &  \\
 & & & G339.716$-$01.119 & C & 16:50:50.1 & $-46$:10:58.7 & $43.34$ &  \\
 & & & G339.717$-$01.102 & C & 16:50:45.9 & $-46$:10:17.8 & $45.09$ &  \\
 & & & G339.717$-$01.211 & C & 16:51:15.0 & $-46$:14:27.8 & $141.60$ &  \\
 & & & G339.723$-$01.119 & C & 16:50:51.8 & $-46$:10:40.0 & $33.95$ &  \\
shrds923 & 16:50:50.7 & $-46$:10:54.3 & G339.639$-$01.061 & Q & 16:50:17.5 & $-46$:12:17.9 & $172.04$ &  \\
 & & & G339.716$-$01.119 & C & 16:50:50.1 & $-46$:10:58.7 & $43.34$ &  \\
 & & & G339.717$-$01.102 & C & 16:50:45.9 & $-46$:10:17.8 & $45.09$ &  \\
 & & & G339.717$-$01.211 & C & 16:51:15.0 & $-46$:14:27.8 & $141.60$ &  \\
 & & & G339.723$-$01.119 & C & 16:50:51.8 & $-46$:10:40.0 & $33.95$ &  \\
shrds925 & 16:51:15.0 & $-46$:14:23.3 & G339.494$-$01.308 & C & 16:50:51.3 & $-46$:28:27.1 & $648.70$ &  \\
 & & & G339.717$-$01.211 & C & 16:51:15.0 & $-46$:14:27.8 & $141.60$ &  \\
g339.723$-$01.119 & 16:50:51.8 & $-46$:10:40.5 & G339.639$-$01.061 & Q & 16:50:17.5 & $-46$:12:17.9 & $172.04$ &  \\
 & & & G339.716$-$01.119 & C & 16:50:50.1 & $-46$:10:58.7 & $43.34$ &  \\
 & & & G339.717$-$01.102 & C & 16:50:45.9 & $-46$:10:17.8 & $45.09$ &  \\
 & & & G339.717$-$01.211 & C & 16:51:15.0 & $-46$:14:27.8 & $141.60$ &  \\
 & & & G339.723$-$01.119 & C & 16:50:51.8 & $-46$:10:40.0 & $33.95$ &  \\
shrds1230 & 16:46:04.6 & $-45$:24:45.8 & G339.728+00.068 & Q & 16:45:40.3 & $-45$:24:30.8 & $69.86$ &  \\
 & & & G339.756+00.063 & Q & 16:45:47.9 & $-45$:23:26.2 & $24.39$ &  \\
 & & & G339.761+00.052 & C & 16:45:51.9 & $-45$:23:38.3 & $32.65$ &  \\
 & & & G339.771+00.011 & C & 16:46:04.6 & $-45$:24:46.0 & $45.38$ &  \\
 & & & G339.777+00.022 & Q & 16:46:03.1 & $-45$:24:03.7 & $21.81$ &  \\
shrds928 & 16:45:03.4 & $-45$:14:54.5 & G339.781+00.243 & C & 16:45:07.0 & $-45$:15:17.0 & $119.86$ &  \\
 & & & G339.845+00.299 & K & 16:45:06.5 & $-45$:10:09.4 & $97.83$ & CH87  \\
ch230 & 16:45:11.6 & $-45$:11:28.9 & G339.781+00.243 & C & 16:45:07.0 & $-45$:15:17.0 & $119.86$ &  \\
 & & & G339.845+00.299 & K & 16:45:06.5 & $-45$:10:09.4 & $97.83$ & CH87  \\
shrds1234 & 16:46:34.5 & $-45$:14:38.8 & G339.952+00.052 & C & 16:46:34.2 & $-45$:14:54.9 & $82.98$ &  \\
 & & & G340.002+00.159 & K & 16:46:17.7 & $-45$:08:29.8 & $164.85$ & GBT HRDS  \\
shrds1236 & 16:48:01.3 & $-45$:17:13.4 & G340.029$-$00.158 & C & 16:47:45.8 & $-45$:19:33.0 & $101.45$ &  \\
 & & & G340.051$-$00.231 & K & 16:48:09.9 & $-45$:21:23.7 & $74.22$ & CH87  \\
 & & & G340.059$-$00.138 & C & 16:47:47.4 & $-45$:17:25.7 & $105.16$ &  \\
 & & & G340.068$-$00.075 & C & 16:47:32.7 & $-45$:14:32.6 & $107.10$ &  \\
 & & & G340.097$-$00.174 & C & 16:48:04.9 & $-45$:17:03.0 & $113.14$ &  \\
 & & & G340.118$-$00.142 & Q & 16:48:01.4 & $-45$:14:52.8 & $26.86$ &  \\
shrds1237 & 16:49:14.3 & $-45$:18:22.4 & G340.106$-$00.354 & K & 16:48:54.0 & $-45$:23:36.5 & $309.80$ & GBT HRDS  \\
 & & & G340.211$-$00.318 & K & 16:49:07.6 & $-45$:17:23.8 & $192.06$ & GBT HRDS  \\
 & & & G340.234$-$00.368 & Q & 16:49:25.7 & $-45$:18:15.8 & $35.86$ &  \\
 & & & G340.247$-$00.373 & C & 16:49:29.8 & $-45$:17:50.8 & $35.86$ &  \\
ch234 & 16:48:57.6 & $-45$:10:34.9 & G340.211$-$00.318 & K & 16:49:07.6 & $-45$:17:23.8 & $192.06$ & GBT HRDS  \\
 & & & G340.294$-$00.193 & K & 16:48:53.1 & $-45$:08:44.7 & $230.28$ & CH87  \\
 & & & G340.296$-$00.276 & C & 16:49:15.1 & $-45$:11:50.9 & $94.92$ &  \\
shrds930 & 16:54:03.6 & $-45$:23:08.7 & G340.678$-$01.049 & G & 16:54:01.6 & $-45$:23:43.0 & $324.38$ &  \\
 & & & G340.780$-$01.022 & K & 16:54:16.5 & $-45$:17:57.7 & $128.22$ & CH87  \\
shrds931 & 16:54:16.4 & $-45$:19:01.8 & G340.678$-$01.049 & G & 16:54:01.6 & $-45$:23:43.0 & $324.38$ &  \\
 & & & G340.766$-$01.033 & Q & 16:54:16.2 & $-45$:18:59.7 & $25.97$ &  \\
 & & & G340.780$-$01.022 & K & 16:54:16.5 & $-45$:17:57.7 & $128.22$ & CH87  \\
 & & & G340.828$-$01.005 & Q & 16:54:22.1 & $-45$:15:03.2 & $25.67$ &  \\
 & & & G340.850$-$01.022 & G & 16:54:31.3 & $-45$:14:40.0 & $211.54$ &  \\
 & & & G340.862$-$00.870 & G & 16:53:53.8 & $-45$:08:22.3 & $463.66$ &  \\
shrds932 & 16:54:22.4 & $-45$:15:05.0 & G340.678$-$01.049 & G & 16:54:01.6 & $-45$:23:43.0 & $324.38$ &  \\
 & & & G340.766$-$01.033 & Q & 16:54:16.2 & $-45$:18:59.7 & $25.97$ &  \\
 & & & G340.780$-$01.022 & K & 16:54:16.5 & $-45$:17:57.7 & $128.22$ & CH87  \\
 & & & G340.828$-$01.005 & Q & 16:54:22.1 & $-45$:15:03.2 & $25.67$ &  \\
 & & & G340.850$-$01.022 & G & 16:54:31.3 & $-45$:14:40.0 & $211.54$ &  \\
 & & & G340.862$-$00.870 & G & 16:53:53.8 & $-45$:08:22.3 & $463.66$ &  \\
shrds936 & 16:55:46.9 & $-45$:08:23.0 & G340.951$-$01.095 & G & 16:55:12.4 & $-45$:12:43.7 & $268.41$ &  \\
 & & & G341.071$-$01.128 & Q & 16:55:46.7 & $-45$:08:21.1 & $127.54$ &  \\
caswell23 & 16:52:33.0 & $-43$:23:38.0 & G341.962+00.437 & K & 16:52:08.3 & $-43$:27:37.8 & $131.28$ & GBT HRDS  \\
 & & & G342.062+00.417 & K & 16:52:34.4 & $-43$:23:45.8 & $175.01$ & CH87  \\
 & & & G342.139+00.430 & C & 16:52:47.2 & $-43$:19:41.0 & $78.90$ &  \\
ch239 & 16:52:37.8 & $-43$:22:28.9 & G342.062+00.417 & K & 16:52:34.4 & $-43$:23:45.8 & $175.01$ & CH87  \\
 & & & G342.102+00.500 & Q & 16:52:21.6 & $-43$:18:44.5 & $44.32$ &  \\
 & & & G342.125+00.494 & Q & 16:52:28.1 & $-43$:17:55.2 & $44.32$ &  \\
 & & & G342.139+00.430 & C & 16:52:47.2 & $-43$:19:41.0 & $78.90$ &  \\
shrds940 & 16:59:53.3 & $-44$:15:40.4 & G342.213$-$01.153 & Q & 16:59:53.3 & $-44$:15:39.8 & $76.65$ &  \\
shrds1238 & 16:55:11.2 & $-43$:21:30.1 & G342.349+00.100 & Q & 16:54:55.4 & $-43$:22:24.7 & $20.78$ &  \\
 & & & G342.360+00.107 & K & 16:54:55.9 & $-43$:21:38.3 & $66.77$ & GBT HRDS  \\
 & & & G342.363+00.124 & Q & 16:54:52.1 & $-43$:20:51.4 & $20.78$ &  \\
 & & & G342.377+00.133 & Q & 16:54:52.8 & $-43$:19:52.8 & $15.69$ &  \\
 & & & G342.384+00.122 & C & 16:54:57.1 & $-43$:19:58.2 & $20.78$ &  \\
 & & & G342.388+00.074 & C & 16:55:10.1 & $-43$:21:34.6 & $68.94$ &  \\
 & & & G342.389+00.125 & C & 16:54:57.4 & $-43$:19:37.8 & $20.78$ &  \\
shrds1239 & 16:55:55.5 & $-43$:24:03.1 & G342.354$-$00.047 & K & 16:55:34.2 & $-43$:27:43.5 & $123.51$ & CH87  \\
 & & & G342.429$-$00.046 & K & 16:55:49.4 & $-43$:24:10.4 & $61.54$ & GBT HRDS  \\
 & & & G342.438$-$00.061 & C & 16:55:55.2 & $-43$:24:19.0 & $43.80$ &  \\
shrds1240 & 16:58:38.4 & $-42$:46:45.4 & G343.224$-$00.065 & C & 16:58:37.3 & $-42$:47:35.6 & $97.50$ &  \\
 & & & G343.234$-$00.078 & C & 16:58:42.6 & $-42$:47:36.4 & $21.37$ &  \\
 & & & G343.328+00.009 & G & 16:58:39.6 & $-42$:39:58.6 & $586.12$ &  \\
shrds1241 & 16:59:04.2 & $-42$:41:24.8 & G343.328+00.009 & G & 16:58:39.6 & $-42$:39:58.6 & $586.12$ &  \\
 & & & G343.352$-$00.081 & C & 16:59:07.3 & $-42$:42:09.9 & $56.50$ &  \\
 & & & G343.353$-$00.068 & C & 16:59:04.2 & $-42$:41:38.1 & $29.71$ &  \\
 & & & G343.355$-$00.101 & Q & 16:59:13.1 & $-42$:42:46.3 & $35.96$ &  \\
 & & & G343.480$-$00.043 & K & 16:59:23.5 & $-42$:34:43.8 & $277.42$ & CH87  \\
caswell24 & 17:03:31.3 & $-42$:37:07.7 & G343.914$-$00.646 & K & 17:03:25.5 & $-42$:36:22.9 & $229.35$ & CH87  \\
ch244 & 17:03:27.0 & $-42$:35:41.5 & G343.914$-$00.646 & K & 17:03:25.5 & $-42$:36:22.9 & $229.35$ & CH87  \\
ch245 & 17:04:12.5 & $-42$:19:26.1 & G344.199$-$00.546 & Q & 17:03:56.1 & $-42$:19:09.5 & $68.88$ &  \\
 & & & G344.224$-$00.594 & K & 17:04:13.5 & $-42$:19:44.0 & $90.88$ & CH87  \\
caswell25 & 17:02:10.3 & $-41$:46:32.2 & G344.424+00.044 & K & 17:02:09.4 & $-41$:46:52.4 & $95.52$ & CH87  \\
ch246 & 17:02:11.5 & $-41$:46:02.2 & G344.424+00.044 & K & 17:02:09.4 & $-41$:46:52.4 & $95.52$ & CH87  \\
ch249 & 17:00:38.1 & $-40$:32:10.4 & G345.202+01.027 & K & 17:00:34.2 & $-40$:33:48.2 & $178.58$ & Q06  \\
 & & & G345.224+01.031 & Q & 17:00:37.6 & $-40$:32:37.5 & $37.32$ &  \\
 & & & G345.235+01.408 & K & 16:59:06.4 & $-40$:18:10.1 & $1371.77$ & CH87  \\
 & & & G345.324+01.022 & K & 17:00:59.2 & $-40$:28:13.8 & $132.23$ & Q06  \\
ch251 & 16:59:39.7 & $-40$:10:16.6 & G345.235+01.408 & K & 16:59:06.4 & $-40$:18:10.1 & $1371.77$ & CH87  \\
 & & & G345.338+01.442 & G & 16:59:17.8 & $-40$:12:01.2 & $132.23$ &  \\
 & & & G345.391+01.398 & K & 16:59:39.0 & $-40$:11:09.3 & $144.02$ & Q06  \\
 & & & G345.463+01.458 & G & 16:59:38.1 & $-40$:05:32.1 & $88.05$ &  \\
ch252 & 17:09:35.8 & $-41$:34:39.1 & G345.346$-$00.900 & G & 17:09:10.3 & $-41$:37:00.8 & $127.92$ &  \\
 & & & G345.377$-$00.904 & G & 17:09:17.2 & $-41$:35:39.2 & $34.59$ &  \\
 & & & G345.410$-$00.953 & K & 17:09:36.1 & $-41$:35:48.9 & $326.58$ & Q06  \\
 & & & G345.462$-$00.920 & G & 17:09:37.6 & $-41$:32:08.2 & $34.59$ &  \\
ch253 & 17:04:47.5 & $-40$:52:02.6 & G345.432+00.207 & K & 17:04:44.4 & $-40$:52:57.3 & $69.79$ & CH87  \\
 & & & G345.510+00.160 & C & 17:05:11.3 & $-40$:50:57.1 & $32.27$ &  \\
ch254 & 17:04:26.7 & $-40$:45:38.4 & G345.486+00.315 & K & 17:04:27.5 & $-40$:46:26.9 & $40.89$ & S04  \\
 & & & G345.486+00.399 & G & 17:04:06.3 & $-40$:43:22.4 & $168.28$ &  \\
 & & & G345.491+00.354 & K & 17:04:18.7 & $-40$:44:47.4 & $53.22$ & CH87  \\
 & & & G345.493+00.303 & K & 17:04:31.9 & $-40$:46:32.6 & $57.25$ & S04  \\
 & & & G345.504+00.347 & Q & 17:04:22.9 & $-40$:44:25.1 & $32.58$ &  \\
 & & & G345.518+00.260 & Q & 17:04:47.5 & $-40$:46:54.6 & $34.98$ &  \\
ch256 & 17:06:15.2 & $-40$:49:56.4 & G345.586$-$00.040 & K & 17:06:16.4 & $-40$:54:33.0 & $142.37$ & CH87  \\
 & & & G345.648+00.015 & C & 17:06:14.3 & $-40$:49:35.1 & $21.18$ &  \\
 & & & G345.651+00.015 & K & 17:06:15.0 & $-40$:49:27.5 & $98.25$ & CH87  \\
 & & & G345.656$-$00.016 & Q & 17:06:23.8 & $-40$:50:20.4 & $48.14$ &  \\
 & & & G345.673$-$00.130 & Q & 17:06:55.9 & $-40$:53:38.7 & $331.27$ &  \\
 & & & G345.696$-$00.055 & Q & 17:06:41.2 & $-40$:49:49.4 & $80.40$ &  \\
 & & & G345.700$-$00.012 & Q & 17:06:31.2 & $-40$:48:05.8 & $52.47$ &  \\
g345.864$-$01.103 & 17:11:41.2 & $-41$:19:14.2 & G345.864$-$01.103 & C & 17:11:41.1 & $-41$:19:13.5 & $53.62$ &  \\
 & & & G345.895$-$01.108 & C & 17:11:48.3 & $-41$:17:54.4 & $77.02$ &  \\
ch260 & 17:08:42.4 & $-40$:03:53.8 & G346.521+00.086 & K & 17:08:41.7 & $-40$:05:08.2 & $59.15$ & Q06  \\
 & & & G346.530+00.115 & Q & 17:08:36.2 & $-40$:03:40.6 & $41.53$ &  \\
 & & & G346.546+00.061 & Q & 17:08:52.8 & $-40$:04:50.8 & $29.38$ &  \\
ch263 & 17:13:05.3 & $-39$:00:19.4 & G347.862+00.004 & K & 17:13:09.6 & $-39$:03:13.8 & $89.85$ & GBT HRDS  \\
 & & & G347.891+00.042 & K & 17:13:05.4 & $-39$:00:28.9 & $42.65$ & CH87  \\
 & & & G347.908+00.051 & K & 17:13:06.0 & $-38$:59:19.0 & $42.65$ & CH87  \\
 & & & G347.965+00.059 & Q & 17:13:14.5 & $-38$:56:17.4 & $21.40$ &  \\
 & & & G347.990+00.048 & C & 17:13:21.6 & $-38$:55:26.4 & $231.61$ &  \\
fa642 & 17:16:32.4 & $-39$:27:17.6 & G347.921$-$00.763 & K & 17:16:33.3 & $-39$:27:12.3 & $69.07$ & GBT HRDS  \\
ch264 & 17:15:19.3 & $-39$:13:49.2 & G347.966$-$00.433 & C & 17:15:18.0 & $-39$:13:29.5 & $33.62$ &  \\
 & & & G347.996$-$00.380 & Q & 17:15:10.2 & $-39$:10:11.3 & $89.82$ &  \\
 & & & G348.000$-$00.496 & K & 17:15:40.1 & $-39$:14:02.7 & $345.41$ & Q06  \\
ch266 & 17:18:24.5 & $-39$:19:37.3 & G348.249$-$00.971 & K & 17:18:24.8 & $-39$:18:20.1 & $289.65$ & Q06  \\
ch268 & 17:20:02.8 & $-38$:57:31.6 & G348.658$-$01.044 & Q & 17:19:56.1 & $-39$:00:46.6 & $27.32$ &  \\
 & & & G348.686$-$01.036 & Q & 17:19:58.8 & $-38$:59:06.0 & $27.32$ &  \\
 & & & G348.691$-$00.826 & K & 17:19:06.6 & $-38$:51:37.7 & $1328.28$ & Q06  \\
 & & & G348.695$-$01.028 & G & 17:19:58.5 & $-38$:58:23.9 & $27.32$ &  \\
 & & & G348.698$-$01.019 & Q & 17:19:56.7 & $-38$:57:56.2 & $27.32$ &  \\
 & & & G348.710$-$01.044 & K & 17:20:05.2 & $-38$:58:12.7 & $388.02$ & Q06  \\
 & & & G348.938$-$01.148 & G & 17:21:11.7 & $-38$:50:32.5 & $1003.59$ &  \\
fa644 & 17:16:59.8 & $-38$:19:28.6 & G348.855$-$00.165 & Q & 17:16:49.7 & $-38$:20:43.2 & $20.62$ &  \\
 & & & G348.858$-$00.167 & Q & 17:16:50.9 & $-38$:20:39.6 & $71.33$ &  \\
 & & & G348.881$-$00.174 & Q & 17:16:56.6 & $-38$:19:45.8 & $27.14$ &  \\
 & & & G348.890$-$00.190 & Q & 17:17:02.3 & $-38$:19:53.3 & $20.99$ &  \\
 & & & G348.892$-$00.179 & K & 17:16:59.9 & $-38$:19:24.7 & $28.14$ & GBT HRDS  \\
gs038 & 17:17:27.3 & $-37$:51:05.9 & G349.293+00.019 & Q & 17:17:21.4 & $-37$:52:55.2 & $21.76$ &  \\
 & & & G349.297+00.088 & Q & 17:17:05.0 & $-37$:50:19.6 & $22.35$ &  \\
 & & & G349.328+00.020 & K & 17:17:27.2 & $-37$:51:09.6 & $83.62$ & GBT HRDS  \\
ch273 & 17:19:30.0 & $-37$:09:31.9 & G350.082+00.149 & Q & 17:19:06.7 & $-37$:09:43.0 & $65.79$ &  \\
 & & & G350.092+00.087 & K & 17:19:23.9 & $-37$:11:22.7 & $39.60$ & Q06  \\
 & & & G350.092+00.100 & Q & 17:19:20.6 & $-37$:10:55.8 & $20.66$ &  \\
 & & & G350.094+00.107 & Q & 17:19:19.1 & $-37$:10:34.0 & $20.66$ &  \\
 & & & G350.104+00.087 & Q & 17:19:25.8 & $-37$:10:46.2 & $20.66$ &  \\
 & & & G350.105+00.064 & Q & 17:19:31.7 & $-37$:11:31.2 & $19.99$ &  \\
 & & & G350.105+00.081 & K & 17:19:27.5 & $-37$:10:56.2 & $39.60$ & Q06  \\
 & & & G350.112+00.036 & Q & 17:19:39.9 & $-37$:12:09.2 & $34.53$ &  \\
 & & & G350.117+00.067 & Q & 17:19:33.0 & $-37$:10:49.6 & $20.66$ &  \\
 & & & G350.117+00.126 & C & 17:19:18.4 & $-37$:08:47.0 & $31.70$ &  \\
 & & & G350.127+00.069 & K & 17:19:34.3 & $-37$:10:16.0 & $62.39$ & Q06  \\
 & & & G350.172+00.028 & Q & 17:19:52.2 & $-37$:09:27.9 & $20.25$ &  \\
ch274 & 17:17:04.6 & $-36$:20:01.5 & G350.401+01.037 & G & 17:16:24.6 & $-36$:23:21.2 & $372.02$ &  \\
 & & & G350.482+00.951 & K & 17:16:59.4 & $-36$:22:22.1 & $96.62$ & L89  \\
 & & & G350.505+00.956 & K & 17:17:02.2 & $-36$:21:04.1 & $96.62$ & L89  \\
 & & & G350.594+01.149 & G & 17:16:30.8 & $-36$:10:01.7 & $1413.65$ &  \\
 & & & G350.617+00.984 & G & 17:17:14.8 & $-36$:14:38.4 & $574.86$ &  \\
ch275 & 17:21:53.6 & $-36$:39:29.7 & G350.769$-$00.079 & K & 17:22:00.7 & $-36$:43:40.9 & $75.01$ & GBT HRDS  \\
 & & & G350.781$-$00.027 & K & 17:21:50.1 & $-36$:41:20.8 & $93.75$ & L89  \\
 & & & G350.850$-$00.040 & Q & 17:22:04.9 & $-36$:38:21.9 & $43.48$ &  \\
overlap1 & 17:20:17.7 & $-35$:54:29.2 & G351.170+00.704 & K & 17:19:57.3 & $-35$:57:09.5 & $171.48$ & Q06  \\
 & & & G351.246+00.673 & K & 17:20:17.7 & $-35$:54:29.2 & $131.55$ & Q06  \\
 & & & G351.311+00.663 & K & 17:20:31.2 & $-35$:51:37.7 & $119.03$ & Q06  \\
 & & & G351.383+00.737 & K & 17:20:25.3 & $-35$:45:31.9 & $303.11$ & Q06  \\
g351.311+ & 17:20:31.2 & $-35$:51:37.7 & G351.246+00.673 & K & 17:20:17.7 & $-35$:54:29.2 & $131.55$ & Q06  \\
 & & & G351.311+00.663 & K & 17:20:31.2 & $-35$:51:37.7 & $119.03$ & Q06  \\
 & & & G351.348+00.593 & G & 17:20:54.4 & $-35$:52:12.1 & $125.78$ &  \\
 & & & G351.367+00.640 & K & 17:20:46.0 & $-35$:49:37.8 & $107.61$ & Q06  \\
 & & & G351.383+00.737 & K & 17:20:25.3 & $-35$:45:31.9 & $303.11$ & Q06  \\
ch278 & 17:25:33.0 & $-36$:22:05.8 & G351.472$-$00.458 & K & 17:25:32.7 & $-36$:21:41.8 & $128.48$ & Q06  \\
 & & & G351.516$-$00.540 & G & 17:26:00.4 & $-36$:22:16.3 & $376.36$ &  \\
 & & & G351.524$-$00.346 & C & 17:25:13.7 & $-36$:15:20.3 & $261.85$ &  \\
ch279 & 17:25:27.2 & $-36$:11:36.3 & G351.524$-$00.346 & C & 17:25:13.7 & $-36$:15:20.3 & $261.85$ &  \\
 & & & G351.570$-$00.372 & Q & 17:25:27.8 & $-36$:13:55.2 & $20.57$ &  \\
 & & & G351.575$-$00.350 & Q & 17:25:23.2 & $-36$:12:56.3 & $20.57$ &  \\
 & & & G351.584$-$00.350 & K & 17:25:24.8 & $-36$:12:30.4 & $80.00$ & L89  \\
ch280 & 17:23:22.6 & $-35$:53:17.2 & G351.557+00.211 & K & 17:23:02.7 & $-35$:54:53.2 & $174.24$ & L89  \\
 & & & G351.558+00.164 & G & 17:23:14.3 & $-35$:56:25.6 & $43.65$ &  \\
 & & & G351.620+00.143 & K & 17:23:29.9 & $-35$:54:05.1 & $207.85$ & L89  \\
 & & & G351.698+00.152 & G & 17:23:40.7 & $-35$:49:54.9 & $143.33$ &  \\
ch282 & 17:29:18.9 & $-36$:39:55.6 & G351.555$-$01.259 & G & 17:29:05.3 & $-36$:44:18.6 & $128.02$ &  \\
 & & & G351.589$-$01.172 & Q & 17:28:49.3 & $-36$:39:43.7 & $164.94$ &  \\
 & & & G351.646$-$01.252 & K & 17:29:18.5 & $-36$:39:30.9 & $132.23$ & Q06  \\
 & & & G351.650$-$01.325 & G & 17:29:37.6 & $-36$:41:45.4 & $87.60$ &  \\
 & & & G351.688$-$01.169 & K & 17:29:04.8 & $-36$:34:39.7 & $216.51$ & Q06  \\
 & & & G351.711$-$01.268 & G & 17:29:33.3 & $-36$:36:48.4 & $78.24$ &  \\
ch283 & 17:29:05.0 & $-36$:34:15.6 & G351.589$-$01.172 & Q & 17:28:49.3 & $-36$:39:43.7 & $164.94$ &  \\
 & & & G351.646$-$01.252 & K & 17:29:18.5 & $-36$:39:30.9 & $132.23$ & Q06  \\
 & & & G351.688$-$01.169 & K & 17:29:04.8 & $-36$:34:39.7 & $216.51$ & Q06  \\
fa016 & 17:27:47.6 & $-35$:39:14.4 & G352.251$-$00.442 & Q & 17:27:37.9 & $-35$:42:23.6 & $99.21$ &  \\
 & & & G352.313$-$00.442 & K & 17:27:48.0 & $-35$:39:17.5 & $79.13$ & GBT HRDS  \\
 & & & G352.333$-$00.455 & Q & 17:27:54.5 & $-35$:38:43.8 & $16.95$ &  \\
 & & & G352.337$-$00.451 & Q & 17:27:54.1 & $-35$:38:23.2 & $37.86$ &  \\
ch286 & 17:27:30.8 & $-35$:15:26.3 & G352.527$-$00.147 & K & 17:27:10.9 & $-35$:18:47.2 & $91.33$ & GBT HRDS  \\
 & & & G352.576$-$00.153 & K & 17:27:20.4 & $-35$:16:32.7 & $410.36$ & GBT HRDS  \\
 & & & G352.597$-$00.188 & K & 17:27:32.3 & $-35$:16:39.3 & $118.41$ & Q06  \\
ch293 & 17:30:31.3 & $-34$:41:00.4 & G353.408$-$00.381 & K & 17:30:30.9 & $-34$:42:31.5 & $193.23$ & Q06  \\
 & & & G353.431$-$00.291 & Q & 17:30:12.6 & $-34$:38:23.7 & $75.63$ &  \\
 & & & G353.495$-$00.384 & Q & 17:30:45.5 & $-34$:38:15.1 & $102.83$ &  \\
ch297 & 17:31:18.0 & $-33$:52:03.2 & G354.175$-$00.062 & K & 17:31:15.8 & $-33$:53:33.1 & $256.70$ & L89  \\
 & & & G354.181$-$00.100 & G & 17:31:26.0 & $-33$:54:30.4 & $38.55$ &  \\
ch298 & 17:31:29.7 & $-33$:33:07.8 & G354.420+00.033 & K & 17:31:31.8 & $-33$:38:08.9 & $89.32$ & GBT HRDS  \\
 & & & G354.465+00.079 & K & 17:31:27.7 & $-33$:34:22.3 & $175.90$ & L89  \\
 & & & G354.497+00.084 & Q & 17:31:31.4 & $-33$:32:34.8 & $23.39$ &  \\
 & & & G354.532+00.057 & G & 17:31:43.7 & $-33$:31:44.3 & $203.39$ &  \\
ch301 & 17:31:42.0 & $-33$:02:41.3 & G354.936+00.330 & K & 17:31:41.5 & $-33$:02:28.6 & $68.81$ & CH87  \\
fa032 & 17:33:29.6 & $-32$:48:02.3 & G355.244+00.109 & K & 17:33:22.6 & $-32$:54:13.9 & $405.64$ & L89  \\
 & & & G355.344+00.145 & K & 17:33:29.6 & $-32$:48:02.3 & $42.50$ & GBT HRDS  \\
ch303 & 17:33:41.4 & $-31$:46:09.8 & G356.230+00.670 & K & 17:33:41.3 & $-31$:46:17.6 & $149.30$ & L89  \\
 & & & G356.270+00.698 & G & 17:33:40.7 & $-31$:43:20.9 & $49.97$ &  \\
 & & & G356.290+00.693 & G & 17:33:45.0 & $-31$:42:30.9 & $49.97$ &  \\
 & & & G356.318+00.600 & C & 17:34:11.3 & $-31$:44:07.5 & $278.99$ &  \\
ch304 & 17:37:22.7 & $-32$:10:55.4 & G356.283$-$00.236 & Q & 17:37:25.0 & $-32$:12:56.7 & $50.08$ &  \\
 & & & G356.310$-$00.206 & K & 17:37:22.1 & $-32$:10:37.7 & $87.71$ & L89  \\
 & & & G356.325$-$00.234 & Q & 17:37:31.1 & $-32$:10:46.7 & $46.30$ &  \\
 & & & G356.347$-$00.230 & C & 17:37:33.5 & $-32$:09:32.0 & $69.35$ &  \\
gs108 & 17:42:28.2 & $-30$:09:30.7 & G358.541$-$00.076 & Q & 17:42:24.0 & $-30$:13:06.7 & $55.85$ &  \\
 & & & G358.552$-$00.026 & K & 17:42:13.7 & $-30$:10:56.9 & $42.50$ & GBT HRDS  \\
 & & & G358.561$-$00.096 & Q & 17:42:31.5 & $-30$:12:42.4 & $21.04$ &  \\
 & & & G358.563$-$00.067 & Q & 17:42:25.0 & $-30$:11:41.4 & $15.41$ &  \\
 & & & G358.586$-$00.076 & Q & 17:42:30.5 & $-30$:10:48.0 & $15.86$ &  \\
 & & & G358.599$-$00.086 & Q & 17:42:34.7 & $-30$:10:27.2 & $19.41$ &  \\
 & & & G358.600$-$00.058 & K & 17:42:28.3 & $-30$:09:30.9 & $47.54$ & GBT HRDS  \\
 & & & G358.616$-$00.077 & K & 17:42:35.1 & $-30$:09:17.8 & $42.50$ & GBT HRDS  \\
 & & & G358.618$-$00.060 & C & 17:42:31.4 & $-30$:08:39.5 & $21.70$ &  \\
 & & & G358.635$-$00.067 & Q & 17:42:35.6 & $-30$:08:01.7 & $11.73$ &  \\
 & & & G358.641$-$00.070 & Q & 17:42:37.1 & $-30$:07:48.6 & $14.14$ &  \\
 & & & G358.643$-$00.035 & K & 17:42:29.1 & $-30$:06:35.7 & $55.30$ & GBT HRDS  \\
 & & & G358.646$-$00.065 & Q & 17:42:36.8 & $-30$:07:25.0 & $13.03$ &  \\
 & & & G358.652$-$00.079 & K & 17:42:40.8 & $-30$:07:31.4 & $42.50$ & GBT HRDS  \\
ch307 & 17:42:33.7 & $-30$:08:37.4 & G358.541$-$00.076 & Q & 17:42:24.0 & $-30$:13:06.7 & $55.85$ &  \\
 & & & G358.561$-$00.096 & Q & 17:42:31.5 & $-30$:12:42.4 & $21.04$ &  \\
 & & & G358.563$-$00.067 & Q & 17:42:25.0 & $-30$:11:41.4 & $15.41$ &  \\
 & & & G358.586$-$00.076 & Q & 17:42:30.5 & $-30$:10:48.0 & $15.86$ &  \\
 & & & G358.599$-$00.086 & Q & 17:42:34.7 & $-30$:10:27.2 & $19.41$ &  \\
 & & & G358.600$-$00.058 & K & 17:42:28.3 & $-30$:09:30.9 & $47.54$ & GBT HRDS  \\
 & & & G358.616$-$00.077 & K & 17:42:35.1 & $-30$:09:17.8 & $42.50$ & GBT HRDS  \\
 & & & G358.618$-$00.060 & C & 17:42:31.4 & $-30$:08:39.5 & $21.70$ &  \\
 & & & G358.635$-$00.067 & Q & 17:42:35.6 & $-30$:08:01.7 & $11.73$ &  \\
 & & & G358.641$-$00.070 & Q & 17:42:37.1 & $-30$:07:48.6 & $14.14$ &  \\
 & & & G358.643$-$00.035 & K & 17:42:29.1 & $-30$:06:35.7 & $55.30$ & GBT HRDS  \\
 & & & G358.646$-$00.065 & Q & 17:42:36.8 & $-30$:07:25.0 & $13.03$ &  \\
 & & & G358.652$-$00.079 & K & 17:42:40.8 & $-30$:07:31.4 & $42.50$ & GBT HRDS  \\
 & & & G358.680$-$00.088 & K & 17:42:47.0 & $-30$:06:22.7 & $42.50$ & GBT HRDS  \\
 & & & G358.684$-$00.117 & K & 17:42:54.5 & $-30$:07:05.8 & $44.06$ & GBT HRDS  \\
 & & & G358.694$-$00.076 & K & 17:42:46.2 & $-30$:05:17.2 & $42.50$ & GBT HRDS  \\
fa054 & 17:42:05.0 & $-30$:04:03.9 & G358.633+00.062 & K & 17:42:05.0 & $-30$:04:03.9 & $42.50$ & GBT HRDS  \\
ch309 & 17:44:35.9 & $-29$:27:56.0 & G359.386$-$00.082 & K & 17:44:28.2 & $-29$:30:08.9 & $118.03$ & GBT HRDS  \\
 & & & G359.401$-$00.096 & Q & 17:44:33.5 & $-29$:29:48.2 & $14.78$ &  \\
 & & & G359.408$-$00.024 & Q & 17:44:17.7 & $-29$:27:11.9 & $22.17$ &  \\
 & & & G359.409$-$00.040 & C & 17:44:21.6 & $-29$:27:38.5 & $42.50$ &  \\
 & & & G359.418$-$00.105 & Q & 17:44:38.2 & $-29$:29:13.9 & $14.78$ &  \\
 & & & G359.432$-$00.036 & Q & 17:44:24.0 & $-29$:26:21.0 & $15.96$ &  \\
 & & & G359.434$-$00.024 & Q & 17:44:21.5 & $-29$:25:52.6 & $15.14$ &  \\
 & & & G359.436$-$00.091 & K & 17:44:37.5 & $-29$:27:52.1 & $98.55$ & CH87  \\
 & & & G359.441$-$00.069 & C & 17:44:33.1 & $-29$:26:55.6 & $19.28$ &  \\
 & & & G359.445$-$00.022 & Q & 17:44:22.7 & $-29$:25:15.2 & $18.60$ &  \\
 & & & G359.448$-$00.030 & C & 17:44:25.0 & $-29$:25:21.0 & $11.39$ &  \\
 & & & G359.452$-$00.042 & Q & 17:44:28.3 & $-29$:25:30.6 & $17.12$ &  \\
 & & & G359.455$-$00.066 & C & 17:44:34.4 & $-29$:26:06.9 & $18.20$ &  \\
 & & & G359.460$-$00.077 & C & 17:44:37.7 & $-29$:26:12.4 & $19.68$ &  \\
 & & & G359.464$-$00.094 & C & 17:44:42.3 & $-29$:26:32.5 & $40.82$ &  \\
 & & & G359.467$-$00.074 & C & 17:44:37.9 & $-29$:25:44.3 & $16.78$ &  \\
 & & & G359.481$-$00.081 & Q & 17:44:41.6 & $-29$:25:14.7 & $19.29$ &  \\
 & & & G359.483$-$00.045 & C & 17:44:33.4 & $-29$:24:00.6 & $35.19$ &  \\
 & & & G359.492$-$00.075 & C & 17:44:41.8 & $-29$:24:30.5 & $30.08$ &  \\
 & & & G359.499$-$00.063 & Q & 17:44:40.0 & $-29$:23:46.6 & $15.01$ &  \\
 & & & G359.504$-$00.108 & Q & 17:44:51.3 & $-29$:24:55.3 & $22.08$ &  \\
fa489 & 17:45:01.1 & $-29$:28:50.3 & G359.436$-$00.091 & K & 17:44:37.5 & $-29$:27:52.1 & $98.55$ & CH87  \\
 & & & G359.464$-$00.094 & C & 17:44:42.3 & $-29$:26:32.5 & $40.82$ &  \\
 & & & G359.467$-$00.173 & K & 17:45:01.1 & $-29$:28:50.3 & $42.50$ & GBT HRDS  \\
 & & & G359.504$-$00.108 & Q & 17:44:51.3 & $-29$:24:55.3 & $22.08$ &  \\
ch310 & 17:48:24.2 & $-27$:45:37.2 & G001.218$-$00.034 & K & 17:48:37.5 & $-27$:54:41.2 & $611.43$ & D80  \\
 & & & G001.321+00.101 & K & 17:48:20.4 & $-27$:45:11.4 & $58.74$ & GBT HRDS  \\
 & & & G001.330+00.088 & K & 17:48:24.7 & $-27$:45:11.9 & $42.50$ & GBT HRDS  \\
 & & & G001.330+00.145 & K & 17:48:11.5 & $-27$:43:22.5 & $78.61$ & GBT HRDS  \\
 & & & G001.362+00.118 & Q & 17:48:22.1 & $-27$:42:33.3 & $70.11$ &  \\
ch313 & 17:54:31.6 & $-25$:51:04.3 & G003.607$-$00.209 & K & 17:54:46.2 & $-25$:56:47.5 & $152.08$ & GBT HRDS  \\
 & & & G003.650$-$00.122 & K & 17:54:31.9 & $-25$:51:55.8 & $72.50$ & L89  \\
 & & & G003.664$-$00.098 & K & 17:54:28.3 & $-25$:50:27.4 & $31.96$ & GBT HRDS  \\
 & & & G003.676$-$00.100 & G & 17:54:30.5 & $-25$:49:54.2 & $29.02$ &  \\
overlap2 & 18:00:31.6 & $-24$:04:20.2 & G005.845$-$00.422 & G & 18:00:32.0 & $-24$:06:57.4 & $80.75$ &  \\
 & & & G005.883$-$00.399 & K & 18:00:31.5 & $-24$:04:18.9 & $22.35$ & Q06  \\
 & & & G005.885$-$00.393 & K & 18:00:30.5 & $-24$:04:00.5 & $22.35$ & Q06  \\
 & & & G005.886$-$00.331 & Q & 18:00:16.4 & $-24$:02:06.7 & $20.17$ &  \\
 & & & G005.887$-$00.443 & K & 18:00:42.2 & $-24$:05:23.0 & $436.69$ & Q06  \\
 & & & G005.900$-$00.431 & K & 18:00:41.1 & $-24$:04:21.9 & $107.69$ & Q06  \\
 & & & G005.902$-$00.360 & Q & 18:00:25.1 & $-24$:02:07.0 & $26.67$ &  \\
 & & & G005.905$-$00.460 & G & 18:00:48.5 & $-24$:04:58.4 & $60.79$ &  \\
 & & & G005.915$-$00.354 & G & 18:00:25.4 & $-24$:01:16.6 & $149.00$ &  \\
 & & & G005.923$-$00.392 & Q & 18:00:35.3 & $-24$:02:00.2 & $23.67$ &  \\
 & & & G005.933$-$00.416 & Q & 18:00:42.0 & $-24$:02:11.5 & $8.89$ &  \\
 & & & G005.939$-$00.426 & G & 18:00:45.2 & $-24$:02:11.1 & $60.79$ &  \\
overlap3 & 18:10:24.7 & $-19$:57:11.5 & G010.518$-$00.289 & Q & 18:09:54.4 & $-19$:58:35.0 & $257.52$ &  \\
 & & & G010.574$-$00.412 & G & 18:10:28.9 & $-19$:59:11.9 & $110.16$ &  \\
 & & & G010.581$-$00.378 & G & 18:10:22.0 & $-19$:57:51.5 & $33.27$ &  \\
 & & & G010.596$-$00.381 & K & 18:10:24.6 & $-19$:57:08.4 & $60.00$ & Q06  \\
 & & & G010.607$-$00.345 & Q & 18:10:17.9 & $-19$:55:32.7 & $11.18$ &  \\
 & & & G010.611$-$00.375 & G & 18:10:25.3 & $-19$:56:11.8 & $26.66$ &  \\
 & & & G010.617$-$00.336 & Q & 18:10:17.1 & $-19$:54:44.2 & $23.14$ &  \\
 & & & G010.617$-$00.405 & G & 18:10:32.7 & $-19$:56:43.8 & $60.22$ &  \\
 & & & G010.618$-$00.383 & G & 18:10:27.9 & $-19$:56:04.5 & $10.76$ &  \\
 & & & G010.621$-$00.318 & K & 18:10:13.7 & $-19$:54:02.4 & $42.50$ & GBT HRDS  \\
 & & & G010.621$-$00.380 & G & 18:10:27.6 & $-19$:55:48.5 & $14.20$ &  \\
 & & & G010.623$-$00.385 & G & 18:10:28.7 & $-19$:55:51.1 & $21.65$ &  \\
 & & & G010.626$-$00.373 & Q & 18:10:26.6 & $-19$:55:21.8 & $15.91$ &  \\
 & & & G010.629$-$00.339 & K & 18:10:19.3 & $-19$:54:11.1 & $42.50$ & GBT HRDS  \\
 & & & G010.629$-$00.342 & K & 18:10:20.1 & $-19$:54:17.6 & $12.97$ & GBT HRDS  \\
 & & & G010.631$-$00.388 & G & 18:10:30.5 & $-19$:55:30.8 & $26.00$ &  \\
 & & & G010.638$-$00.434 & K & 18:10:41.6 & $-19$:56:30.1 & $42.50$ & GBT HRDS  \\
 & & & G010.769$-$00.487 & K & 18:11:09.6 & $-19$:51:08.9 & $580.43$ & GBT HRDS  \\
g012.804$-$ & 18:14:15.1 & $-17$:55:59.0 & G012.726$-$00.219 & K & 18:14:08.4 & $-18$:00:23.6 & $32.97$ & GBT HRDS  \\
 & & & G012.761$-$00.133 & K & 18:13:53.4 & $-17$:56:04.4 & $208.38$ & L89  \\
 & & & G012.787$-$00.178 & G & 18:14:06.6 & $-17$:56:02.6 & $22.30$ &  \\
 & & & G012.788$-$00.218 & Q & 18:14:15.6 & $-17$:57:06.6 & $30.85$ &  \\
 & & & G012.794$-$00.188 & Q & 18:14:09.7 & $-17$:55:55.6 & $12.79$ &  \\
 & & & G012.794$-$00.199 & G & 18:14:12.1 & $-17$:56:15.2 & $19.29$ &  \\
 & & & G012.795$-$00.192 & Q & 18:14:10.6 & $-17$:55:58.3 & $9.19$ &  \\
 & & & G012.804$-$00.165 & Q & 18:14:05.6 & $-17$:54:44.4 & $17.83$ &  \\
 & & & G012.804$-$00.207 & K & 18:14:15.0 & $-17$:55:56.4 & $21.15$ & Q06  \\
 & & & G012.805$-$00.196 & K & 18:14:12.8 & $-17$:55:35.6 & $21.15$ & Q06  \\
 & & & G012.813$-$00.200 & K & 18:14:14.6 & $-17$:55:14.8 & $21.15$ & Q06  \\
 & & & G012.820$-$00.238 & G & 18:14:23.8 & $-17$:56:00.0 & $126.83$ &  \\
 & & & G012.829$-$00.170 & G & 18:14:09.8 & $-17$:53:33.9 & $22.74$ &  \\
 & & & G012.848$-$00.230 & Q & 18:14:25.5 & $-17$:54:15.9 & $16.92$ &  \\
 & & & G012.884$-$00.237 & G & 18:14:31.3 & $-17$:52:33.2 & $122.21$ &  \\
overlap4 & 18:14:35.7 & $-16$:45:09.9 & G013.857+00.226 & Q & 18:14:45.8 & $-16$:48:01.2 & $86.81$ &  \\
 & & & G013.880+00.285 & K & 18:14:35.7 & $-16$:45:09.7 & $144.31$ & Q06  \\
 & & & G013.905+00.219 & Q & 18:14:53.2 & $-16$:45:43.8 & $67.22$ &  \\
overlap5 & 18:31:04.2 & $-10$:22:45.0 & G021.356$-$00.179 & C & 18:30:44.3 & $-10$:22:10.5 & $51.82$ &  \\
 & & & G021.372$-$00.228 & Q & 18:30:56.8 & $-10$:22:42.0 & $23.76$ &  \\
 & & & G021.378$-$00.295 & Q & 18:31:11.9 & $-10$:24:13.9 & $43.26$ &  \\
 & & & G021.386$-$00.255 & K & 18:31:04.0 & $-10$:22:43.4 & $57.60$ & GBT HRDS  \\
 & & & G021.404$-$00.238 & C & 18:31:02.4 & $-10$:21:17.6 & $82.30$ &  \\
 & & & G021.433$-$00.273 & Q & 18:31:13.2 & $-10$:20:43.5 & $72.50$ &  \\
g025.397+ & 18:37:30.8 & $-6$:41:12.5 & G025.357+00.102 & Q & 18:37:11.6 & $-6$:41:25.5 & $122.47$ &  \\
 & & & G025.382$-$00.151 & K & 18:38:08.6 & $-6$:47:01.4 & $456.02$ & Q06  \\
 & & & G025.397+00.033 & K & 18:37:30.8 & $-6$:41:08.8 & $39.69$ & L89  \\
 & & & G025.398$-$00.031 & Q & 18:37:44.6 & $-6$:42:54.6 & $27.47$ &  \\
 & & & G025.401+00.021 & K & 18:37:33.7 & $-6$:41:17.7 & $28.72$ & L89  \\
 & & & G025.426+00.055 & Q & 18:37:29.3 & $-6$:39:02.0 & $22.58$ &  \\
 & & & G025.477+00.040 & K & 18:37:38.2 & $-6$:36:45.0 & $42.50$ & GBT HRDS  \\
g029.956$-$ & 18:46:04.6 & $-2$:39:26.7 & G029.889$-$00.007 & G & 18:45:54.5 & $-2$:42:39.1 & $49.40$ &  \\
 & & & G029.901$-$00.029 & G & 18:46:00.4 & $-2$:42:36.0 & $80.07$ &  \\
 & & & G029.928$-$00.057 & G & 18:46:09.3 & $-2$:41:55.7 & $103.10$ &  \\
 & & & G029.955$-$00.093 & G & 18:46:20.1 & $-2$:41:25.5 & $124.40$ &  \\
 & & & G029.956$-$00.020 & K & 18:46:04.5 & $-2$:39:25.2 & $94.36$ & Q06  \\
 & & & G029.978+00.020 & C & 18:45:58.4 & $-2$:37:07.4 & $30.99$ &  \\
 & & & G030.007$-$00.084 & G & 18:46:23.9 & $-2$:38:25.5 & $82.38$ &  \\
 & & & G030.014+00.017 & Q & 18:46:03.1 & $-2$:35:18.7 & $23.70$ &  \\
 & & & G030.015+00.025 & Q & 18:46:01.5 & $-2$:35:02.4 & $22.33$ &  \\
 & & & G030.022$-$00.042 & K & 18:46:16.6 & $-2$:36:31.4 & $60.94$ & GBT HRDS  \\
 & & & G030.030+00.005 & C & 18:46:07.4 & $-2$:34:45.9 & $38.18$ &  \\
\enddata
\tablenotetext{a}{The \textit{WISE} Catalog designation: ``K'' is known \hii\ region, ``C'' is \hii\ region candidate, ``Q'' is radio-quiet \hii\ region candidate, and ``G'' is \hii\ candidate associated with an \hii\ region group.}
\tablerefs{(GBT HRDS) \citet{anderson2011,anderson2015b,anderson2018}; (B11) \citet{balser2011}; (CH87) \citet{caswell1987}; (D80) \citet{downes1980}; (L89) \citet{lockman1989}; (Q06) \citet{quireza2006a}; (S04) \citet{sewilo2004}; (W70) \citet{wilson1970}}
\end{deluxetable*}
\end{longrotatetable}

